Predictor Antenna Systems: Exploiting Channel State Information for Vehicle Communications

Vehicle communication is one of the most important use cases in the fifth generation of wireless networks (5G). The growing demand for quality of service (QoS) characterized by performance metrics, such as spectrum efficiency, peak data rate, and outage probability, is mainly limited by inaccurate prediction/estimation of channel state information (CSI) of the rapidly changing environment around moving vehicles. One way to increase the prediction horizon of CSI in order to improve the QoS is deploying predictor antennas (PAs). A PA system consists of two sets of antennas typically mounted on the roof of a vehicle, where the PAs positioned at the front of the vehicle are used to predict the CSI observed by the receive antennas (RAs) that are aligned behind the PAs. In realistic PA systems, however, the actual benefit is affected by a variety of factors, including spatial mismatch, antenna utilization, temporal correlation of scattering environment, and CSI estimation error. This thesis investigates different resource allocation schemes for the PA systems under practical constraints.

==> Abstract.tex <==
Vehicle communication is one of the most important use cases in the fifth generation of wireless networks (5G).  The growing demand for quality of service (QoS) characterized by performance metrics, such as spectrum efficiency, peak data rate,  and outage probability, is mainly limited by inaccurate prediction/estimation of channel state information (CSI) of the rapidly changing environment around moving vehicles. One way to increase the prediction horizon of CSI in order to improve the  QoS is  deploying predictor antennas (PAs).  A PA system consists of two sets of antennas typically mounted on the roof of a vehicle, where the PAs positioned at the front of the vehicle are used to predict the CSI observed by the receive antennas (RAs) that are aligned behind the PAs. In  realistic PA systems, however, the actual benefit is affected by a variety of factors, including spatial mismatch, antenna utilization, temporal correlation of scattering environment, and  CSI estimation error. This thesis investigates different resource allocation schemes for the PA systems under practical constraints, with main contributions summarized as follows.

First, in Paper A, we study the PA system in the presence of the so-called spatial mismatch problem, i.e., when the channel observed by the PA is not exactly the same as the one experienced by the RA. We derive closed-form expressions for the throughput-optimized rate adaptation, and evaluate the system performance in various temporally-correlated conditions for the scattering environment. Our results indicate that PA-assisted adaptive rate adaptation leads to a considerable performance improvement, compared to the cases with no rate adaptation. Then, to simplify e.g., various integral calculations as well as different operations such as parameter optimization, in Paper B, we  propose a semi-linear approximation of the Marcum Q-function, and apply the proposed approximation to the evaluation of the PA system. We also perform deep analysis of the effect of various parameters such as antenna separation as well as CSI estimation error. As we show, our proposed approximation scheme enables us to analyze PA systems with high accuracy. 

The second part of the thesis focuses on improving the spectral efficiency of the PA system by involving the PA into data transmission. In Paper C,  we analyze the outage-limited performance of PA systems using hybrid automatic repeat request (HARQ). With our proposed approach, the PA is used not only for improving the CSI in the retransmissions to the RA, but also for data transmission in the initial round.  As we show in the analytical and the simulation results, the combination of PA and HARQ protocols makes it possible to improve the  spectral efficiency  and adapt transmission parameters to mitigate the effect of spatial mismatch. 






==> Acknowledgement.tex <==
\vspace{1cm}

As my PhD voyage is now half-way through, I would like to take the opportunity to recognize the people without whom this thesis would not have been possible.

First and foremost, I would like to express my deepest gratitude to Prof. Tommy Svensson for being my examiner and main supervisor and for giving me the opportunity to become a PhD student. Thank you for all the guidance, nice discussions and the constant support you have provided me for the last couple of years. This deepest gratitude also goes to my co-supervisor, Dr. Behrooz Makki, for over 1500 emails from you containing your fruitful comments and  detailed guidance, for the meetings you came all the way from Ericsson, for your valuable time even when you were super busy with the job hand-over and babies. I recommend everyone to collaborate with you and enjoy your kind, friendly, and pure personality.

Special thanks to Prof. Mohamed-Slim Alouini, for reviewing my draft and providing fruitful feedback and ideas. I would also like to thank Dr. Jingya Li for reading the rough draft of my paper, and all the help she has provided me outside of my research. I am also grateful to Prof. Mikael Sternad, Associate Prof. Carmen Botella, Prof. Xiaoming Chen, Dr. Fuxi Wen, and Dr. Nima Jamaly for all the nice discussions and collaborations we have had.

I would also like to thank the current and former members of the Communication Systems group. Many thanks to the head of our division, Prof. Erik Ström, and the head of our group, Prof. Fredrik Brännström, for ensuring a stimulating and joyful research atmosphere. Special thanks to Prof. Erik Agrell for our nice collaborations in the teaching work, and for everything you have shown me to be a kind and responsible teacher. Also, many thanks go to Professors Giuseppe Durisi, Henk Wymeersch, Alexandre Graell i Amat, Thomas Eriksson, and Jian Yang for the very interesting discussions in the courses. Gratitude also goes to Agneta,  Natasha,  Daniela,  Annie,  Yvonne, and  Madeleine for all your help. Thank you, Jinlin, Chao, Chenjie, Xinlin, Li, Yuxuan, Lei, Dapeng, Cristian, Johan, Keerthi, Anver, Shen, Roman, Chouaib, Mohammad, Björn, Sven, and Rahul for all the support and encouragement you have given to me.  I would also like to thank all my Chinese friends in Gothenburg for all the great moments we have experienced together. 

Special thanks to Yigeng, Xiao, Mengcheng, Pei, Hongxu, Qiang, and Kai for always being there for me. 

Finally, I would like to express my sincerest gratitude to mom and dad for your constant support, love, and encouragement over the years. I love you.




\vfill
\hfill   Hao Guo

\hfill  G\"{o}teborg, \TheMonth~\TheYear

\vfill



\clearpage

==> TemplateFiles/cover/Chalmers_Cover.tex <==

%% REQUIRED PACKAGES:
%% \usepackage{geography}
%% \usepackage{graphicx}
%% \usepackage{color}
%% \usepackage{tikz}
%% \usepackage{wrapfig}
%% \usepackage{amsmath}

\begingroup

    \usetikzlibrary{calc}
    \usetikzlibrary{positioning}
    \providecommand\rotatebox[2]{#2}%

    \ifx \TheThesisType\ThesisTypeLic
        \newcommand{\CoverBackground}{Chalmers_Cover_Lic}
        \newcommand{\CoverColor}{0.35,0.69,0.886}
    \else
        \newcommand{\CoverBackground}{Chalmers_Cover_PhD}
        \newcommand{\CoverColor}{0.11372549,0.30588235,0.61960784}
    \fi
    
    \newenvironment{covertext}[3][0.22,0.22,0.22]
        {
        \begin{minipage}[t]{14cm}
            \color[rgb]{#1}
            \fontfamily{phv}\fontsize{#2pt}{#3pt}\selectfont
        }
        {\end{minipage}}
    
    \noindent
    \begin{tikzpicture}[
        remember picture,
        overlay,
        anchor=north west,
        inner sep=0pt
        ]
        \node[anchor=center] at ($(current page.east)+(0.3, 0)$){
            \includegraphics[width=\pdfpagewidth,height=\pdfpageheight]{TemplateFiles/cover/\CoverBackground}
        };
        
        \node (image) at (19.15,-3.7){
            \ifx \TheCoverImage\undefined
            \else
                \if \TheCoverImage\empty
                \else
                    \includegraphics[width=14cm,height=8cm]{\TheCoverImage}
                \fi
            \fi
        };
        
        % Title
        \node (title) at ($ (image.north west) + (-.1,-8.5) $){
            \begin{covertext}{\TheCoverPageTitleFontSize}{\TheCoverPageTitleFontSize}
                \textbf{\TheCoverPageTitle} 
            \end{covertext}
        };
        % Subtitle
        \node (subtitle) at ($ (title.south west) + (0,-.2) $){
            \ifdefined \TheCoverPageSubtitle \if \TheCoverPageSubtitle\empty\else
                \begin{covertext}{11.5}{11.5}
                    \textit{\TheCoverPageSubtitle}
                \end{covertext}
            \fi\fi
        };
            
        % Name
        \node (author) at ($ (subtitle.south west) + (0,-1.5) $){
            \begin{covertext}{13.5}{0}
                \MakeUppercase{\TheAuthor}
            \end{covertext}
        };
            
        % Department
        \node (department) at (19.05,-20.55){
            \begin{covertext}[\CoverColor]{8}{10}
                \MakeUppercase{\textbf{DEPARTMENT OF \TheDepartment}}
            \end{covertext}
        };
        
        \node (contact) at  ($ (department.south west) + (0,-.25) $){
            \begin{covertext}{8}{10}
                \MakeUppercase{CHALMERS UNIVERSITY OF TECHNOLOGY}\\
                Gothenburg, Sweden \TheYear \\
                \textbf{www.chalmers.se}
             \end{covertext}
        };
        
        
        
        \node (spine) at  (17, -3.7){
            \begin{covertext}{8}{11}
                \rotatebox{-90}{
                    \MakeUppercase{\TheAuthor}$\quad\bullet\quad$\TheTitle$\quad\bullet\quad$\TheYear
                }
             \end{covertext}
        };
            
        
    \end{tikzpicture}
    
    % Back side with popular science presentation
    \vspace{3.5cm}
    \noindent\hspace{1.45cm}
    \begin{minipage}[t]{14cm}
        %\color[rgb]{0.22,0.22,0.22}
        \fontfamily{phv}\fontsize{9pt}{13}\selectfont
        \ifx \TheCoverPortrait\undefined
        \else
            \begin{wrapfigure}{l}{5cm}
                \includegraphics[width=4.7cm]{\TheCoverPortrait}
            \end{wrapfigure}
        \fi
        \raggedright
        \input{YourThesis/PopularScienceSummary}
    \end{minipage}
\endgroup
    
\clearpage

==> YourThesis/PopularScienceSummary.tex <==
Abor am qui ipsa poristis ut faccaborum, temporio. Bo. Ic tor sit laboritius incto qui sit, utem eum sae none nis alitas maximperro quae. Lentis et, vel minti corepe dundi ressita sperrum res ea quunt pro cus am sume sernam velluptis earum rest asitatu riorum a sumqui res quam qui autem es simodia parchit, autempe lendiam expelentia dolupta nusam aut optas a quuntinum reria dolo molupis con rercia aniam qui alignima assed experch icipsanimint plitatet vitatenetus ius suntiunt optioria nullum hiciliq uatiusam expel inihit quatquodi ipis prem qui in parum derit erovidem liquunt, consequ ibust, torerrorem sim eatem que dipid ut quam dolorum, idebis ditatia ea earumet occabo. Cum aborro modit ut et occullanihil eum, secus incilli quossimpero doluptas maxim ex este pellit apient eatendi volut apient faccusandest quam doloritiis eum eos et aliquam, accaestibus ex est et ulpa sum fugit lacerna tempori antota. picia nobitas dis abor adias et face lorem pisum dolor inlat. Sim fugitas aliqui blate pelest, quiande rundiam sam delest hicid quid est re simolec aepudist, odi consenis iliquo eum et dit res simi, everae autet prores autem volo mossentest aut ma cus dolum, officatus dolum arum, que pos magnate quo te net litate doluptatur am, officil id utem ni omnimus aliquisFugiandit volupis ex et mint iur se num audanda essimpora sime verci blatias aut officilit, to mosame necati comnihi lluptatemo modi nos modiorem hillore delendenimus audaerumquam quiate et mo minciis estius asitassequis que ommoluptatur sedit alis et eatium que ent dolorit, alicipitibus essum earchitemo cus con consedit officitio ditium rem voluptaectem res etur aut aut prae sum et as volo consequi nosae consentis et que nimusdae idebis nosapis mo dolecti illab is aspere porende nus incideb isimus alit pa es ut voloris evendio que nobis eiciatist aatasped.

==> YourThesis/papers/Letter1/info.tex <==


% only comma separated full names
\paperauthor{\textbf{H. Guo}, B. Makki,  and T. Svensson}
% \paperinfo[short info]{full info}
\paperinfo[\textit{IEEE Wireless Communications Letters}, vol. 9, no. 4, pp. 448-451, Apr. 2020]{
    \textit{IEEE Wireless Communications Letters},\\
	 vol. 9, no. 4, pp. 448-451, Apr. 2020.\\
	\copyright 2020 IEEE
}

% \papertitle[short title]{full title}
\papertitle[Rate Adaptation in Predictor Antenna Systems]{Rate adaptation in predictor antenna systems}

% if you want to use an auto-generated paper summary, please fill in the variable \papersummary{}.
\papersummary{In this paper we...}






==> YourThesis/papers/Letter2/content.tex <==
\begin{abstract}
In this work, we study the performance of predictor antenna (PA) systems using hybrid automatic repeat request (HARQ). Here, the PA system is referred to as a system with two sets of antennas on the roof of a vehicle. In this setup, the PA positioned in the front of the vehicle can be used to predict the channel state information at the transmitter (CSIT) for data transmission to the receive antenna (RA) that is aligned behind the PA. Considering spatial mismatch, due to the vehicle mobility, we derive closed-form expressions for the optimal power allocation and the minimum average power of the PA systems under different outage probability constraints. The results are presented for different types of HARQ protocols and we study the effect of different parameters on the performance of PA systems. As we show, our proposed approximation scheme enables us to analyze PA systems with high accuracy. Moreover, for different vehicle speeds, we show that HARQ-based feedback can reduce the outage-limited power consumption of PA systems by orders of magnitude.
\end{abstract}

\section{Introduction}
Vehicle communication is one of the important use cases in the fifth generation of wireless networks (5G) and beyond \cite{Dang2020what}.  Here, the focus is to provide efficient and reliable connections to cars and public transports, e.g., busses and trains. Channel state information at the transmitter (CSIT), plays an important role in achieving these goals, as it enables advanced closed-loop transmission schemes such as link adaptation, multi-user scheduling, interference coordination and spatial multiplexing schemes.  However,  typical CSIT acquisition systems, which are mostly designed for (semi)static channels, may not work well as the speed of the vehicle increases. This is because, depending on the vehicle speed, the position of the antennas may change quickly and the CSIT becomes inaccurate. 

To overcome this issue, \cite{Sternad2012WCNCWusing} proposes the concept of predictor antenna (PA).  Here, in its standard version, a  PA system is referred to as a setup with two (sets of) antennas on the roof of a vehicle. The PA positioned in the front of the vehicle can be used to improve the CSIT for data transmission to the receive antenna (RA) that is aligned behind the PA. The potential of such setups have been previously shown through experimental tests \cite{Sternad2012WCNCWusing,Dinh2013ICCVEadaptive,Jamaly2014EuCAPanalysis}, and its performance has been analyzed in, e.g., \cite{Guo2019WCLrate,guo2020semilinear,guo2020rate}. 

One of the challenges of the PA setup is spatial mismatch that  causes CSIT for the RA to be partially inaccurate. This occurs if the RA does not reach the same spatial point as the PA, due to, e.g.,  the delay for preparing the data  is not equal to the time that is needed until the RA reaches the same point as the PA \cite{Dinh2013ICCVEadaptive}.  On the other hand, in a typical PA setup the spectrum  is underutilized, and the spectral efficiency could be further improved in case the PA could be used not only for channel  prediction, but also for data transmission. We address these challenges by implementing hybrid automatic repeat request (HARQ)-based protocols in PA systems as follows.

% HARQ is a well-know approach to improve the data transmission reliability and efficiency. The main idea of HARQ is to re-transmit the message that experienced poor channel conditions in order to reduce the outage probability \cite{bh1}\cite{bh2}. Here, we define occurs when the transmitted message cannot be decoded at the receiver. Infinite power is required to achieve zero outage probably for all channel realizations and we replace the strict outage constraint by a more realistic requirement, where a transmission is acceptable, as long as the message can always be decoded by the receiver with probability $\epsilon$. We define $\epsilon$ as a parameter about the system outage tolerance.

% As the PA system includes the feedback link, i.e., from the PA to the BS,  HARQ can be supported by the PA structure. That is, the BS could potentially adjust its transmit rate/power to the RA based on the feedback from the PA. In this way, it is expected that the joint implementation of the PA system and the HARQ scheme can improve the efficiency and reliability of outage-constrained systems. There are limited number of work on deploying HARQ in moving scenarios, i.e., when the channel change quickly over time compared to the feedback delay. Also, \cite{6879267}  studied the performance of INR over double Rayleigh channels, a common model for the fading amplitude of vehicle-to-vehicle communication systems. However,  \cite{6879267} deals with the same channel probability density function (PDF)  for different re-transmission rounds, which has limited contribution to the spatial/temporal variation of the channel in vehicle communications.

In this work, we analyze the outage-limited performance of PA systems using HARQ.   With our proposed approach, the PA is used not only for improving the CSIT in the retransmissions to the RA, but also for data transmission in the initial round. In this way, as we show,  the combination of PA and HARQ protocols makes it possible to improve the spectral efficiency, and adapt the transmission parameters to mitigate the effect of spatial mismatch.

The problem is cast in the form of minimizing the average transmission power subject to an outage probability constraint. Particularly, we  develop approximation techniques to derive closed-form expressions for the instantaneous and average transmission power as well as the optimal power allocation minimizing the outage-limited power consumption. The results are presented for the cases with different repetition time diversity (RTD) and incremental redundancy (INR) HARQ protocols \cite{makki2014green,chaitanya2011outage,djonin2008joint}. Moreover, we study the effect of different parameters such as the antennas separation and the vehicle speed on the system performance. 

As we show through analysis and simulations, the implementation of HARQ as well as power allocation can improve the outage-limited performance of PA systems by orders of magnitude, compared to the cases with no retransmission. For example, consider an outage probability constraint of  $10^{-4}$, initial rate $R=2$ nats-per-channel-use (npcu) and a maximum of two transmission rounds. Then, compared to the cases with no retransmission, our proposed power-adaptive PA-HARQ scheme can reduce the required signal-to-noise ratio (SNR) by  18 dB and 20 dB for the RTD and the INR schemes, respectively.










% \section{Applications in HARQ-based PA Systems}
% In this section, we first introduce the PA concept. Then, we extend the PA setup to the cases using HARQ where the spectrum utilization is improved by using the PA not only for channel estimation but also for initial data transmission. Finally, we use our proposed semi-linear approximation method to optimize the power allocation in outage-constrained conditions. 

% \subsection{Background}
% Vehicle communication is one of the most important use cases in the fifth generation of wireless networks (5G).  Here, the main focus is to provide efficient and reliable connections to cars and public transports, e.g., busses and trains. Channel state information at the transmitter (CSIT), i.e., at the base station (BS), plays an important role in achieving these goals, as it affects, e.g., multiplexing and multi-user scheduling.  However, the typical CSIT acquisition systems, which are mostly designed for (semi)static channels, may not work well for high-speed vehicles. This is because, depending on the vehicle speed, the position of the antennas may change quickly and the channel information becomes inaccurate. 

% To overcome this issue, \cite{Sternad2012WCNCWusing} proposes the concept of PA wherein at least two antennas are deployed on the top of the vehicle. The first antenna, which is the PA,  estimates the channel and sends feedback to the BS. Then, the BS uses the CSIT provided by the PA to communicate with a second antenna, which we refer to as RA, when it arrives at the same position as the PA (see Fig. \ref{system}). In this way, RA can use CSIT acquired from PA and perform different CSIT-based schemes, e.g., multiplexing and multi-user scheduling. The feasibility and efficiency of PA systems have been evaluated through different testbed-based experiments, as reported in, e.g., \cite{Sternad2012WCNCWusing,7962633}.  

% One of the challenges of PA setup is spatial mismatch that if RA does not reach the same spatial point as the PA, due to, e.g.,  the delay for preparing the data (CSI estimation from the PA-BS link) is not equal to the time that we need until the RA reaches the same point as PA, the CSIT for RA may be inaccurate. In this case, we need to design proper schemes to compensate for such mismatch effect \cite{DT2015ITSMmaking}[our letter].  On the other hand, the PA setup may suffer from poor spectral efficiency because the PA is only used for channel estimation and not data transmission.

% [we write this later] Different ways to compensate for such issue have been proposed in \cite{DT2015ITSMmaking}. On the other hand, the BS can potentially adjust the transmission power according to the mismatch problem, if the spatial difference between the PA and the RA in successive time slots is known by the BS. However, to the best of our knowledge, there is no work on power allocation in PA systems.

% [making this paragraph short later]

% Outage-constrained power allocation problem in HARQ system has been studied in e.g, \cite{771147} with perfect CSI assumption, and \cite{6566132} with power allocation schemes aiming at minimizing average power for HARQ systems.  Also, in block fading scenario, \cite{5439316} studied the outage-limited performance of different HARQ protocols.  Moreover, the outage-constrained power optimization for the RTD and INR HARQ protocols were investigated in \cite{5754756}. Finally, \cite{7438859} proposed a linear-programming approach with a buffer cost constraint to solve the power adaptive problem in HARQ systems where the power is adaptive changed based on the received CSI.



% As the PA system includes the feedback link, i.e., from the PA to the BS,  HARQ can be supported by the PA structure in the moving scenarios. That is, the RA could potentially adjust its transmit rate/power based on the feedback from the PA. In this way, it is expected that the joint implementation of the PA system and the HARQ scheme can improve the efficiency and reliability of outage-constrained systems. There are limited number of work on deploying HARQ in moving scenarios, i.e., when the channel change quickly over time compared to the feedback delay. Also, \cite{6879267}  studied the performance of INR over double Rayleigh channels, a common model for the fading amplitude of vehicle-to-vehicle communication systems. However,  \cite{6879267} deals with the same channel probability density function (PDF)  for different re-transmission rounds, which has limited contribution to the spatial/temporal variation of the channel in vehicle communications.


% In this section, we develop the HARQ-based power allocation scheme in the PA systems. The goal is to minimize the transmit power in the presence of imperfect CSIT. We model the mismatch of the PA system as an equivalent non-central Chi-squared channel and perform the power optimization with an outage probability constraint. Particularly, we derive closed-form expressions for the minimum transmit power with/without power allocation. Finally, we evaluate the effect of different parameters such as the antennas distance and the vehicle speed on the outage-limited average transmission power.  Our results, which are of interest for different outage-constrained scenarios of vehicle communications, indicate that HARQ-based power adaptation can effectively compensate for the mismatch issue in PA systems.


\section{Problem Formulation}

Here, we first introduce the basics of PA systems which is followed by our proposed HARQ-based PA setup.

\subsection{Standard PA System}
\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure1.pdf}\\
\caption{Predictor antenna system with mismatch problem.}\label{ARQmodel}
\end{figure}
Figure \ref{ARQmodel} shows the standard PA system with two antennas on the roof of a vehicle. Here, the PA first sends pilots in time $t$. Then, the base station (BS) estimates the PA-BS channel $h_1$ and sends the data in time $t+\delta$ to the RA where  $\delta$ depends on the processing time at the BS. At the same time, the vehicle moves forward $d_\text{m}$ while the antenna separation between the PA and the RA is $d_\text{a}$. Then, considering downlink transmission in the BS-RA link, the  signal received by the RA is
\begin{align}\label{eq_Y}
y = \sqrt{P}h_2 x + z.
\end{align}
Here, $P$ represents the transmit power, $x$ is the input message with unit variance, and $h_2$ is the fading coefficient between the BS and the RA. Also, $z \sim \mathcal{CN}(0,1)$ denotes the independent and identically distributed (IID) complex Gaussian noise added at the receiver.

We represent the probability density function (PDF) and cumulative density function (CDF) of a random variable $A$ by $f_A(\cdot)$ and $F_A(\cdot)$, respectively.  Due to spatial mismatch between the PA and the RA, assuming a semi-static propagation environment, i.e., assuming that the coherence time of the propagation environment is much larger than $\delta$ \footnote{This has been experimentally verified in, e.g., \cite{Jamaly2014EuCAPanalysis}}, $h_2$ and $h_1$ are correlated according to \cite[Eq. 5]{Guo2019WCLrate} 
\begin{align}\label{eq_H}
    h_2 = \sqrt{1-\sigma^2} h_1 + \sigma q,
\end{align}
where $q \sim \mathcal{CN}(0,1)$ which is independent of the known channel value $h_1\sim \mathcal{CN}(0,1)$, and $\sigma$ is a function of the mis-matching distance $d = |d_\text{a}-d_\text{m}|$ \cite[Eq. 4]{Guo2019WCLrate}. Defining $g_1 = |h_1|^2$ and $ g_2 = |h_2|^2$, the CDF $F_{g_2|g_1}$ is given by
\begin{align}\label{eq_cdf}
    F_{g_2|g_1}(x) = 1 - Q_1\left( \sqrt{\frac{2g_1(1-\sigma^2)}{\sigma^2}}, \sqrt{\frac{2x}{\sigma^2}}  \right),
\end{align}
where $Q_1(s,\rho) = \int_{\rho}^{\infty} xe^{-\frac{x^2+s^2}{2}}I_0(xs)\text{d}x$, $s, \rho \ge 0$, is the first-order Marcum $Q$-function. Also, $I_n(x) = (\frac{x}{2})^n \sum_{i=0}^{\infty}\frac{(\frac{x}{2})^{2i} }{i!\Gamma(n+i+1)}$ is the $n$-order modified Bessel function of the first kind, and $\Gamma(z) = \int_0^{\infty} x^{z-1}e^{-x} \mathrm{d}x$ represents the Gamma function. In this way, although parameter adaptation is performed based on perfect CSIT of $h_1$ at time $t$, the spatial mismatch may lead to unsuccessful decoding by the RA  at $t+\delta$.


\subsection{Proposed HARQ-based PA System}
Along with the spatial mismatch problem, the typical PA system  still suffers from poor spectral efficiency, compared to regular multiple-antenna system in static conditions, because the PA is used only for channel estimation. On the other hand, because the PA system includes the PA-BS feedback link,  HARQ can be supported by the PA structure. For this reason, we propose a setup as follows.

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure2.pdf}\\
\caption{Time structure for the proposed PA-HARQ scheme.}\label{fig_timeslot}
\end{figure}

Here, as  seen in Fig. \ref{fig_timeslot}, with no CSIT, at $t_1$ the BS sends pilots as well as the encoded data with certain initial rate $R$ and power $P_1$ to the PA. At $t_2$, the PA estimates the channel $h_1$ from the received pilots. At the same time, the PA tries to decode the signal. If the message is correctly decoded, i.e., $R\leq \log(1+g_1P_1)$,  an acknowledgment (ACK) is fed back to the BS at $t_3$, and the data transmission stops. Otherwise, the PA sends both a negative acknowledgment (NACK) and high accuracy quantized CSI feedback about $h_1$. The number of quantization bits are large enough such that we can assume the BS to have perfect CSIT of $h_1$ (see \cite{guo2020semilinear} for the effect of imperfect CSIT on the performance of PA systems). With NACK, in the second transmission round at time $t_4$, the BS  transmits the message to the RA with power $P_2$  which is a function of the instantaneous channel quality $g_1$. The outage occurs if the RA cannot decode the message at the end of the second round. 

\section{Analytical Results}
Let $\epsilon$ be the outage probability constraint. Here, we present the results for the cases with RTD and INR HARQ protocols. With an RTD protocol, the same signal (with possibly different power) is sent in each retransmission round, and the receiver performs maximum ratio combining of all received copies of the signal. With INR, on the other hand, new redundancy bits are sent in the retransmissions, and the receiver decodes the message by combining all received signals \cite{makki2014green,chaitanya2011outage,djonin2008joint}.

Considering Rayleigh fading conditions with $f_{g_1}(x) =  e^{- x}$, the outage probability at the end of Round 1 is given by
\begin{align}\label{eq_pout}
&\text{Pr}(\text{Outage, Round 1}) = \text{Pr}\left\{R\leq \log(1+g_1P_1)\right\}\nonumber\\
&~~ = \text{Pr}\left\{g_1\leq \frac{e^{R}-1}{P_1}\right\}
 = 1-e^{ -\frac{\theta}{P_1}}, 
\end{align}
where $\theta = e^{R}-1$. Then, using the results of, e.g.,  \cite[Eq. 7, 18]{makki2014green} on the outage probability of the RTD- and INR-based HARQ protocols, the power allocation problem for the proposed HARQ-based PA system can be stated as
\begin{equation}
\label{eq_optproblem}
\begin{aligned}
\min_{P_1,P_2} \quad & \mathbb{E}_{g_1}\left[P_\text{tot}|g_1\right] \\
\textrm{s.t.} \quad &  P_1, P_2 > 0,\\
&P_\text{tot}|g_1 = \left[P_1 + P_2(g_1) \times \mathcal{I}\left\{g_1 \le \frac{\theta}{P_1}\right\}\right],
\end{aligned}
\end{equation}
with
\begin{align}\label{eq_optproblemrtd}
F_{g_2|g_1}\left\{\frac{\theta-g_1P_1}{P_2(g_1)}    \right\} = \epsilon, \quad\text{for RTD}
\end{align}
\begin{align}\label{eq_optprobleminr}
F_{g_2|g_1}\left\{\frac{e^{R-\log(1+g_1P_1)}-1}{P_2(g_1)}    \right\} = \epsilon, \quad\text{for INR}. 
\end{align}
Here, $P_\text{tot}|g_1$ is the total instantaneous transmission power for two transmission rounds (i.e., one retransmission) with given $g_1$, and we define $\Bar{P} \doteq \mathbb{E}_{g_1}\left[P_\text{tot}|g_1\right]$ as the expected power, averaged over $g_1$. Moreover, $\mathcal{I}(x)=1$ if $x>0$ and $\mathcal{I}(x)=0$ if $x \le 0$. Also, $\mathbb{E}_{g_1}[\cdot]$ represents the expectation operator over $g_1$. Here, we ignore the peak power constraint and assume that the BS is capable of transmitting  sufficiently high power. Finally, (\ref{eq_optproblem})-(\ref{eq_optprobleminr}) come from the fact that, with our proposed scheme, $P_1$ is fixed and optimized with no CSIT at the BS and based on average system performance. On the other hand, $P_2$ is adapted continuously based on the predicted CSIT.


Using (\ref{eq_optproblem}), the required power in Round 2 is given by
\begin{equation}
\label{eq_PRTDe}
    P_2(g_1) = \frac{\theta-g_1P_1}{F_{g_2|g_1}^{-1}(\epsilon)},
\end{equation}
for the RTD, and
\begin{equation}
\label{eq_PINRe}
    P_2(g_1) = \frac{e^{R-\log(1+g_1P_1)}-1}{F_{g_2|g_1}^{-1}(\epsilon)},
\end{equation}
for the INR, where $F_{g_2|g_1}^{-1}(\cdot)$ is the inverse of the CDF given in (\ref{eq_cdf}). Note that, $F_{g_2|g_1}^{-1}(\cdot)$ is a complex function of $g_1$ and, consequently, it is not possible to express $P_2$ in closed-form. For this reason, one can use   \cite[Eq. 2, 7]{6414576}
\begin{align}
    Q_1 (s, \rho) &\simeq e^{\left(-e^{\mathcal{I}(s)}\rho^{\mathcal{J}(s)}\right)}, \nonumber\\
    \mathcal{I}(s)& = -0.840+0.327s-0.740s^2+0.083s^3-0.004s^4,\nonumber\\
    \mathcal{J}(s)& = 2.174-0.592s+0.593s^2-0.092s^3+0.005s^4,
\end{align}
to approximate $F_{g_2|g_1}$ and consequently $F_{g_2|g_1}^{-1}(\epsilon)$. In this way, (\ref{eq_PRTDe}) and (\ref{eq_PINRe}) can be approximated as
\begin{equation}
\label{eq_PRTDa}
    P_2(g_1) = \Omega\left(\theta-g_1P_1\right),
\end{equation}
for the RTD, and
\begin{equation}
\label{eq_PINRa}
   P_2(g_1) = \Omega\left(e^{R-\log(1+g_1P_1)}-1\right),
\end{equation}
for the INR, where
\begin{equation}\label{eq_omega}
    \Omega (g_1) = \frac{2}{\sigma^2}\left(\frac{\log(1-\epsilon)}{-e^{\mathcal{I}\left(\sqrt{\frac{2g_1(1-\sigma^2)}{\sigma^2}}\right)}}\right)^{-\frac{2}{\mathcal{J}\left(\sqrt{\frac{2g_1(1-\sigma^2)}{\sigma^2}}\right)}}.
\end{equation}



In this way, for different HARQ protocols, we can express the  instantaneous transmission power of Round 2, for every given $g_1$ in closed-form. Then, the  power allocation problem (\ref{eq_optproblem}) can be solved numerically. However, (\ref{eq_omega}) is still complicated and it is not possible to solve (\ref{eq_optproblem}) in closed-form. For this reason, we propose an approximation scheme to solve (\ref{eq_optproblem}) as follows.




Let us initially concentrate on the RTD protocol. Then,  combining (\ref{eq_optproblem}) and (\ref{eq_PRTDe}), the expected total transmission power  is given by
\begin{align}\label{eq_barP}
    \Bar{P}_\text{RTD} = P_1 + \int_0^{\theta/P_1} e^{- x}P_2\text{d}x= P_1 + \int_0^{\theta/P_1} e^{- x}\frac{\theta-x P_1}{F_{g_2|x}^{-1}(\epsilon)}\text{d}x.
\end{align}
Then, Theorem \ref{theorem1} derives the minimum required power  in Round 1 and the average total power consumption as follows. 



\begin{theorem}\label{theorem1}
With RTD and given outage constraint $\epsilon$, the minimum required power in Round 1 and the average total power are given by (\ref{eq_P1}) and (\ref{eq_666666}), respectively. 
\end{theorem}
\begin{proof}
Plugging (\ref{eq_cdf}) into (\ref{eq_optproblemrtd}), we have
\begin{align}
    1-Q_1\left(\sqrt{\frac{2g_1(1-\sigma^2)}{\sigma^2}},\sqrt{\frac{2(\theta-g_1P_1)}{\sigma^2 P_2}}\right) = \epsilon.
\end{align}
By using the approximation \cite[Eq. 17]{Azari2018TCultra} for moderate/large $\sigma$, i.e., if $1-Q_1(s,\rho) = 1-\epsilon$, then $\rho = Q_1^{-1}(s, 1-\epsilon) \simeq \sqrt{-2\log(1-\epsilon)}e^{\frac{s^2}{4}}$, we can obtain 
\begin{align}
    \sqrt{\frac{2(\theta-g_1P_1)}{\sigma^2 P_2}}\simeq \sqrt{-2\log(1-\epsilon)}e^{\frac{g_1(1-\sigma^2)}{2\sigma^2}}.
\end{align}
In this way, $P_2$ in (\ref{eq_barP}) is approximated by
\begin{align}
    P_2 \simeq (\theta - g_1P_1)\frac{e^{-\frac{g_1(1-\sigma^2)}{\sigma^2}}}{-\sigma^2\log(1-\epsilon)},
\end{align}
and considering RTD, (\ref{eq_barP}) can be rewritten as
\begin{align}\label{eq_Papprobeforederrivative}
    \Bar{P} = P_1 + \int_0^{\theta/P_1} e^{- x}(\theta - xP_1)\frac{e^{-\frac{x(1-\sigma^2)}{\sigma^2}}}{-\sigma^2\log(1-\epsilon)}\text{d}x \overset{(a)}{=} P_1 + \frac{c}{m^2}\left(P_1 e^{-\frac{m\theta}{P_1}}-P_1 + m\theta\right),
\end{align}
where, in (a) we set $m = 1 + \frac{1-\sigma^2}{\sigma^2}$ and $c = \frac{-1}{\sigma^2\log(1-\epsilon)}$ for simplicity. Then, setting the derivative of (\ref{eq_Papprobeforederrivative})  with respect to $P_1$ equal to zero, the minimum $P_1$ for the minimum total power can be found as
\begin{align}
  \label{eq_P1}
    \hat{P}_{1,\text{RTD}} & = \operatorname*{arg}_{P_1 > 0} \Bigg\{ 1 +  \frac{c}{m^2}e^{-\frac{\theta m}{P_1}}\left(\frac{m\theta}{P_1}+1\right) - \frac{c}{m^2} = 0\Bigg\}\nonumber\\
    & = \operatorname*{arg}_{P_1 > 0} \left\{e^{-\frac{\theta m}{P_1}}\left(\frac{m\theta}{P_1}+1\right) = 1-\frac{m^2}{c} \right\}\nonumber\\
    & \overset{(b)}= \frac{-m\theta}{\mathcal{W}_{-1}\left(\frac{m^2}{ce}-\frac{1}{e}\right)+1}.
\end{align}
Here, $(b)$ is obtained by the definition of the Lambert W function $xe^x = y \Leftrightarrow x = \mathcal{W}(y)$ \cite{corless1996lambertw}. Also, because $\frac{m^2}{ce}-\frac{1}{e}<0$, we use the $\mathcal{W}_{-1}(\cdot)$ branch \cite[Eq. 16]{veberic2010having}. Then, plugging (\ref{eq_P1}) into (\ref{eq_Papprobeforederrivative}), we obtain the  minimum total transmission power as
\begin{align}\label{eq_666666}
    \hat{\Bar{P}}_{\text{RTD}} =\hat{P}_{1,\text{RTD}} + \frac{c}{m^2}\left(\hat{P}_{1,\text{RTD}} e^{-\frac{m\theta}{\hat{P}_{1,\text{RTD}}}}-\hat{P}_{1,\text{RTD}} + m\theta\right).
\end{align}
\end{proof}


\subsection{On the Effect of CSI Feedback/Power Allocation}
In this part, we consider the case without exploiting CSIT, i.e., we consider the typical HARQ schemes where CSI feedback is not sent along with NACK, and we do not perform power adaptation.  Here, the outage probability,  for the RTD and the INR  are given by
\begin{align}\label{eq_PrRTD}
    \zeta_{\text{RTD}} = \text{Pr}\left\{\log\left(1+\left(g_1+g_2\right)P\right)<R ~\&~ g_1<\frac{\theta}{P}  \right\},
\end{align}
\begin{align}\label{eq_PrINR}
\begin{split}
    \zeta_{\text{INR}}=\text{Pr}\left\{\log\left(1+g_1P\right) + \log\left(1+g_2P\right)<R ~\&~ g_1<\frac{\theta}{P}\right\}.
\end{split}
\end{align}
Note that as opposed to (\ref{eq_optproblem})-(\ref{eq_optprobleminr}), where the transmit power in Round 2 is set instantaneously such that, for every given $g_1$, the instantaneous outage constraint is satisfied, (\ref{eq_PrRTD}) and (\ref{eq_PrINR}) are based on the average outage probability, i.e., a less constrained condition. Also, in both protocols, the total average power is given by
\begin{align}\label{eq_barpbench}
    \Bar{P} = P + P\cdot\text{Pr}\{\log\left(1+g_1P\right)<R\}=P(2-e^{-\frac{\theta}{P}}).
\end{align}
\begin{theorem}\label{theorem2}
Without CSIT feedback/power allocation, the outage probability of the RTD-based PA-HARQ scheme is given by (\ref{eq_RTDnopa}).
\end{theorem}
\begin{proof}
Using (\ref{eq_PrRTD}), we have
\begin{align}
    \zeta_{\text{RTD}}= \text{Pr}\left\{g_2< \frac{\theta}{P}-g_1  ~\&~ g_1 < \frac{\theta}{P} \right\}=\int_{0}^{\frac{\theta}{P}} e^{- x} F_{g_2|x}\left(\frac{\theta}{P}-x\right) \text{d}x. \label{eq_nocloseform}
\end{align}
Considering (\ref{eq_cdf}), there is no closed-form solution for (\ref{eq_nocloseform}).  For this reason, we use the  approximation \cite[Eq. 14]{andras2011generalized} 
\begin{align}
    Q_1\left( s, \rho  \right) \simeq  1 - \left( 1 + \frac{s^2}{2} \right)e^{-\frac{s^2}{2}} +
    \left( 1 + \frac{s^2}{2} + \frac{s^2\rho^2}{4} \right)e^{-\frac{s^2+\rho^2}{2}},
\end{align}
which simplifies (\ref{eq_nocloseform}) to 
% \begin{align}\label{eq_RTDnopa}
%     \zeta_{\text{RTD}} &\simeq \int_{0}^{\frac{\theta}{P}}\left(1+\frac{ax}{2}\right)e^{-\frac{ax}{2}-x} \text{d}x -\nonumber\\ 
%     & \int_{0}^{\frac{\theta}{P}} \left(1+\frac{ax}{2}+\frac{a^2\frac{\theta}{P} x-a^2x^2}{4}\right)e^{-\frac{a\frac{\theta}{P}}{2}-x}\text{d}x\nonumber\\
%     & = \Bigg( (16a +16)e^{\frac{a\frac{\theta}{P}}{2}+\frac{\theta}{P}} +\bigg(\left(-a^4-4a^3-4a^2\right)\frac{\theta}{P}+\nonumber\\
%     &     2a^4+6a^3-4a^2-24a-16\bigg)e^{\frac{\theta}{P}} +(-a^4-2a^3)\frac{\theta}{P}-\nonumber\\ &2a^4-6a^3+4a^2+8a \Bigg)\frac{e^{-\frac{a\frac{\theta}{P}}{2}-\frac{\theta}{P}}}{4a^2+16a+16}.
% \end{align}
\begin{align}\label{eq_RTDnopa}
    &\zeta_{\text{RTD}} \simeq 
    -\frac{e^{-\frac{\theta}{P\sigma^2}}}{6\sigma^4}\Bigg(\left(6\sigma^8-12\sigma^6\right)e^{\frac{\theta}{P\sigma^2}}+12\sigma^6+\nonumber\\&\left(3\sigma^2-3\sigma^4\right)\frac{\theta^2}{P^2}+\left(12\sigma^4-6\sigma^6\right)\frac{\theta}{P}+\left(1-\sigma^2\right)\frac{\theta^3}{P^3}-6\sigma^8\Bigg)
\end{align}
% -\dfrac{\mathrm{e}^{-\frac{{\theta}}{a^2}}\left(\left(6a^8-12a^6\right)\mathrm{e}^\frac{{\theta}}{a^2}+\left(1-a^2\right){\theta}^3+\left(3a^2-3a^4\right){\theta}^2+\left(12a^4-6a^6\right){\theta}-6a^8+12a^6\right)}{6a^4}

% \begin{align}
%     (e^{-(a*\theta)/2-\theta}*((16*a+16)*e^{(a*\theta)/2+\theta}+((-a^4-4*a^3-4*a^2)*\theta+2*a^4+6*a^3-4*a^2-24*a-16)*e^{\theta}+(-a^4-2*a^3)*\theta-2*a^4-6*a^3+4*a^2+8*a))/(4*a^2+16*a+16)
% \end{align}
% \begin{equation}\label{eq_lemma2list}
% \left\{
%              \begin{array}{ll}
%              a   = &\frac{2}{\sigma^2},  \\
%              l_1 = & (16a + 16)e^{\frac{a\frac{\theta}{P}}{2}+\frac{\theta}{P}},\\
%              l_2 = & \left(\left(-a^4-4a^3-4a^2\right)\frac{\theta}{P}+ \right. \\  &  \left. 2a^4+6a^3-4a^2-24a-16\right)e^{\frac{\theta}{P}},\\
%              l_3 = & (-a^4-2a^3)\frac{\theta}{P}-2a^4-6a^3+4a^2+8a.
%              \end{array}
% \right.
% \end{equation}
\end{proof}

\subsection{On the Effect of Introducing INR}
For the INR scheme, by using Jensen's inequality and the concavity of the logarithm function \cite[Eq. 30]{makki2016TWCRFFSO}
\begin{align}\label{eq_jensen}
   \frac{1}{n}\sum_{i=1}^{n} \log (1+x_i)\leq\log\left(1+\frac{1}{n}\sum_{i=1}^{n}x_i\right),
\end{align}
the closed-form expressions for the minimum required power, the average total power, as well as outage probability without power allocation are given by the following Corollary.
\begin{corollary}
With INR, the minimum required power in Round 1 and the average total power are given by (\ref{eq_P1inr}) and (\ref{eq_barpinr}), respectively.  Also, without power allocation, the outage probability of the INR-based scheme is given by (\ref{eq_INRnopa}).
\end{corollary}
\begin{proof}
Using (\ref{eq_optprobleminr}), the Jensen's inequality (\ref{eq_jensen}) and defining $\theta_1 =2\left(e^{\frac{R}{2}}-1\right)$, (\ref{eq_PINRe}) can be approximated by
\begin{align}
     P_2(g_1) \simeq \frac{\theta_1 - g_1P_1}{F_{g_2|g_1}^{-1}(\epsilon)},
\end{align}
and, following the same steps as in Theorem \ref{theorem1}, we obtain the minimum required $P_1$ for the minimum total power in the INR scheme as
\begin{align}
  \label{eq_P1inr}
    \hat{P}_{1,\text{INR}}= \frac{-m\theta_1}{\mathcal{W}_{-1}\left(\frac{m^2}{ce}-\frac{1}{e}\right)+1}.
\end{align}
Also, the  minimum total  power can be calculated by
\begin{align}\label{eq_barpinr}
    \hat{\Bar{P}}_{\text{INR}} =\hat{P}_{1,\text{INR}} + \frac{c}{m^2}\left(\hat{P}_{1,\text{INR}} e^{-\frac{m\theta_1}{\hat{P}_{1,\text{INR}}}}-\hat{P}_{1,\text{INR}} + m\theta_1\right).
\end{align}

Finally, (\ref{eq_PrINR}) can be further derived by
\begin{align}
    \zeta_{\text{INR}} &= \text{Pr}\left\{  g_2< \frac{e^{R-\log(1+g_1)}-1}{P}~\&~ g_1 < \frac{\theta}{P} \right\}\nonumber\\
    % &= \frac{1}{1-e^{-\frac{\theta}{P}}}\int_{0}^{\frac{\theta}{P}} e^{- x} F_{g_2|x}\left(\frac{e^{R-\log(1+x)}-1}{P}\right) \text{d}x\nonumber\\
    &\overset{(c)}{\simeq}\int_{0}^{\frac{\theta}{P}} e^{- x} F_{g_2|x}\left(\frac{\theta_1}{P}-x\right) \text{d}x,
\end{align}
with $(c)$ using Jensen's inequality. Then, following the same steps as in Theorem \ref{theorem2}, the outage probability is found as 
\begin{align}\label{eq_INRnopa}
    \zeta_{\text{INR}} \simeq \zeta_{\text{RTD}}(\theta = \theta_1).
\end{align}
\end{proof}

Finally, as a benchmark, we consider the case with no retransmission where the outage probability is given by $1-e^{-\frac{\theta}{P}}$. In this case, the required outage-constrained power without retransmission is given by $P \geq \frac{1-e^{R}}{\log(1-\epsilon)}$.

% \subsection{On the Effect of PA System}
% For the case without PA, i.e., with no retransmission,  the outage probability can be written as

% \begin{align}\label{eq_nocsinopa}
%     \zeta_{\text{no-CSI}} = \int_0^{\frac{\theta}{P}} e^{- x} \text{d}x = 1-e^{-\frac{\theta}{P}}.
% \end{align}

% Here, results obtained from Lemma 2, Corollary 2 and (\ref{eq_nocsinopa}) provide the benchmark for the HARQ-based PA system terms of outage probability. Also, the transmission power is set according to
% \begin{align}\label{eq_nofeedback}
% &\text{Pr}\left\{ \log(1+g_1P_1) < R \right\} \leq \epsilon\nonumber\\
%   & \Rightarrow P_1 \geq \frac{1-e^{R}}{\log(1-\epsilon)}.
% \end{align}
% This provides the lower bound of the system performance.









\section{{Simulation Results}}

In the simulations, we set $ \delta$ = 5 ms, $f_\text{c}$ = 2.68 GHz, and $d_\text{a} = 1.5\lambda$. Each point in the figures is obtained by averaging the system performance over $1\times10^5$ channel realizations. 

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure3.pdf}\\
\caption{Minimum required power under various outage constraints for the RTD and the INR, $\sigma = 0.8$, $R = 0.5, 2$ npcu.}\label{figure3}
\end{figure}

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure4.pdf}\\
\caption{Minimum required power without optimized power allocation (\ref{eq_barpbench}) under various outage probabilities, $\sigma$ = 0.8, $R$ = 1, 5 npcu.}\label{figure4}
\end{figure}


\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure5.pdf}\\
\caption{Minimum required power for the RTD and the INR with given outage constraint, for different speed $v$. $R = 3$ npcu, $\epsilon = 10^{-3}$.}\label{figure5}
\end{figure}

Figure \ref{figure3} shows the results of the power allocation problem (\ref{eq_optproblem}) for both the RTD and the INR with different initial rates $R = 0.5, 2$ npcu, $\sigma = 0.8$, and different outage probability constraints $\epsilon$. Here, the simulation results are obtained from  solving the optimization problem (\ref{eq_optproblem}) numerically, while the approximation results for the RTD and the INR are obtained by Theorem \ref{theorem1} and Corollary 1, respectively.  In Fig. \ref{figure4}, we plot the outage probability using the  RTD and the INR  without power optimization. Here, we set $\sigma = 0.8$, and the initial rate $R = 1, 5$ npcu. The simulation results are obtained by (\ref{eq_PrRTD}) and (\ref{eq_PrINR}), while the analytical approximations are obtained from Theorem \ref{theorem2} for the RTD and Corollary 1 for the INR. Finally, in Fig. \ref{figure5},  we study the minimum required transmission power for different speeds $v$. Here, manipulating $v$ is  equivalent to changing the level of spatial correlation for given values of $\delta$, $f_\text{c}$ and $d_\text{a}$ (see \cite{guo2020semilinear} for the detailed effect of the vehicle speed on the spatial correlation). Also, we study the effect of different values of $d_\text{a}$ on the system performance.   According to the figures, we can conclude the following:






%=============
%Fig: benchmark
%=============



%=============
%Fig: numerical solution-speed v
%=============









%=============
%Fig: numerical solution-outage constraint
%=============








\begin{itemize}
    \item The approximation schemes of Theorem \ref{theorem1} and Corollary 1 are  tight for a broad range of values of initial rate $R$, speed $v$,  as well as $\epsilon$ (Figs. \ref{figure3} and \ref{figure5}). Thus, for different parameter settings, the outage-constrained power allocation for the RTD and the INR can be well determined by Theorem \ref{theorem1} and Corollary 1. 
    \item Also, the approximation scheme of Theorem \ref{theorem2} is tight for a broad range of values of average power (\ref{eq_barpbench}) as well as initial rate $R$ (Fig. \ref{figure4}). Thus, for different parameter settings, the outage probability for the proposed PA-HARQ scheme without power allocation, can be well determined by Theorem \ref{theorem2} and Corollary 1.
    \item With the deployment of the PA and power allocation, remarkable power gain is achieved especially at low outage probabilities  (Figs. \ref{figure3} and \ref{figure5}). Moreover,  as also indicated in, e.g.,  \cite{makki2014green}, INR outperforms RTD, in terms of outage-limited average power. However, the difference between the performance of these protocols decreases as the data rate or $\sigma$ decreases (Figs. \ref{figure3} and \ref{figure5}).
    \item Figures \ref{figure3}-\ref{figure5} emphasize the efficiency of HARQ as well as adaptive power allocation in the PA system. From Figs. \ref{figure3}-\ref{figure4}, we can see that with the PA-HARQ setup, with different instantaneous- and average-outage constrained power allocation cases, we can obtain considerable performance improvements compared to the case with no retransmission.  For instance, with $\epsilon=10^{-4}$ and $R = 2$ npcu, the RTD- and INR-based PA-HARQ can reduce the required power, compared to no retransmission case, by 18 and 20 dB, respectively. Then, as can be seen from Fig.  \ref{figure5}, the effect of power-optimized PA-HARQ increases with $\sigma$. This is because the larger $\sigma$ provides better spatial diversity of the channel, which can improve the performance with retransmissions. For the peaks in Fig. \ref{figure5}, the channel for the retransmission has the largest correlation with the one in the first round, which leads to the smallest power gain. Moreover, when the antenna separation $d_\text{a}$ decreases, the speed where the power gain is minimum, also decreases, due to the reduction of the mismatch distance $d$.
\end{itemize}



\section{Conclusion}
We studied the PA-HARQ system with the spatial mismatch problem, in the context of outage-constrained power allocation. We derived  closed-form expressions for the minimum instantaneous and  total transmit power. The approximations are tight for a broad range of system configurations. Also, the  results show that, while PA-assisted adaptive power adaptation leads to considerable performance improvements, the total transmission power and the outage probability are remarkably affected by the spatial mismatch.




% use section* for acknowledgment
%  \section*{Acknowledgment}
% % % The research leading to these results received funding from the European Commission H2020 programme under grant agreement $n^{\circ}$671650 (5G PPP mmMAGIC project), and from the Swedish Governmental Agency for Innovation Systems (VINNOVA) within the VINN Excellence Center Chase.

% This work has been partly performed in the framework of the H2020 project 5GCAR co-funded by the EU and has also been supported in part by VINNOVA (Swedish Government Agency for Innovation Systems) within the VINN Excellence Center ChaseOn. The authors would like to acknowledge the contributions of their colleagues.




==> YourThesis/papers/Letter2/content1.tex <==
\begin{abstract}
In this work, we study the performance of predictor antenna (PA) systems using hybrid automatic repeat request (HARQ). Here, the PA system is referred to as a system with two sets of antennas on the roof of a vehicle. In this setup, the PA positioned in the front of the vehicle can be used to predict the channel state information at the transmitter (CSIT) for data transmission to the receive antenna (RA) that is aligned behind the PA. Considering spatial mismatch, due to the vehicle mobility, we derive closed-form expressions for the optimal power allocation and the minimum average power of the PA systems under different outage probability constraints. The results are presented for different types of HARQ protocols and we study the effect of different parameters on the performance of PA systems. As we show, our proposed approximation scheme enables us to analyze PA systems with high accuracy. Moreover, for different vehicle speeds, we show that HARQ-based feedback can reduce the outage-limited power consumption of PA systems by orders of magnitude.
\end{abstract}


\section{Introduction}
Vehicle communication is one of the important use cases in the fifth generation of wireless networks (5G) and beyond \cite{Dang2020what}.  Here, the focus is to provide efficient and reliable connections to cars and public transports, e.g., busses and trains. Channel state information at the transmitter (CSIT), plays an important role in achieving these goals, as it enables advanced closed-loop transmission schemes such as link adaptation, multi-user scheduling, interference coordination and spatial multiplexing schemes.  However,  typical CSIT acquisition systems, which are mostly designed for (semi)static channels, may not work well as the speed of the vehicle increases. This is because, depending on the vehicle speed, the position of the antennas may change quickly and the CSIT becomes inaccurate. 

To overcome this issue, \cite{Sternad2012WCNCWusing} proposes the concept of predictor antenna (PA).  Here, in its standard version (it can be generalize to more antennas) a  PA system is referred to as a setup with two (sets of) antennas on the roof of a vehicle. The PA positioned in the front of the vehicle can be used to improve the CSIT for data transmission to the receive antenna (RA) that is aligned behind the PA. The feasibility of such setups have been previously shown through experimental tests \cite{Sternad2012WCNCWusing,DT2015ITSMmaking}, and its performance has been analyzed in, e.g., \cite{Jamaly2019IETeffects,Guo2019WCLrate,guo2020semilinear}. 

One of the challenges of the PA setup is spatial mismatch that  causes CSIT for the RA to be inaccurate. This occurs if the RA does not reach the same spatial point as the PA, due to, e.g.,  the delay for preparing the data  is not equal to the time that is needed until the RA reaches the same point as the PA.  On the other hand, in a typical PA setup the antenna  is under utilized, and the spectral efficiency could be further improved in case the PA could be used not only used for channel  prediction, but also for data transmission. We address these challenges by implementing hybrid automatic repeat request (HARQ)-based protocols in PA systems as follows.

% HARQ is a well-know approach to improve the data transmission reliability and efficiency. The main idea of HARQ is to re-transmit the message that experienced poor channel conditions in order to reduce the outage probability \cite{bh1}\cite{bh2}. Here, we define occurs when the transmitted message cannot be decoded at the receiver. Infinite power is required to achieve zero outage probably for all channel realizations and we replace the strict outage constraint by a more realistic requirement, where a transmission is acceptable, as long as the message can always be decoded by the receiver with probability $\epsilon$. We define $\epsilon$ as a parameter about the system outage tolerance.

% As the PA system includes the feedback link, i.e., from the PA to the BS,  HARQ can be supported by the PA structure. That is, the BS could potentially adjust its transmit rate/power to the RA based on the feedback from the PA. In this way, it is expected that the joint implementation of the PA system and the HARQ scheme can improve the efficiency and reliability of outage-constrained systems. There are limited number of work on deploying HARQ in moving scenarios, i.e., when the channel change quickly over time compared to the feedback delay. Also, \cite{6879267}  studied the performance of INR over double Rayleigh channels, a common model for the fading amplitude of vehicle-to-vehicle communication systems. However,  \cite{6879267} deals with the same channel probability density function (PDF)  for different re-transmission rounds, which has limited contribution to the spatial/temporal variation of the channel in vehicle communications.

In this work, we analyze the outage-limited performance of PA systems using HARQ.   With our proposed approach, the PA is used not only for improving the CSIT in the retransmissions to the RA, but also for data transmission in the initial round. In this way, as we show,  the combination of PA and HARQ protocols makes it possible to improve the spectral efficiency, and adapt the transmission parameters to mitigate the effect of spatial mismatch.

The problem is cast in the form of minimizing the average transmission power subject to an outage probability constraint. Particularly, we  develop approximation techniques to derive closed-form expressions for the instantaneous and average transmission power as well as the optimal power allocation minimizing the outage-limited power consumption. The results are presented for the cases with different repetition time diversity (RTD) and incremental redundancy (INR) HARQ protocols \cite{makki2014green,chaitanya2011outage,djonin2008joint}. Moreover, we study the effect of different parameters such as the antennas separation and the vehicle speed on the system performance. 

As we show through analysis and simulations, the implementation of HARQ as well as power allocation can improve the outage-limited performance of PA systems by orders of magnitude, compared to the cases with no retransmission. For example, consider an outage probability constraint of  $10^{-5}$, initial rate $R=4$ nats-per-channel-use (npcu) and a maximum of two transmission rounds. Then, compared to the cases with no retransmission, our proposed power-adaptive PA-HARQ scheme can reduce the required signal-to-noise ratio (SNR) by  25 dB and 30 dB for the RTD and the INR schemes, respectively.










% \section{Applications in HARQ-based PA Systems}
% In this section, we first introduce the PA concept. Then, we extend the PA setup to the cases using HARQ where the spectrum utilization is improved by using the PA not only for channel estimation but also for initial data transmission. Finally, we use our proposed semi-linear approximation method to optimize the power allocation in outage-constrained conditions. 

% \subsection{Background}
% Vehicle communication is one of the most important use cases in the fifth generation of wireless networks (5G).  Here, the main focus is to provide efficient and reliable connections to cars and public transports, e.g., busses and trains. Channel state information at the transmitter (CSIT), i.e., at the base station (BS), plays an important role in achieving these goals, as it affects, e.g., multiplexing and multi-user scheduling.  However, the typical CSIT acquisition systems, which are mostly designed for (semi)static channels, may not work well for high-speed vehicles. This is because, depending on the vehicle speed, the position of the antennas may change quickly and the channel information becomes inaccurate. 

% To overcome this issue, \cite{Sternad2012WCNCWusing} proposes the concept of PA wherein at least two antennas are deployed on the top of the vehicle. The first antenna, which is the PA,  estimates the channel and sends feedback to the BS. Then, the BS uses the CSIT provided by the PA to communicate with a second antenna, which we refer to as RA, when it arrives at the same position as the PA (see Fig. \ref{system}). In this way, RA can use CSIT acquired from PA and perform different CSIT-based schemes, e.g., multiplexing and multi-user scheduling. The feasibility and efficiency of PA systems have been evaluated through different testbed-based experiments, as reported in, e.g., \cite{Sternad2012WCNCWusing,7962633}.  

% One of the challenges of PA setup is spatial mismatch that if RA does not reach the same spatial point as the PA, due to, e.g.,  the delay for preparing the data (CSI estimation from the PA-BS link) is not equal to the time that we need until the RA reaches the same point as PA, the CSIT for RA may be inaccurate. In this case, we need to design proper schemes to compensate for such mismatching effect \cite{DT2015ITSMmaking}[our letter].  On the other hand, the PA setup may suffer from poor spectral efficiency because the PA is only used for channel estimation and not data transmission.

% [we write this later] Different ways to compensate for such issue have been proposed in \cite{DT2015ITSMmaking}. On the other hand, the BS can potentially adjust the transmission power according to the mismatching problem, if the spatial difference between the PA and the RA in successive time slots is known by the BS. However, to the best of our knowledge, there is no work on power allocation in PA systems.

% [making this paragraph short later]

% Outage-constrained power allocation problem in HARQ system has been studied in e.g, \cite{771147} with perfect CSI assumption, and \cite{makki2014green} with power allocation schemes aiming at minimizing average power for HARQ systems.  Also, in block fading scenario, \cite{5439316} studied the outage-limited performance of different HARQ protocols.  Moreover, the outage-constrained power optimization for the RTD and INR HARQ protocols were investigated in \cite{chaitanya2011outage}. Finally, \cite{7438859} proposed a linear-programming approach with a buffer cost constraint to solve the power adaptive problem in HARQ systems where the power is adaptive changed based on the received CSI.



% As the PA system includes the feedback link, i.e., from the PA to the BS,  HARQ can be supported by the PA structure in the moving scenarios. That is, the RA could potentially adjust its transmit rate/power based on the feedback from the PA. In this way, it is expected that the joint implementation of the PA system and the HARQ scheme can improve the efficiency and reliability of outage-constrained systems. There are limited number of work on deploying HARQ in moving scenarios, i.e., when the channel change quickly over time compared to the feedback delay. Also, \cite{6879267}  studied the performance of INR over double Rayleigh channels, a common model for the fading amplitude of vehicle-to-vehicle communication systems. However,  \cite{6879267} deals with the same channel probability density function (PDF)  for different re-transmission rounds, which has limited contribution to the spatial/temporal variation of the channel in vehicle communications.


% In this section, we develop the HARQ-based power allocation scheme in the PA systems. The goal is to minimize the transmit power in the presence of imperfect CSIT. We model the mismatching of the PA system as an equivalent non-central Chi-squared channel and perform the power optimization with an outage probability constraint. Particularly, we derive closed-form expressions for the minimum transmit power with/without power allocation. Finally, we evaluate the effect of different parameters such as the antennas distance and the vehicle speed on the outage-limited average transmission power.  Our results, which are of interest for different outage-constrained scenarios of vehicle communications, indicate that HARQ-based power adaptation can effectively compensate for the mismatching issue in PA systems.


\section{Problem Formulation}

Here, we first introduce the basics of PA systems which is followed by our proposed HARQ-based PA setup.

\subsection{Standard PA System}
\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure1.pdf}\\
\caption{Predictor antenna system with mismatching problem.}\label{ARQmodel}
\end{figure}
Figure \ref{ARQmodel} shows the standard PA system with two antennas on the roof of a vehicle. Here, the PA first sends pilots in time $t$. Then, the base station (BS) estimates the PA-BS channel $h_1$ and sends the data in time $t+\delta$ to the RA where  $\delta$ depends on the processing time at the BS. At the same time, the vehicle moves forward $d_\text{m}$ while the antenna separation between the PA and the RA is $d_\text{a}$. Then, considering downlink transmission in the BS-RA link, the  signal received by the RA is
\begin{align}\label{eq_Y}
y = \sqrt{P}h_2 x + z.
\end{align}
Here, $P$ represents the transmit power, $x$ is the input message with unit variance, and $h_2$ is the fading coefficient between the BS and the RA. Also, $z \sim \mathcal{CN}(0,1)$ denotes the independent and identically distributed (IID) complex Gaussian noise added at the receiver.

We represent the probability density function (PDF) and cumulative density function (CDF) of a random variable $A$ by $f_A(\cdot)$ and $F_A(\cdot)$, respectively.  Due to spatial mismatch between the PA and the RA, assuming a semi-static propagation environment, i.e., assuming that the coherence time of the propagation environment is much larger than $\delta$, $h_2$ and $h_1$ are correlated according to \cite[Eq. 5]{Guo2019WCLrate} 
\begin{align}\label{eq_H}
    h_2 = \sqrt{1-\sigma^2} h_1 + \sigma q,
\end{align}
where $q \sim \mathcal{CN}(0,1)$ which is independent of the known channel value $h_1\sim \mathcal{CN}(0,1)$, and $\sigma$ is a function of the mis-matching distance $d = |d_\text{a}-d_\text{m}|$ \cite[Eq. 4]{Guo2019WCLrate}. Defining $g_1 = |h_1|^2$ and $ g_2 = |h_2|^2$, the CDF $F_{g_2|g_1}$ is given by
\begin{align}\label{eq_cdf}
    F_{g_2|g_1}(x) = 1 - Q_1\left( \sqrt{\frac{2g_1(1-\sigma^2)}{\sigma^2}}, \sqrt{\frac{2x}{\sigma^2}}  \right),
\end{align}
where $Q_1(s,\rho) = \int_{\rho}^{\infty} xe^{-\frac{x^2+s^2}{2}}I_0(xs)\text{d}x$, $s, \rho \ge 0$, is the first-order Marcum $Q$-function. Also, $I_n(x) = (\frac{x}{2})^n \sum_{i=0}^{\infty}\frac{(\frac{x}{2})^{2i} }{i!\Gamma(n+i+1)}$ is the $n$-order modified Bessel function of the first kind, and $\Gamma(z) = \int_0^{\infty} x^{z-1}e^{-x} \mathrm{d}x$ represents the Gamma function. In this way, although parameter adaptation is performed based on perfect CSIT of $h_1$ at time $t$, the spatial mismatch may lead to unsuccessful decoding by the RA  at $t+\delta$.


\subsection{Proposed HARQ-based PA System}
Along with the spatial mismatch problem, the typical PA system suffers from poor spectral efficiency because the PA is used only for channel estimation. On the other hand, because the PA system includes the PA-BS feedback link,  HARQ can be supported by the PA structure. For this reason, we propose a setup as follows.

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure2.pdf}\\
\caption{Time structure for the proposed PA-HARQ scheme.}\label{fig_timeslot}
\end{figure}

Here, as  seen in Fig. \ref{fig_timeslot}, with no CSIT, at $t_1$ the BS sends pilots as well as the encoded data with certain initial rate $R$ and power $P_1$ to the PA. At $t_2$, the PA estimates the channel $h_1$ from the received pilots. At the same time, the PA tries to decode the signal. If the message is correctly decoded, i.e., $R\leq \log(1+g_1P_1)$,  an acknowledgment (ACK) is fed back to the BS at $t_3$, and the data transmission stops. Otherwise, the PA sends both a negative acknowledgment (NACK) and high accuracy quantized CSI feedback about $h_1$. The number of quantization bits are large enough such that we can assume the BS to have perfect CSIT of $h_1$ (see \cite{guo2020semilinear} for the effect of imperfect CSIT on the performance of PA systems). With NACK, in the second transmission round at time $t_4$, the BS  transmits the message to the RA with power $P_2$  which is a function of the instantaneous channel quality $g_1$. The outage occurs if the RA cannot decode the message at the end of the second round. 

\section{Analytical Results}
Let $\epsilon$ be the outage probability constraint. Here, we present the results for the cases with RTD and INR HARQ protocols. With an RTD protocol, the same signal (with possibly different power) is sent in each retransmission round, and the receiver performs maximum ratio combining of all received copies of the signal. With INR, on the other hand, new redundancy bits are sent in the retransmissions, and the receiver decodes the message by combining all received signals \cite{makki2014green,chaitanya2011outage,djonin2008joint}.

Considering Rayleigh fading conditions with $f_{g_1}(x) =  e^{- x}$, the outage probability at the end of Round 1 is given by
\begin{align}\label{eq_pout}
&\text{Pr}(\text{Outage, Round 1}) = \text{Pr}\left\{R\leq \log(1+g_1P_1)\right\}\nonumber\\
&~~ = \text{Pr}\left\{g_1\leq \frac{e^{R}-1}{P_1}\right\}
 = 1-e^{ -\frac{\theta}{P_1}}, 
\end{align}
where $\theta = e^{R}-1$. Then, using the results of, e.g.,  \cite[Eq. 7, 18]{makki2014green} on the outage probability of the RTD- and INR-based HARQ protocols, the power allocation problem for the proposed HARQ-based PA system can be stated as
\begin{equation}
\label{eq_optproblem}
\begin{aligned}
\min_{P_1,P_2} \quad & \mathbb{E}_{g_1}\left[P_\text{tot}|g_1\right] \\
\textrm{s.t.} \quad &  P_1, P_2 > 0,\\
&P_\text{tot}|g_1 = \left[P_1 + P_2(g_1) \times \mathcal{I}\left\{g_1 \le \frac{\theta}{P_1}\right\}\right],
\end{aligned}
\end{equation}
with
\begin{align}\label{eq_optproblemrtd}
F_{g_2|g_1}\left\{\frac{\theta-g_1P_1}{P_2(g_1)}    \right\} = \epsilon, \quad\text{for RTD}
\end{align}
\begin{align}\label{eq_optprobleminr}
F_{g_2|g_1}\left\{\frac{e^{R-\log(1+g_1P_1)}-1}{P_2(g_1)}    \right\} = \epsilon, \quad\text{for INR}. 
\end{align}
Here, $P_\text{tot}|g_1$ is the total instantaneous transmission power for two transmission rounds (i.e., one retransmission) with given $g_1$, and we define $\Bar{P} \doteq \mathbb{E}_{g_1}\left[P_\text{tot}|g_1\right]$ as the expected power, averaged over $g_1$. Moreover, $\mathcal{I}(x)=1$ if $x>0$ and $\mathcal{I}(x)=0$ if $x \le 0$. Also, $\mathbb{E}_{g_1}[\cdot]$ represents the expectation operator over $g_1$. Here, we ignore the peak power constraint and assume that the BS is capable for  sufficiently high transmission powers. Finally, (\ref{eq_optproblem})-(\ref{eq_optprobleminr}) come from the fact that, with our proposed scheme, $P_1$ is fixed and optimized with no CSIT at the BS and based on average system performance. On the other hand, $P_2$ is adapted continuously based on the predicted CSIT.


Using (\ref{eq_optproblem}), the required power in Round 2 is given by
\begin{equation}
\label{eq_PRTDe}
    P_2(g_1) = \frac{\theta-g_1P_1}{F_{g_2|g_1}^{-1}(\epsilon)},
\end{equation}
for the RTD, and
\begin{equation}
\label{eq_PINRe}
    P_2(g_1) = \frac{e^{R-\log(1+g_1P_1)}-1}{F_{g_2|g_1}^{-1}(\epsilon)},
\end{equation}
for the INR, where $F_{g_2|g_1}^{-1}(\cdot)$ is the inverse of the CDF given in (\ref{eq_cdf}). Note that, $F_{g_2|g_1}^{-1}(\cdot)$ is a complex function of $g_1$ and, consequently, it is not possible to express $P_2$ in closed-form. For this reason, one can use   \cite[Eq. 2, 7]{6414576}
\begin{align}
    Q_1 (s, \rho) &\simeq e^{\left(-e^{\mathcal{I}(s)}\rho^{\mathcal{J}(s)}\right)}, \nonumber\\
    \mathcal{I}(s)& = -0.840+0.327s-0.740s^2+0.083s^3-0.004s^4,\nonumber\\
    \mathcal{J}(s)& = 2.174-0.592s+0.593s^2-0.092s^3+0.005s^4,
\end{align}
to approximate $F_{g_2|g_1}$ and consequently $F_{g_2|g_1}^{-1}(\epsilon)$. In this way, (\ref{eq_PRTDe}) and (\ref{eq_PINRe}) can be approximated as
\begin{equation}
\label{eq_PRTDa}
    P_2(g_1) = \Omega\left(\theta-g_1P_1\right),
\end{equation}
for the RTD, and
\begin{equation}
\label{eq_PINRa}
   P_2(g_1) = \Omega\left(e^{R-\log(1+g_1P_1)}-1\right),
\end{equation}
for the INR, where
\begin{equation}\label{eq_omega}
    \Omega (g_1) = \frac{2}{\sigma^2}\left(\frac{\log(1-\epsilon)}{-e^{\mathcal{I}\left(\sqrt{\frac{2g_1(1-\sigma^2)}{\sigma^2}}\right)}}\right)^{-\frac{2}{\mathcal{J}\left(\sqrt{\frac{2g_1(1-\sigma^2)}{\sigma^2}}\right)}}.
\end{equation}



In this way, for different HARQ protocols, we can express the  instantaneous transmission power of Round 2, for every given $g_1$ in closed-form. Then, the  power allocation problem (\ref{eq_optproblem}) can be solved numerically. However, (\ref{eq_omega}) is still complicated and it is not possible to solve (\ref{eq_optproblem}) in closed-form. For this reason, we propose an approximation scheme to solve (\ref{eq_optproblem}) as follows.




Let us initially concentrate on the RTD protocol. Then,  combining (\ref{eq_optproblem}) and (\ref{eq_PRTDe}), the expected total transmission power  is given by
\begin{align}\label{eq_barP}
    \Bar{P}_\text{RTD} = P_1 + \int_0^{\theta/P_1} e^{- x}P_2\text{d}x
    = P_1 + \int_0^{\theta/P_1} e^{- x}\frac{\theta-x P_1}{F_{g_2|x}^{-1}(\epsilon)}\text{d}x.
\end{align}
Then, Theorem \ref{theorem1} derives the minimum required power  in Round 1 and the average total power consumption as follows. 



\begin{theorem}\label{theorem1}
With RTD and given outage constraint $\epsilon$, the minimum required power in Round 1 and the average total power are given by (\ref{eq_P1}) and (\ref{eq_666666}), respectively. 
\end{theorem}
\begin{proof}
Plugging (\ref{eq_cdf}) into (\ref{eq_optproblemrtd}), we have
\begin{align}
    1-Q_1\left(\sqrt{\frac{2g_1(1-\sigma^2)}{\sigma^2}},\sqrt{\frac{2(\theta-g_1P_1)}{\sigma^2 P_2}}\right) = \epsilon.
\end{align}
By using the approximation \cite[Eq. 17]{Azari2018TCultra} for moderate/large $\sigma$, i.e., if $1-Q_1(s,\rho) = 1-\epsilon$, then $\rho = Q_1^{-1}(s, 1-\epsilon) \simeq \sqrt{-2\log(1-\epsilon)}e^{\frac{s^2}{4}}$, we can obtain 
\begin{align}
    \sqrt{\frac{2(\theta-g_1P_1)}{\sigma^2 P_2}}\simeq \sqrt{-2\log(1-\epsilon)}e^{\frac{g_1(1-\sigma^2)}{2\sigma^2}}.
\end{align}
In this way, $P_2$ in (\ref{eq_barP}) is approximated by
\begin{align}
    P_2 \simeq (\theta - g_1P_1)\frac{e^{-\frac{g_1(1-\sigma^2)}{\sigma^2}}}{-\sigma^2\log(1-\epsilon)},
\end{align}
and considering RTD, (\ref{eq_barP}) can be rewritten as
\begin{align}\label{eq_Papprobeforederrivative}
    \Bar{P} &= P_1 + \int_0^{\theta/P_1} e^{- x}(\theta - xP_1)\frac{e^{-\frac{x(1-\sigma^2)}{\sigma^2}}}{-\sigma^2\log(1-\epsilon)}\text{d}x \nonumber\\
    &\overset{(a)}{=} P_1 + \frac{c}{m^2}\left(P_1 e^{-\frac{m\theta}{P_1}}-P_1 + m\theta\right),
\end{align}
where, in (a) we set $m = 1 + \frac{1-\sigma^2}{\sigma^2}$ and $c = \frac{-1}{\sigma^2\log(1-\epsilon)}$ for simplicity. Then, setting the derivative of (\ref{eq_Papprobeforederrivative})  with respect to $P_1$ equal to zero, the minimum $P_1$ for the minimum total power can be find as
\begin{align}
  \label{eq_P1}
    \hat{P}_{1,\text{RTD}} & = \operatorname*{arg}_{P_1 > 0} \Bigg\{ 1 +  \frac{c}{m^2}e^{-\frac{\theta m}{P_1}}\left(\frac{m\theta}{P_1}+1\right) - \frac{c}{m^2} = 0\Bigg\}\nonumber\\
    & = \operatorname*{arg}_{P_1 > 0} \left\{e^{-\frac{\theta m}{P_1}}\left(\frac{m\theta}{P_1}+1\right) = 1-\frac{m^2}{c} \right\}\nonumber\\
    & \overset{(b)}= \frac{-m\theta}{\mathcal{W}_{-1}\left(\frac{m^2}{ce}-\frac{1}{e}\right)+1}.
\end{align}
Here, $(b)$ is obtained by the definition of the Lambert W function $xe^x = y \Leftrightarrow x = \mathcal{W}(y)$ \cite{corless1996lambertw}. Also, because $\frac{m^2}{ce}-\frac{1}{e}<0$, we use the $\mathcal{W}_{-1}(\cdot)$ branch \cite[Eq. 16]{veberic2010having}. Then, plugging (\ref{eq_P1}) into (\ref{eq_Papprobeforederrivative}), we obtain the  minimum total transmission power as
\begin{align}\label{eq_666666}
    \hat{\Bar{P}}_{\text{RTD}} =\hat{P}_{1,\text{RTD}} + \frac{c}{m^2}\left(\hat{P}_{1,\text{RTD}} e^{-\frac{m\theta}{\hat{P}_{1,\text{RTD}}}}-\hat{P}_{1,\text{RTD}} + m\theta\right).
\end{align}
\end{proof}


\subsection{On the Effect of CSI Feedback/Power Allocation}
As a benchmark, in this part, we consider the case without exploiting CSIT, i.e., we consider the typical HARQ schemes where CSI feedback is not sent along with NACK, and we do not perform power adaptation.  Here, the outage probability,  for the RTD and the INR  are given by
\begin{align}\label{eq_PrRTD}
    \zeta_{\text{RTD}} = \text{Pr}\left\{\log\left(1+\left(g_1+g_2\right)P\right)<R\Big|g_1<\frac{\theta}{P}  \right\},
\end{align}
\begin{align}\label{eq_PrINR}
\begin{split}
    \zeta_{\text{INR}}=\text{Pr}\left\{\log\left(1+g_1P\right) + \log\left(1+g_2P\right)<R\Big|g_1<\frac{\theta}{P}\right\}.
\end{split}
\end{align}
Also, in both protocols, the total average power is given by
\begin{align}\label{eq_barpbench}
    \Bar{P} &= P + P\cdot\text{Pr}\{\log\left(1+g_1P\right)<R\}\nonumber\\
    &=P(2-e^{-\frac{\theta}{P}}).
\end{align}
\begin{theorem}\label{theorem2}
Without CSIT feedback/power allocation, the outage probability of the RTD-based PA-HARQ scheme is given by (\ref{eq_RTDnopa}).
\end{theorem}
\begin{proof}
Using (\ref{eq_PrRTD}), we have
\begin{align}
    \zeta_{\text{RTD}} &= \text{Pr}\left\{g_2< \frac{\theta}{P}-g_1  \Big| g_1 < \frac{\theta}{P} \right\}\nonumber\\
    &= \frac{1}{1-e^{-\frac{\theta}{P}}}\int_{0}^{\frac{\theta}{P}} e^{- x} F_{g_2|x}\left(\frac{\theta}{P}-x\right) \text{d}x. \label{eq_nocloseform}
\end{align}
Considering (\ref{eq_cdf}), there is no closed-form solution for (\ref{eq_nocloseform}).  For this reason, we use the  approximation \cite[Eq. 14]{andras2011generalized} 
\begin{align}
    Q_1\left( s, \rho  \right) \simeq  1 - \left( 1 + \frac{s^2}{2} \right)e^{-\frac{s^2}{2}} +
    \left( 1 + \frac{s^2}{2} + \frac{s^2\rho^2}{4} \right)e^{-\frac{s^2+\rho^2}{2}},
\end{align}
which simplifies (\ref{eq_nocloseform}) to 
% \begin{align}\label{eq_RTDnopa}
%     \zeta_{\text{RTD}} &\simeq \int_{0}^{\frac{\theta}{P}}\left(1+\frac{ax}{2}\right)e^{-\frac{ax}{2}-x} \text{d}x -\nonumber\\ 
%     & \int_{0}^{\frac{\theta}{P}} \left(1+\frac{ax}{2}+\frac{a^2\frac{\theta}{P} x-a^2x^2}{4}\right)e^{-\frac{a\frac{\theta}{P}}{2}-x}\text{d}x\nonumber\\
%     & = \Bigg( (16a +16)e^{\frac{a\frac{\theta}{P}}{2}+\frac{\theta}{P}} +\bigg(\left(-a^4-4a^3-4a^2\right)\frac{\theta}{P}+\nonumber\\
%     &     2a^4+6a^3-4a^2-24a-16\bigg)e^{\frac{\theta}{P}} +(-a^4-2a^3)\frac{\theta}{P}-\nonumber\\ &2a^4-6a^3+4a^2+8a \Bigg)\frac{e^{-\frac{a\frac{\theta}{P}}{2}-\frac{\theta}{P}}}{4a^2+16a+16}.
% \end{align}
\begin{align}\label{eq_RTDnopa}
    &\zeta_{\text{RTD}} \simeq 
    -\frac{e^{-\frac{\theta}{P\sigma^2}}}{6\sigma^4\left(1-e^{-\frac{\theta}{P}}\right)}\Bigg(\left(6\sigma^8-12\sigma^6\right)e^{\frac{\theta}{P\sigma^2}}+12\sigma^6+\nonumber\\&\left(3\sigma^2-3\sigma^4\right)\frac{\theta^2}{P^2}+\left(12\sigma^4-6\sigma^6\right)\frac{\theta}{P}+\left(1-\sigma^2\right)\frac{\theta^3}{P^3}-6\sigma^8\Bigg)
\end{align}
% -\dfrac{\mathrm{e}^{-\frac{{\theta}}{a^2}}\left(\left(6a^8-12a^6\right)\mathrm{e}^\frac{{\theta}}{a^2}+\left(1-a^2\right){\theta}^3+\left(3a^2-3a^4\right){\theta}^2+\left(12a^4-6a^6\right){\theta}-6a^8+12a^6\right)}{6a^4}

% \begin{align}
%     (e^{-(a*\theta)/2-\theta}*((16*a+16)*e^{(a*\theta)/2+\theta}+((-a^4-4*a^3-4*a^2)*\theta+2*a^4+6*a^3-4*a^2-24*a-16)*e^{\theta}+(-a^4-2*a^3)*\theta-2*a^4-6*a^3+4*a^2+8*a))/(4*a^2+16*a+16)
% \end{align}
% \begin{equation}\label{eq_lemma2list}
% \left\{
%              \begin{array}{ll}
%              a   = &\frac{2}{\sigma^2},  \\
%              l_1 = & (16a + 16)e^{\frac{a\frac{\theta}{P}}{2}+\frac{\theta}{P}},\\
%              l_2 = & \left(\left(-a^4-4a^3-4a^2\right)\frac{\theta}{P}+ \right. \\  &  \left. 2a^4+6a^3-4a^2-24a-16\right)e^{\frac{\theta}{P}},\\
%              l_3 = & (-a^4-2a^3)\frac{\theta}{P}-2a^4-6a^3+4a^2+8a.
%              \end{array}
% \right.
% \end{equation}
\end{proof}

\subsection{On the Effect of INR-based Scheme}
For the INR scheme, by using Jensen's inequality and the concavity of the logarithm function \cite[Eq. 30]{makki2016TWCRFFSO}
\begin{align}\label{eq_jensen}
   \frac{1}{n}\sum_{i=1}^{n} \log (1+x_i)\leq\log\left(1+\frac{1}{n}\sum_{i=1}^{n}x_i\right),
\end{align}
the closed-form expressions for the minimum required power, the average total power, as well as outage probability without power allocation are given by the following Corollary.
\begin{corollary}
With INR, the minimum required power in Round 1 and the average total power are given by (\ref{eq_P1inr}) and (\ref{eq_barpinr}), respectively.  Also, without power allocation, the outage probability of INR-based scheme is given by (\ref{eq_INRnopa}).
\end{corollary}
\begin{proof}
Using (\ref{eq_optprobleminr}), the Jensen's inequality (\ref{eq_jensen}) and defining $\theta_1 =2\left(e^{\frac{R}{2}}-1\right)$, (\ref{eq_PINRe}) can be approximated by
\begin{align}
     P_2(g_1) \simeq \frac{\theta_1 - g_1P_1}{F_{g_2|g_1}^{-1}(\epsilon)},
\end{align}
and, following the same steps as in Theorem \ref{theorem1}, we obtain the minimum required $P_1$ for the minimum total power in INR scheme as
\begin{align}
  \label{eq_P1inr}
    \hat{P}_{1,\text{INR}}= \frac{-m\theta_1}{\mathcal{W}_{-1}\left(\frac{m^2}{ce}-\frac{1}{e}\right)+1}.
\end{align}
Also, the  minimum total  power can be calculated by
\begin{align}\label{eq_barpinr}
    \hat{\Bar{P}}_{\text{INR}} =\hat{P}_{1,\text{INR}} + \frac{c}{m^2}\left(\hat{P}_{1,\text{INR}} e^{-\frac{m\theta_1}{\hat{P}_{1,\text{INR}}}}-\hat{P}_{1,\text{INR}} + m\theta_1\right).
\end{align}

Finally, (\ref{eq_PrINR}) can be further derived by
\begin{align}
    \zeta_{\text{INR}} &= \text{Pr}\left\{  g_2< \frac{e^{R-\log(1+g_1)}-1}{P}\Big|g_1 < \frac{\theta}{P} \right\}\nonumber\\
    % &= \frac{1}{1-e^{-\frac{\theta}{P}}}\int_{0}^{\frac{\theta}{P}} e^{- x} F_{g_2|x}\left(\frac{e^{R-\log(1+x)}-1}{P}\right) \text{d}x\nonumber\\
    &\overset{(c)}{\simeq}\frac{1}{1-e^{-\frac{\theta}{P}}}\int_{0}^{\frac{\theta}{P}} e^{- x} F_{g_2|x}\left(\frac{\theta_1}{P}-x\right) \text{d}x,
\end{align}
with $(c)$ using Jensen's inequality. Then, following the same steps as in Theorem \ref{theorem2}, the outage probability is found as 
\begin{align}\label{eq_INRnopa}
    \zeta_{\text{INR}} \simeq \zeta_{\text{RTD}}(\theta = \theta_1).
\end{align}
\end{proof}


% \subsection{On the Effect of PA System}
% For the case without PA, i.e., with no retransmission,  the outage probability can be written as

% \begin{align}\label{eq_nocsinopa}
%     \zeta_{\text{no-CSI}} = \int_0^{\frac{\theta}{P}} e^{- x} \text{d}x = 1-e^{-\frac{\theta}{P}}.
% \end{align}

% Here, results obtained from Lemma 2, Corollary 2 and (\ref{eq_nocsinopa}) provide the benchmark for the HARQ-based PA system terms of outage probability. Also, the transmission power is set according to
% \begin{align}\label{eq_nofeedback}
% &\text{Pr}\left\{ \log(1+g_1P_1) < R \right\} \leq \epsilon\nonumber\\
%   & \Rightarrow P_1 \geq \frac{1-e^{R}}{\log(1-\epsilon)}.
% \end{align}
% This provides the lower bound of the system performance.









\section{{Simulation Results}}

In the simulations, we set $ \delta$ = 5 ms, $f_\text{c}$ = 2.68 GHz, and $d_\text{a} = 1.5\lambda$. Each point in the figures is obtained by averaging the system performance over $1\times10^5$ channel realizations. 

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure3.pdf}\\
\caption{Minimum required power under different outage constraints for the RTD and the INR, $\sigma = 0.8$, $R = 0.5, 2$ npcu.}\label{figure3}
\end{figure}

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure4.pdf}\\
\caption{Outage probability for a broad range of  average power (\ref{eq_barpbench}), without power optimization, $\sigma$ = 0.8, $R$ = 0.5, 2 npcu.}\label{figure4}
\end{figure}


\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure5.pdf}\\
\caption{Minimum required power for the RTD and the INR with given outage constraint, for different speed $v$. $R = 3$ npcu, $\epsilon = 10^{-3}$.}\label{figure5}
\end{figure}

Figure \ref{figure3} shows the results of the power allocation problem (\ref{eq_optproblem}) for both the RTD and the INR with different initial rates $R = 0.5, 2$ npcu, $\sigma = 0.8$, and different outage probability constraints $\epsilon$. Here, the simulation results are obtained from  solving the optimization problem (\ref{eq_optproblem}) numerically, while the approximation results for the RTD and the INR are obtained by Theorem \ref{theorem1} and Corollary 1, respectively. Also, as a benchmark, we consider the case with no retransmission where the outage probability is given by $1-e^{-\frac{\theta}{P}}$. In this case, the required outage-constrained power without retransmission is given by $P \geq \frac{1-e^{R}}{\log(1-\epsilon)}$.  In Fig. \ref{figure4}, we plot the outage probability using the  RTD and the INR  without power optimization. Here, we set $\sigma = 0.8$, and the initial rate $R = 0.5, 2$ npcu. The simulation results are obtained by (\ref{eq_PrRTD}) and (\ref{eq_PrINR}), while the analytical approximations are obtained from Theorem \ref{theorem2} for the RTD and Corollary 1 for the INR. Finally, in Fig. \ref{figure5},  we study the minimum required transmission power for different speeds $v$. Here, manipulating $v$ is  equivalent to changing the level of spatial correlation for given values of $\delta$, $f_\text{c}$ and $d_\text{a}$ (see \cite{guo2020semilinear} for the detailed effect of the vehicle speed on the spatial correlation). Also, we study the effect of different values of $d_\text{a}$ on the system performance.   According to the figures, we can conclude the following:






%=============
%Fig: benchmark
%=============



%=============
%Fig: numerical solution-speed v
%=============









%=============
%Fig: numerical solution-outage constraint
%=============








\begin{itemize}
    \item The approximation schemes of Theorem \ref{theorem1} and Corollary 1 are  tight for a broad range of values of initial rate $R$, speed $v$,  as well as $\epsilon$ (Figs. \ref{figure3} and \ref{figure5}). Thus, for different parameter settings, the outage-constrained power allocation for the RTD and the INR can be well determined by Theorem \ref{theorem1} and Corollary 1. 
    \item Also, the approximation scheme of Theorem \ref{theorem2} is tight for a broad range of values of average power (\ref{eq_barpbench}) as well as initial rate $R$ (Fig. \ref{figure4}). Thus, for different parameter settings, the outage probability for the proposed PA-HARQ scheme without power allocation, can be well determined by Theorem \ref{theorem2} and Corollary 1.
    \item With the deployment of the PA and power allocation, remarkable power gain is achieved especially at low outage probabilities  (Figs. \ref{figure3} and \ref{figure5}). Moreover,  as also indicated in, e.g.,  \cite{makki2014green}, INR outperforms RTD, in terms of outage-limited average power. However, the difference between the performance of these protocols decreases as the data rate or $\sigma$ decreases (Figs. \ref{figure3} and \ref{figure5}).
    \item Figures \ref{figure3}-\ref{figure5} emphasize the efficiency of HARQ as well as adaptive power allocation in the PA system. From Fig. \ref{figure4}, we can see that with the PA-HARQ setup, even without power allocation, we can obtain considerable performance improvements compared to the case with no retransmission. Then, as seen in Fig. \ref{figure3}, with power allocation there is much larger gain for the system performance. For instance, with $\epsilon=10^{-5}$ and $R = 4$ npcu, the RTD- and INR-based PA-HARQ can reduce the required power, compared to no retransmission case, by 25 and 30 dB, respectively. Then, as can be seen from Fig.  \ref{figure5}, the effect of power-optimized PA-HARQ increases with $\sigma$. This is because the larger $\sigma$ provides better spatial diversity of the channel, which can improve the performance with retransmissions. For the peaks in Fig. \ref{figure5}, the channel for the retransmission has the largest correlation with the one in the first round, which leads to the smallest power gain. Moreover, when the antenna separation $d_\text{a}$ decreases, the speed where the power gain is minimum, also decreases, due to the reduction of the mismatching distance $d$.
\end{itemize}



\section{Conclusion}
We studied the PA-HARQ system with the mismatching problem, in the context of outage-constrained power allocation. We derived  closed-form expressions for the minimum instantaneous and  total transmit power. The approximations are tight for a broad range of system configurations. Also, the  results show that, while PA-assisted adaptive power adaptation leads to considerable performance improvements, the total transmission power and the outage probability are remarkably affected by the spacial mismatching.




% use section* for acknowledgment
%  \section*{Acknowledgment}
% % % The research leading to these results received funding from the European Commission H2020 programme under grant agreement $n^{\circ}$671650 (5G PPP mmMAGIC project), and from the Swedish Governmental Agency for Innovation Systems (VINNOVA) within the VINN Excellence Center Chase.

% This work has been partly performed in the framework of the H2020 project 5GCAR co-funded by the EU and has also been supported in part by VINNOVA (Swedish Government Agency for Innovation Systems) within the VINN Excellence Center ChaseOn. The authors would like to acknowledge the contributions of their colleagues.






==> YourThesis/papers/Letter2/info.tex <==


% only comma separated full names
\paperauthor{\textbf{H. Guo}, B. Makki, M.-S. Alouini, and T. Svensson}

% \paperinfo[short info]{full info}
\paperinfo[Submitted to  \textit{IEEE Wireless Communication Letters}, Apr. 2020, under minor revision]{
    \textit{Submitted to IEEE Wireless Communication Letters},\\
	 Apr. 2020, under minor revision.\\
	\copyright 2020 IEEE
}

% \papertitle[short title]{full title}
\papertitle[Power Allocation in HARQ-based Predictor Antenna Systems]{Power allocation in HARQ-based predictor antenna systems}

% if you want to use an auto-generated paper summary, please fill in the variable \papersummary{}.
\papersummary{In this paper we...}






==> YourThesis/papers/T1/c.tex <==



\begin{abstract}
First-order Marcum $Q$-function is observed in various problem formulations. However, it is not an easy-to-handle function. For this reason, in this paper, we first present a semi-linear approximation of the Marcum $Q$-function. Our proposed approximation is useful because it simplifies, e.g., various integral calculations including the Marcum $Q$-function as well as different operations such as parameter optimization. Then, as an example of interest, we apply our proposed approximation approach to the performance analysis of predictor antenna (PA) systems. Here, the PA system is referred to as a system with two sets of antennas on the roof of a vehicle. Then, the PA positioned in the front of the vehicle can be used to improve the channel state estimation for data transmission of the receive antenna  that is aligned behind the PA. Considering spatial mismatch due to the mobility, we derive closed-form expressions for the instantaneous and average throughput as well as the throughput-optimized rate allocation. As we show, our proposed approximation scheme enables us to analyze PA systems with high accuracy. Moreover, our results show that rate adaptation can improve the performance of PA systems with different levels of spatial mismatch.
\end{abstract}
\keywords{Backhaul, channel state information (CSI),  integrated access and backhaul (IAB), linear approximation, Marcum $Q$-function, mobility, mobile relay, outage probability, predictor antenna, rate adaptation, spatial correlation, throughput.}

% no keywords




% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle





\section{Introduction}

The first-order Marcum $Q$-function\footnote{To simplify the analysis, our paper concentrates on the approximation of the first-order Marcum-$Q$ function. However, our approximation technique can be easily extended to the cases with different orders of Marcum $Q$-function.} is defined as  \cite[Eq. (1)]{Bocus2013CLapproximation}
\begin{align}
    Q_1(\alpha,\beta) = \int_{\beta}^{\infty} xe^{-\frac{x^2+\alpha^2}{2}}I_0(x\alpha)\text{d}x,
\end{align}
where $\alpha, \beta \geq 0$ and $I_n(x) = (\frac{x}{2})^n \sum_{i=0}^{\infty}\frac{(\frac{x}{2})^{2i} }{i!\Gamma(n+i+1)}$ is the $n$-order modified Bessel function of the first kind, and $\Gamma(z) = \int_0^{\infty} x^{z-1}e^{-x} \mathrm{d}x$ represents the Gamma function. Reviewing the literature,  the Marcum $Q$-function has appeared in many areas such as statistics/signal detection \cite{helstrom1994elements}, and in the performance analysis of different setups such as temporally correlated channels \cite{Makki2013TCfeedback}, spatially correlated channels \cite{Makki2011Eurasipcapacity},  free-space optical (FSO) links \cite{Makki2018WCLwireless}, relay networks \cite{Makki2016TVTperformance}, as well as  cognitive radio and radar systems \cite{Simon2003TWCsome,Suraweera2010TVTcapacity,Kang2003JSAClargest,Chen2004TCdistribution,Ma2000JSACunified,Zhang2002TCgeneral,Ghasemi2008ICMspectrum,Digham2007TCenergy, simon2002bookdigital,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan,ermolova2014laplace,peppas2013performance}. However, in these applications, the presence of the Marcum $Q$-function makes the mathematical analysis challenging, because it is  difficult to manipulate  with no closed-form  expressions especially when it appears in parameter optimizations and integral calculations. For this reason, several methods have been developed in \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,zhao2008ELtight,Simon2000TCexponential,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral,jimenez2014connection}  to bound/approximate the  Marcum $Q$-function. For example, \cite{Fu2011GLOBECOMexponential,zhao2008ELtight} have proposed  modified forms of the function, while \cite{Simon2000TCexponential,annamalai2001WCMCcauchy} have derived exponential-type bounds which are good for the bit error rate analysis at high signal-to-noise ratios (SNRs). Other types of bounds are expressed by, e.g., error function \cite{Kam2008TCcomputing} and Bessel functions \cite{Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral}. Some alternative methods have been also proposed in \cite{Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Bocus2013CLapproximation,Gaur2003TVTsome}. Although each of these approximation/bounding techniques are fairly tight for their considered problem formulation, they are still based on difficult functions, or have complicated summation/integration formations, which may be not easy to deal with in, e.g., integral calculations and parameter optimizations. 


In this paper, we first propose a simple semi-linear approximation of the first-order Marcum $Q$-function (Lemma \ref{Lemma1}, Corollaries \ref{coro1}-\ref{coro2}). As we explain in the following (Lemmas \ref{Lemma1}-\ref{Lemma4}), in contrast to the schemes of \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,zhao2008ELtight,Simon2000TCexponential,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral,jimenez2014connection}, our proposed approximation is not tight at the tails of  the Marcum $Q$-function. Therefore, it is not useful in, e.g., error probability-based problem formulations.  On the other hand, the advantages of our proposed approximation method, compared to \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,zhao2008ELtight,Simon2000TCexponential,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral,jimenez2014connection}, are 1) its simplicity, and 2) tightness in the moderate values of the function. This is important because, as observed in, e.g., \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,Makki2013TCfeedback,Makki2011Eurasipcapacity,Makki2018WCLwireless,Makki2016TVTperformance,Simon2003TWCsome,Suraweera2010TVTcapacity,Ma2000JSACunified,Digham2007TCenergy,Cao2016CLsolutions,sofotasios2015solutions,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan}, in different applications, the Marcum $Q$-function is typically combined with other functions which tend to zero at the tails of the Marcum $Q$-function. In such cases, the inaccuracy of the approximation at the tails does not affect the tightness of the final analysis. Thus, our proposed scheme provides tight and simple approximation results for different problem formulations such as capacity calculation \cite{Makki2011Eurasipcapacity,Suraweera2010TVTcapacity}, throughput/average rate derivation \cite{Makki2013TCfeedback,Makki2018WCLwireless,Makki2016TVTperformance}, energy detection of unknown signals over various multipath fading channels \cite{Digham2007TCenergy,Cao2016CLsolutions,sofotasios2015solutions}, as well as  performance evaluation of  non-coherent receivers in radar systems \cite{Cui2012ELtwo}. Also, the simplicity of the approximation method makes it possible to perform further analysis such as parameter optimization and to obtain intuitive insights from the derivations.


To demonstrate the usefulness of the proposed approximation technique in communication systems, we analyze the performance of predictor antenna (PA) systems in presence of spatial mismatch. Here, the PA system is referred to as a setup with two (sets of) antennas on the roof of a vehicle. The PA positioned in the front of a vehicle can be used to improve the channel state estimation for downlink data reception at the receive antenna (RA) on the vehicle that is aligned behind the PA \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects,Guo2019WCLrate}. 


The feasibility of PA setups, which are of interest particularly in public transport systems such as trains and buses, but potentially also for the more design-constrained cars, has been previously shown through experimental tests \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman}. Particularly, as shown in testbed implementations, e.g.,  \cite{BJ2017PIMRCpredictor} and \cite{BJ2017ICCWusing}, with a two-antenna PA setup a normalised mean square error  of around -10 dB can be obtained for speeds up to 50 km/h, with  measured predictions horizons up to three times the wavelengths. This is by an order of magnitude better than state-of-the-art Kalman prediction-based systems \cite{Ekman2002,Aronsson2011} with prediction horizon limited to 0.1-0.3 times the wavelength. Moreover, the  European project deliverables, e.g., ARTIST4G project \cite[Chapter 2]{ARTIST4G}, METIS project \cite[P. 107]{metis2015d33} and 5GCAR project \cite[Chapter 3]{5gcar2019d33}, have  well addressed the feasibility of the PA concept in network-level design. Finally, different works have analyzed the PA system in both frequency division duplex (FDD) \cite{BJ2017ICCWusing,BJ2017PIMRCpredictor,phan2018WSAadaptive} and time division duplex (TDD) \cite{DT2015ITSMmaking,Apelfrojd2018PIMRCkalman} systems, with some developments on addressing the system challenges such as  antenna coupling \cite{Jamaly2014EuCAPanalysis,Jamaly2019IETeffects}, spatial mismatch \cite{Jamaly2019IETeffects,Guo2019WCLrate}, and spectrum underutilization \cite{guo2020power,guo2020rate}. 

Among the challenges of the PA system is the spatial mismatch. If the RA does not arrive in the same position as the PA, the actual channel for the RA would not be identical to the one experienced by the PA before. Such inaccurate channel state information (CSI) estimation will affect the system performance considerably at moderate/high speeds \cite{DT2015ITSMmaking,Guo2019WCLrate}. 

In this paper, we address the spatial  mismatch problem by implementing adaptive rate allocation. In our proposed setup, the instantaneous CSI provided by the PA is used to adapt the data rate of the signals sent to the RA from the base station (BS). The problem is cast in the form of throughput maximization. Particularly, we use our developed approximation approach to derive closed-form expressions for the instantaneous and average throughput as well as the optimal rate allocation maximizing the throughput (Lemma \ref{Lemma4}). Moreover, we study the effect of different parameters such as the antennas distance, the vehicle speed, and the processing delay of the BS on the performance of PA setups. 


Our paper is different from the state-of-the-art literature because the proposed semi-linear approximation of the first-order Marcum $Q$-function and the derived closed-form expressions for the considered integrals have not been presented by, e.g., \cite{Bocus2013CLapproximation,helstrom1994elements,Fu2011GLOBECOMexponential,Makki2013TCfeedback,Makki2011Eurasipcapacity,Makki2018WCLwireless,Makki2016TVTperformance,Simon2003TWCsome,Suraweera2010TVTcapacity,Kang2003JSAClargest,Chen2004TCdistribution,Ma2000JSACunified,Zhang2002TCgeneral,Ghasemi2008ICMspectrum,Digham2007TCenergy, simon2002bookdigital,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan,ermolova2014laplace,peppas2013performance,zhao2008ELtight,Simon2000TCexponential,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral,jimenez2014connection,Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects,Guo2019WCLrate}. Also, as opposed to \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects}, we perform analytical evaluations on the system performance with CSIT (T: at the transmitter)-based rate optimization to mitigate the effect of the spatial mismatch. Moreover, compared to our preliminary results in \cite{Guo2019WCLrate}, this paper develops the semi-linear approximation method for the Marcum $Q$-function, and uses our proposed approximation method to analyze the performance of the PA system. Also, we perform deep analysis of the effect of various parameters, such as imperfect CSIT feedback schemes, and processing delay of the BS on the system performance. 



The simulation and the analytical results indicate that the proposed semi-linear approximation is useful for the mathematical analysis of different Marcum $Q$-function-based problem formulations. Particularly, our approximation method enables us to represent different Marcum $Q$-function-based integrations and optimizations in closed-form. Considering the PA system, our derived analytical results show that adaptive rate allocation can considerably improve the performance of the PA system in the presence of spatial mismatch. Finally, with different levels of channel estimation, our results show that there exists an optimal speed for the vehicle optimizing the throughput/outage probability, and the system performance is sensitive to the vehicle speed/processing delay as the speed moves away from its optimal value. 


This paper is organized as follows. In Section II, we present our proposed semi-linear approximation of the first-order Marcum $Q$-function, and derive closed-form solutions for some integrals of interest. Section III deals with the application of the approximation in the PA system,  deriving closed-form expressions for the optimal rate adaptation, the instantaneous throughput as well as the expected throughput.  In this way, Sections II and III demonstrate examples on how the proposed approximation can be useful in, respectively, expectation- and optimization-based problem formulations involving the Marcum $Q$-function. Concluding remarks are provided in Section IV. 





\section{Approximation of the first-order Marcum $Q$-function}
In this section, we present our semi-linear approximation of the cumulative distribution function (CDF) in the form of $y(\alpha, \beta ) = 1-Q_1(\alpha,\beta)$. The idea of this proposed approximation is to use one point and its corresponding slope in that point to create a line  approximating the CDF. The approximation method is summarized in Lemma \ref{Lemma1} as follows.
\begin{lem}\label{Lemma1}
 The CDF of the form $y(\alpha, \beta ) = 1-Q_1(\alpha,\beta)$ can be semi-linearly approximated as $Y(\alpha,\beta)\simeq \mathcal{Z}(\alpha, \beta)$ where
\begin{align}\label{eq_lema1}
\mathcal{Z}(\alpha, \beta)=
\begin{cases}
0,  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta < c_1  \\ 
 \frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}\times\\
 ~~~I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)\times\left(\beta-\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)+\\
 ~~~1-Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right),  ~~~~~~\mathrm{if}~ c_1 \leq\beta\leq c_2 \\
1,  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta> c_2,
\end{cases}
\end{align}
with
\begin{align}\label{eq_c1}
   & c_1(\alpha) =~~~ \max\Bigg(0,\frac{\alpha+\sqrt{\alpha^2+2}}{2}+\nonumber\\
    &~~~\frac{Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)-1}{\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)}\Bigg),
\end{align}
\begin{align}\label{eq_c2}
   & c_2(\alpha) = \frac{\alpha+\sqrt{\alpha^2+2}}{2}+\nonumber\\
   & ~~~\frac{Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)}{\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)}.
\end{align}
\end{lem}
\begin{proof}

We aim to approximate the CDF in the range $y \in [0, 1]$ by 
\begin{align}\label{eq_YY}
    y-y_0 = m(x-x_0),
\end{align}
where $\mathcal{C} = (x_0,y_0)$ is a point on the CDF curve and $m$ is the slope at point $\mathcal{C}$ of $y(\alpha,\beta)$. Then, the parts of the line outside this region are replaced by $y=0$ and $y=1$ (see Fig. \ref{fig_CDFilu}).

To obtain a good approximation of the CDF, we select the point $\mathcal{C}$ by solving

\begin{align}\label{eq_partialsquare}
   x = \mathop{\arg}_{t} \left\{  \frac{\partial^2\left(1-Q_1(\alpha,t)\right)}{\partial t^2} = 0\right\},
\end{align}
because the function is symmetric around this point, and (\ref{eq_partialsquare}) gives the best fit for a linear function. Then, using the derivative of the first-order Marcum $Q$-function with respect to $x$ \cite[Eq. (2)]{Pratt1968PIpartial}
\begin{align}\label{eq_derivativeMarcumQ}
    \frac{\partial Q_1(\alpha,x)}{\partial x} = -x e^{-\frac{\alpha^2+x^2}{2}}I_0(\alpha x),
\end{align}
(\ref{eq_partialsquare}) is equivalent to 
\begin{align}
   x =  \mathop{\arg}_{x} \left\{\frac{\partial\left(x e^{-\frac{\alpha^2+x^2}{2}}I_0(\alpha x)\right)}{\partial x}=0\right\}.
\end{align}
Using the approximation $I_0(x) \simeq \frac{e^x}{\sqrt{2\pi x}} $ \cite[Eq. (9.7.1)]{abramowitz1999ia} and writing
\begin{align}
    &~~~\frac{\partial\left(\sqrt{\frac{x}{2\pi \alpha}}e^{-\frac{(x-\alpha)^2}{2}}\right)}{\partial x} = 0\nonumber\\
   \Rightarrow &\frac{1}{\sqrt{2\pi\alpha}}\left(\frac{e^{-\frac{(x-\alpha)^2}{2}}}{2\sqrt{x}}+\sqrt{x}e^{-\frac{(x-\alpha)^2}{2}}(\alpha-x)\right)  = 0\nonumber\\
    \Rightarrow &2x^2-2\alpha x-1 =0,
\end{align}
we obtain 
\begin{align}\label{eq_beta0}
    x = \frac{\alpha+\sqrt{\alpha^2+2}}{2},
\end{align}
since $x\geq0$. In this way, we find the point 
\begin{align}
    \mathcal{C}=\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}, 1-Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)\right).
\end{align}

To calculate the slope $m$ at the point $\mathcal{C}$, we plug (\ref{eq_beta0}) into (\ref{eq_derivativeMarcumQ}) leading to
\begin{align}\label{eq_m}
   & m = \frac{\alpha+\sqrt{\alpha^2+2}}{2}\times\nonumber\\
    & ~~~e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right).
\end{align}
Finally, using (\ref{eq_YY}), (\ref{eq_beta0}) and (\ref{eq_m}), the CDF $y(\alpha, \beta) = 1-Q_1(\alpha,\beta)$ can be approximated  as in (\ref{eq_lema1}). Note that, because the CDF is limited to the range [0 1], the boundaries $c_1$ and $c_2$ in (\ref{eq_lema1}) are obtained by setting $y=0$ and $y=1$ which leads to the semi-linear approximation as given in (\ref{eq_lema1}).
\end{proof}


%==============
%Corollary 1, 2, 3
%==============
To further simplify the calculation, considering different ranges of $\alpha$, the approximation (\ref{eq_lema1}) can be simplified as stated in the following corollaries. 

\begin{corollary}\label{coro1}
For moderate/large values of $\alpha$, we have $y(\alpha,\beta)\simeq\tilde{\mathcal{Z}}(\alpha,\beta)$ where
\begin{align}\label{eq_coro1}
\tilde{\mathcal{Z}}(\alpha,\beta)&\simeq
\begin{cases}
0,  ~~~~~~~~~~~~~\mathrm{if}~\beta < \frac{-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha  \\ 
\alpha e^{-\alpha^2}I_0(\alpha^2)(\beta-\alpha) + 
\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right), \\ ~~~~~~~~~~~~~~~~\mathrm{if}~\frac{-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha \leq\beta\\
~~~~~~~~~~~~~~~~~~~~\leq\frac{1-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha \\
1,  ~~~~~~~~~~~~~\mathrm{if}~ \beta> \frac{1-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha.
\end{cases}\\
&\overset{(a)}{\simeq}
\begin{cases}
0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \beta < \breve{c}_1  \\ 
\frac{1}{\sqrt{2\pi}}(\beta-\alpha) + 
\frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \breve{c}_1 \leq\beta\leq \breve{c}_2 \\
1, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta>\breve{c}_2,
\end{cases}
\end{align}
with $\breve{c}_1$ and $\breve{c}_2$ given in (\ref{eq_dotc1}) and (\ref{eq_dotc2}), respectively.
\end{corollary}

\begin{proof}
Using (\ref{eq_beta0}) for moderate/large values of $\alpha$, we have $x \simeq \alpha$ and
\begin{align}
        \tilde{c}_1 = \frac{-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha,
\end{align}
\begin{align}
     \tilde{c}_2 = \frac{1-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha,
\end{align}
which leads to (\ref{eq_coro1}). Note that in (\ref{eq_coro1}) we have used the fact that \cite[Eq.  (A-3-2)]{schwartz1995communication}
\begin{align}
    Q_1(\alpha,\alpha) = \frac{1}{2}\left(1+e^{-\alpha^2}I_0(\alpha^2)\right).
\end{align}
Finally, $(a)$ is obtained by using the approximation $I_0(x) \simeq \frac{e^x}{\sqrt{2\pi x}}$ where
\begin{align}\label{eq_dotc1}
        \breve{c}_1 = -\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha,
\end{align}
and
\begin{align}\label{eq_dotc2}
     \breve{c}_2 = \sqrt{2\pi}-\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha.
\end{align}
\end{proof}

\begin{corollary}\label{coro2}
For small values of $\alpha$, we have  $y(\alpha,\beta)\simeq\hat{ \mathcal{Z}}(\alpha,\beta)$ with
\begin{align}\label{eq_coro2}
\hat{ \mathcal{Z}}(\alpha,\beta)\simeq
\begin{cases}
0,   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~\beta < \hat{c}_1  \\ 
\frac{\alpha+\sqrt{2}}{2}  e^{-\frac{\alpha^2+\left(\frac{\alpha+\sqrt{2}}{2}\right)^2}{2}}\times\\
~~~I_0\left(\frac{\alpha(\alpha+\sqrt{2})}{2}\right)(\beta-\frac{\alpha+\sqrt{2}}{2}) + \\
~~~1-Q_1\left(\alpha,\frac{\alpha+\sqrt{2}}{2}\right), 
~~~~~~~~\mathrm{if}~\hat{c}_1 \leq\beta\leq \hat{c}_2 \\
1, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta> \hat{c}_2
\end{cases}
\end{align}
with $\hat{c}_1$ and $\hat{c}_2$ given in (\ref{eq_hatc1}) and (\ref{eq_hatc2}), respectively.
\end{corollary}
\begin{proof}
Using (\ref{eq_beta0}) for small values of $\alpha$, we have $x\simeq \frac{\alpha+\sqrt{2}}{2}$, which leads to 
\begin{equation}\label{eq_hatc1}
    \hat{c}_1 = \frac{-1+Q_1\left(\alpha,\frac{\alpha+\sqrt{2}}{2}\right)}{\left(\frac{\alpha+\sqrt{2}}{2} \right)^2 e^{-\frac{\alpha^2+\left(\frac{\alpha+\sqrt{2}}{2}\right)^2}{2}} I_0\left(\frac{\alpha(\alpha+\sqrt{2})}{2}\right)}+\alpha,
\end{equation}
and
\begin{equation}\label{eq_hatc2}
    \hat{c}_2 = \frac{Q_1\left(\alpha,\frac{\alpha+\sqrt{2}}{2}\right)}{\left(\frac{\alpha+\sqrt{2}}{2} \right)^2 e^{-\frac{\alpha^2+\left(\frac{\alpha+\sqrt{2}}{2}\right)^2}{2}} I_0\left(\frac{\alpha(\alpha+\sqrt{2})}{2}\right)}+\alpha,
\end{equation}
and simplifies (\ref{eq_lema1}) to (\ref{eq_coro2}).
\end{proof}



% \begin{corollary}\label{coro3}
% Equation (\ref{eq_coro1}) can be further simplified as
% \begin{align}\label{eq_coro3}
% \breve{\mathcal{Z}}(\alpha,\beta)\simeq
% \begin{cases}
% 0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \beta < \breve{c}_1  \\ 
% \frac{1}{\sqrt{2\pi}}(\beta-\alpha) + 
% \frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \breve{c}_1 \leq\beta\leq \breve{c}_2 \\
% 1, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta>\breve{c}_2
% \end{cases}
% \end{align}
% with $\breve{c}_1$ and $\breve{c}_2$ given by (\ref{eq_dotc1}) and (\ref{eq_dotc2}), respectively.
% \end{corollary}
% \begin{proof}
% For moderate/large values of $\alpha$, using the approximation $I_0(x) \simeq \frac{e^x}{\sqrt{2\pi x}}$ for (\ref{eq_coro1}) leads to (\ref{eq_coro3}) where
% \begin{align}\label{eq_dotc1}
%         \breve{c}_1 = -\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha,
% \end{align}
% and
% \begin{align}\label{eq_dotc2}
%      \breve{c}_2 = \sqrt{2\pi}-\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha.
% \end{align}
% \end{proof}














To illustrate these semi-linear approximations, Fig. \ref{fig_CDFilu} shows the CDF $y(\alpha,\beta)= 1-Q_1(\alpha,\beta)$ for both small and large values of $\alpha$, and compares the exact CDF with the approximation schemes of Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro2}. From Fig. \ref{fig_CDFilu}, we can observe that Lemma \ref{Lemma1} is tight for a broad range of $\alpha$  and moderate values of $\beta$. Moreover, the tightness is improved as $\alpha$ decreases. Also,  Corollaries \ref{coro1}-\ref{coro2} provide good approximations for large and small values of $\alpha$, respectively. Then, the proposed approximations are not tight at the tails of the CDF. However, as observed in \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,Makki2013TCfeedback,Makki2011Eurasipcapacity,Makki2018WCLwireless,Makki2016TVTperformance,Simon2003TWCsome,Suraweera2010TVTcapacity,Ma2000JSACunified,Digham2007TCenergy,Cao2016CLsolutions,sofotasios2015solutions,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan}  and in the following, in different applications,  the Marcum $Q$-function is normally combined with other functions which tend to zero of the tails of the CDF. In such cases, the inaccuracy of the approximation at the tails does not affect the tightness of the final result. 





\begin{figure}
\centering
  \includegraphics[width=1.0\columnwidth]{Figure1.pdf}\\
\caption{Illustration of the semi-linear approximation with Lemma \ref{Lemma1}, and Corollaries \ref{coro1}-\ref{coro2}. For each value of $\alpha\in[1,1.5,2]$, the approximated results obtained by Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro2} are compared with the exact value for a broad range of $\beta$.}
\label{fig_CDFilu}
\end{figure}








As an example, we first consider a general integral in the form of
\begin{align}\label{eq_integral}
G(\alpha,\rho)=\int_\rho^\infty{e^{-nx} x^m \left(1-Q_1(\alpha,x)\right)\text{d}x} ~~\forall n,m,\alpha,\rho>0.
\end{align}
Such an integral has been observed in various applications, e.g., in bit-error-probability evaluation of a Rayleigh fading channel \cite[eq. (1) (13)]{Simon2003TWCsome}, in energy detection of unknown signals over various multipath fading channels \cite[eq. (2)]{Cao2016CLsolutions}, in capacity analysis with channel inversion and fixed rate over correlated Nakagami fading \cite[eq. (1)]{sofotasios2015solutions}, in performance evaluation of  incoherent receivers in radar systems \cite[eq. (3)]{Cui2012ELtwo}, and in error probability analysis of diversity receivers \cite[eq. (1)]{Gaur2003TVTsome}. However, depending on the values of $n, m$ and $\rho$, (\ref{eq_integral}) may have no closed-form expression. Using Lemma \ref{Lemma1}, $G(\alpha,\rho)$ can be approximated in closed-form as presented in Lemma \ref{Lemma2}.

\begin{lem}\label{Lemma2}
The integral (\ref{eq_integral}) is approximately given by
\begin{align}
G(\alpha,\rho)\simeq
\begin{cases}
\Gamma(m+1,n\rho)n^{-m-1}, ~~~~~~~~~~~~~~~~~~\mathrm{if}~  \rho \geq \breve{c}_2  \\ 
\Gamma(m+1,n\breve{c}_2)n^{-m-1} + \\
~~\left(-\frac{\alpha}{\sqrt{2\pi}}+0.5*\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\times n^{-m-1}\times\\
~~\left(\Gamma(m+1,n\max(\breve{c}_1,\rho))-\Gamma(m+1,n\breve{c}_2)\right)+\\
~~\left(\Gamma(m+2,n\max(\breve{c}_1,\rho))-\Gamma(m+2,n\breve{c}_2)\right)\times\\
~~\frac{n^{-m-2}}{\sqrt{2\pi}},
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \rho<\breve{c}_2,
\end{cases}
\end{align}
where $\Gamma(s,x) = \int_{x}^{\infty} t^{s-1}e^{-t} \mathrm{d}t$ is the upper incomplete gamma function \cite[Eq. 6.5.1]{abramowitz1999ia}.
\end{lem}
\begin{proof}
See Appendix \ref{proof_Lemma2}. 
\end{proof}









As a second integration example of interest, consider
\begin{align}\label{eq_integralT}
    T(\alpha,m,a,\theta_1,\theta_2) = \int_{\theta_1}^{\theta_2} e^{-mx}\log(1+ax)Q_1(\alpha,x)\text{d}x \nonumber\\\forall m>0,a,\alpha,
\end{align}
with $\theta_2>\theta_1\geq0$, which does not have a closed-form expression for different values of $m, a, \alpha$. This type of integral is interesting as it could be used to analyze the expected performance of outage-limited systems, e.g,  the considered integral in the shape of \cite[eq. (1) (13)]{Simon2003TWCsome}, \cite[eq. (2)]{Cao2016CLsolutions}, \cite[eq. (3)]{Cui2012ELtwo}, and \cite[eq. (1)]{Gaur2003TVTsome}, applied in the analysis of the outage-limited throughput, i.e., when the outage-limited throughput $\log(1+ax)Q_1(\alpha,x)$  \cite[p. 2631]{Biglieri1998TITfading}\cite[Theorem 6]{Verdu1994TITgeneral}\cite[Eq. (9)]{Makki2014TCperformance} is averaged over fading statistics. Then, using Lemma \ref{Lemma1}, (\ref{eq_integralT}) can be approximated in closed-form as follows.

\begin{lem}\label{Lemma3}
The integral (\ref{eq_integralT}) is approximately given by
\begin{align}
  T(\alpha,m,a,\theta_1,\theta_2)\simeq~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\nonumber\\
\begin{cases}
\mathcal{F}_1(\theta_2)-\mathcal{F}_1(\theta_1), ~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  0\leq\theta_1<\theta_2 < c_1  \\ 
\mathcal{F}_1(c_1)-\mathcal{F}_1(\theta_1)+\mathcal{F}_2(\max(c_2,\theta_2))-\mathcal{F}_2(c_1),  \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1<c_1, \theta_2\geq c_1\\
 \mathcal{F}_2(\max(c_2,\theta_2))-\mathcal{F}_2(c_1), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1>c_1\\
0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1 > c_2,
\end{cases}  
\end{align}
where 
$c_1$ and $c_2$ are given by (\ref{eq_c1}) and (\ref{eq_c2}), respectively. Moreover,
\begin{align}\label{eq_F1}
    \mathcal{F}_1(x) \doteq \frac{1}{m}\left(-e^{\frac{m}{a}}\operatorname{E_1}\left(mx+\frac{m}{a}\right)-e^{-mx}\log(ax+1)\right),
\end{align}
and
\begin{align}\label{eq_F2}
    \mathcal{F}_2(x) \doteq &~ \mathrm{e}^{-mx}\Bigg(\left(mn_2-an_2-amn_1\right)\mathrm{e}^\frac{m\left(ax+1\right)}{a}\nonumber\\&~~ \operatorname{E_1}\left(\frac{m\left(ax+1\right)}{a}\right)-
    a\left(mn_2x+n_2+mn_1\right)\nonumber\\&~~\log\left(ax+1\right)-an_2\Bigg),
\end{align}
with
\begin{align}\label{eq_n1}
    n_1 = 1+\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}\times\nonumber\\
 I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)\times\frac{\alpha+\sqrt{\alpha^2+2}}{2}-\nonumber\\
 1+Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right),
\end{align}
and
\begin{align}\label{eq_n2}
    n_2 = -\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}\times\nonumber\\
 I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right).
\end{align}
In (\ref{eq_F1}) and (\ref{eq_F2}), $\operatorname{E_1}(x) = \int_x^{\infty} \frac{e^{-t}}{t} \mathrm{d}t$ is the Exponential Integral function \cite[p. 228, (5.1.1)]{abramowitz1999ia}.
\end{lem}

\begin{proof}
See Appendix \ref{proof_Lemma3}.
\end{proof}

Finally, setting $m = 0$ in (\ref{eq_integralT}), i.e.,
\begin{align}\label{eq_integralTs}
     T(\alpha,0,a,\theta_1,\theta_2) = \int_{\theta_1}^{\theta_2} \log(1+ax)Q_1(\alpha,x)\text{d}x,  \forall a,\alpha,
\end{align}
one can follow the same procedure in (\ref{eq_integralT}) to approximate (\ref{eq_integralTs}) as
\begin{align}\label{eq_integralTss}
  T(\alpha,0,a,\theta_1,\theta_2)\simeq~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\nonumber\\
\begin{cases}
\mathcal{F}_3(\theta_2)-\mathcal{F}_3(\theta_1), ~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  0\leq\theta_1<\theta_2 < c_1  \\ 
\mathcal{F}_3(c_1)-\mathcal{F}_3(\theta_1)+\mathcal{F}_4(\max(c_2,\theta_2))-\mathcal{F}_4(c_1),  \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1<c_1, \theta_2\geq c_1\\
 \mathcal{F}_4(\max(c_2,\theta_2))-\mathcal{F}_4(c_1), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1>c_1\\
0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1 > c_2,
\end{cases}  
\end{align}
with $c_1$ and $c_2$ given by (\ref{eq_c1}) and (\ref{eq_c2}), respectively. Also,
\begin{align}
    \mathcal{F}_3 = \frac{(ax+1)(\log(ax+1)-1)}{a},
\end{align}
and
\begin{align}
    \mathcal{F}_4 = \frac{n_2\left((2a^2x^2-2)\log(ax+1)-a^2x^2+2ax\right)}{4a^2}+\nonumber\\\frac{n_1(ax+1)(\log(ax+1)-1)}{a},
\end{align}
where $n_1$ and $n_2$ are given by (\ref{eq_n1}) and (\ref{eq_n2}), respectively.


\begin{figure}
\centering
  \includegraphics[width=1.0\columnwidth]{Figure2.pdf}\\
\caption{The  integral (\ref{eq_integral}) involving Marcum $Q$-function. Solid lines are exact values while crosses are the results obtained from Lemma \ref{Lemma2}, $\alpha = 2$,  $(m,n) = \{(4,4), (3,3), (2,2), (0,1), (1,1)\}$.}\label{fig_integrald}
\end{figure}


\begin{figure}
\centering
  \includegraphics[width=1.0\columnwidth]{Figure3.pdf}\\
\caption{The integral (\ref{eq_integralT}) involving the Marcum $Q$-function. Solid lines are exact values while crosses are the results obtained from Lemma \ref{Lemma3} and (\ref{eq_integralTss}). $\theta_1 = 0, \theta_2 = \infty$. }\label{fig_t2}
\end{figure}



In Figs. \ref{fig_integrald} and \ref{fig_t2}, we evaluate the tightness of the approximations in Lemmas \ref{Lemma2}, \ref{Lemma3} and (\ref{eq_integralTss}), for different values of $m$, $n$, $\rho$, $a$ and $\alpha$. From the figures, it can be observed that the approximation schemes of   Lemmas \ref{Lemma2}-\ref{Lemma3} and (\ref{eq_integralTss}) are very tight for different parameter settings, while our proposed semi-linear approximation makes it possible to represent the integrals in closed-form.  In this way, although the approximation (\ref{eq_lema1}) is not tight at the tails of the CDF, it gives tight approximation results when it appears in different integrals (Lemmas \ref{Lemma2}-\ref{Lemma3}) with the Marcum-$Q$ function  combined with other functions tending to zero at the tails of the function. Also, as we show in Section III, the semi-linear approximation scheme is efficient in optimization problems involving the Marcum $Q$-function. Finally, to tightly approximate the Marcum $Q$-function at the tails, which are the range of interest in, e.g., error probability analysis, one can use the approximation schemes of \cite{Simon2000TCexponential,annamalai2001WCMCcauchy}. 






\section{Applications in PA Systems}
In Section II, we showed how the proposed approximation scheme enables us to derive closed-form expressions for a broad range of integrals, as required in various expectation-based calculations, e.g., \cite{Simon2003TWCsome,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,Gaur2003TVTsome,Simon2000TCexponential,6911973}. On the other hand, the Marcum $Q$-function may also  appear in  optimization problems, e.g., \cite[eq. (8)]{Azari2018TCultra},\cite[eq. (9)]{Alam2014INFOCOMWrobust}, \cite[eq. (10)]{Gao2018IAadmm}, \cite[eq. (10)]{Shen2018TVToutage}, \cite[eq. (15)]{Song2017JLTimpact}, \cite[eq. (22)]{Tang2019IAan}.  For this reason, in this section, we provide an example of using our proposed semi-linear approximation in an optimization problem for the PA systems.

\subsection{Problem Formulation}
Vehicle communication is one of the most important use cases in 5G.  Here, the main focus is to provide efficient and reliable connections to cars and public transports, e.g., busses and trains. CSIT plays an important role in achieving these goals, since the data transmission efficiency can be improved by updating the transmission parameters relative to the instantaneous channel state.  However, the typical CSIT acquisition systems, which are mostly designed for (semi)static channels, may not work well for high-speed vehicles. This is because, depending on the vehicle speed, the position of the antennas may change quickly and the channel information becomes inaccurate.  To overcome this issue, \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing} propose the PA setup as shown in Fig. \ref{system}. With a PA setup, which is of interesting in Vehicle-to-everything (V2X) communications \cite{Sternad2012WCNCWusing} as well as integrated access and backhauling \cite{Teyeb2019VTCintegrated}, two antennas are deployed on the top of the vehicle. The first antenna,  the PA,  estimates the channel and sends feedback to the BS at time $t$. Then, the BS uses the CSIT provided by the PA to communicate with a second antenna, which we refer to as RA, at time $t+\delta$, where $\delta$ is the processing time at the BS. In this way, the BS can use the CSIT acquired from the PA and perform various CSIT-based transmission schemes, e.g.,  \cite{Sternad2012WCNCWusing,BJ2017ICCWusing}.  


\begin{figure}
%\vspace{-3mm}
\centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=1.0\columnwidth]{Figure4.pdf}\\
 %\vspace{-4mm}
\caption{A PA system with the mismatch problem. Here, $\hat h$ is the channel between the BS and the PA while $h$ refers to the BS-RA link. The vehicle is moving with speed $v$ and the antenna separation is $d_\text{a}$. The red arrow indicates the spatial mismatch, i.e., when the RA does not reach at the same  point as the PA when sending pilots. Also, $d_\text{m}$ is the moving distance of the vehicle which is affected by the processing delay $\delta$ of the BS. }\label{system}
\end{figure}


We assume that the vehicle moves through a stationary electromagnetic standing wave pattern \footnote{This has been experimentally verified in, e.g., \cite{Jamaly2014EuCAP}}. Thus, if the RA reaches exactly the same position as the position of the PA when sending the pilots, it will experience the same channel and the CSIT will be perfect. However, if the RA does not reach the same spatial point as the PA, due to, e.g., the BS processing delay is not equal to the time that we need until the RA reaches the same point as the PA, the RA may receive the data in a place different from the one in which the PA was sending the pilots. Such spatial mismatch may lead to CSIT inaccuracy, which will affect the system performance considerably. Thus, we need adaptive schemes to compensate for it.

Considering downlink transmission in the BS-RA link, the received signal is given by
\begin{align}\label{eq_Y}
{{Y}} = \sqrt{P}hX + Z.
\end{align}
Here, $P$ represents the transmit power, $X$ is the input message with unit variance, and $h$ is the fading coefficient between the BS and the RA. Also, $Z \sim \mathcal{CN}(0,1)$ denotes the independent and identically distributed (IID) complex Gaussian noise added at the receiver.



We denote the channel coefficient of the PA-BS uplink as $\hat{h}$. Also, we define $d$ as the effective distance between  the place where the PA estimates the channel at time $t$, and the place where the RA reaches at time $t+\delta$. As can be seen in Fig. \ref{system}, $d$ can be calculated as
\begin{align}\label{eq_d}
    d = |d_\text{a} - d_\text{m} | = |d_\text{a} - v\delta|,
\end{align}
where $d_\text{m}$ is the moving distance of the vehicle during time interval $\delta$, and $v$ is the velocity of the vehicle. Also, $d_\text{a}$ is the antenna separation between the PA and the RA. In conjunction to (\ref{eq_d}), here, we assume $d$ can be calculated by the BS. 

Using the classical Jake's correlation model \cite[p. 2642]{Shin2003TITcapacity} and  assuming a semi-static propagation environment, i.e., assuming that the coherence time of the propagation environment is larger than $\delta$,  the channel coefficient of the BS-RA downlink can be modeled as 
\begin{align}\label{eq_H}
    h = \sqrt{1-\sigma^2} \hat{h} + \sigma q.
\end{align}
Here, $q \sim \mathcal{CN}(0,1)$ which is independent of the known channel value $\hat{h}\sim \mathcal{CN}(0,1)$, and $\sigma$ is a function of the effective distance $d$ as 
\begin{align}
    \sigma = \frac{\frac{\phi_2^2-\phi_1^2}{\phi_1}}{\sqrt{ \left(\frac{\phi_2}{\phi_1}\right)^2 + \left(\frac{\phi_2^2-\phi_1^2}{\phi_1}\right)^2 }} = \frac{\phi_2^2-\phi_1^2}{\sqrt{ \left(\phi_2\right)^2 + \left(\phi_2^2-\phi_1^2\right)^2 }} .
\end{align}
Here, $\phi_1 = \bm{\Phi}_{1,1}^{1/2} $ and $\phi_2 = \bm{\Phi}_{1,2}^{1/2} $, where $\bm{\Phi}$ is  from Jake's model \cite[p. 2642]{Shin2003TITcapacity}
\begin{align}\label{eq_tildeH}
     \bigl[ \begin{smallmatrix}
  \hat{h}\\h
\end{smallmatrix} \bigr]= \bm{\Phi}^{1/2} \bm{H}_{\varepsilon}.
\end{align}
Note that, the channel model (\ref{eq_H}) has been experimentally verified in, e.g., \cite{Jamaly2014EuCAP} for PA setups. Also, one can follow the same method as in \cite{Guo2019WCLrate} to extend the model to the cases with temporally-correlated channels. Moreover, in (\ref{eq_tildeH}), $\bm{H}_{\varepsilon}$ has independent circularly-symmetric zero-mean complex Gaussian entries with unit variance, and $\bm{\Phi}$ is the channel correlation matrix with the $(i,j)$-th entry given by
\begin{align}\label{eq_phi}
    \Phi_{i,j} = J_0\left((i-j)\cdot2\pi d/ \lambda\right) \forall i,j.
\end{align}
Here, $J_n(x) = (\frac{x}{2})^n \sum_{i=0}^{\infty}\frac{(\frac{x}{2})^{2i}(-1)^{i} }{i!\Gamma(n+i+1)}$ represents the $n$-th order Bessel function of the first kind. Moreover, $\lambda$ denotes the carrier wavelength, i.e., $\lambda = c/f_\text{c}$ where $c$ is the speed of light and $f_\text{c}$ is the carrier frequency. 






From (\ref{eq_H}), for a given $\hat{h}$ and $\sigma \neq 0$, $|h|$ follows a Rician distribution, i.e., the  probability density function (PDF) of $|h|$ is given by 
\begin{align}
    f_{|h|\big|\hat{g}}(x) = \frac{2x}{\sigma^2}e^{-\frac{x^2+\hat{g}}{\sigma^2}}I_0\left(\frac{2x\sqrt{\hat{g}}}{\sigma^2}\right),
\end{align}
where $\hat{g} = (1-\sigma^2)|\hat{h}|^2$. Let us define the channel gain between BS-RA as $ g = |{h}|^2$. Then, the PDF of $f_{g|\hat{g}}$ is given by

\begin{align}\label{eq_pdf}
    f_{g|\hat{g}}(x) = \frac{1}{\sigma^2}e^{-\frac{x+\hat{g}}{\sigma^2}}I_0\left(\frac{2\sqrt{x\hat{g}}}{\sigma^2}\right),
\end{align}
which is non-central Chi-squared distributed with the CDF containing the first-order Marcum $Q$-function as
\begin{align}\label{eq_cdf}
    F_{g|\hat{g}}(x) = 1 - Q_1\left( \sqrt{\frac{2\hat{g}}{\sigma^2}}, \sqrt{\frac{2x}{\sigma^2}}  \right).
\end{align}



\subsection{Analytical Results on Rate Adaptation Using the Semi-Linear Approximation of the First-order Marcum $Q$-Function}\label{In Section III.C,}
We assume that $d_\text{a}$, $\delta $ and $\hat{g}$ are known by the BS. It can be seen from (\ref{eq_pdf}) that $f_{g|\hat{g}}(x)$ is a function of $v$. For a given $v$, the distribution of $g$ is known by the BS, and a rate adaption scheme can be performed to improve the system performance.

For a given instantaneous value of $\hat g$, the data is transmitted with instantaneous rate $R_{|\hat{g}}$ nats-per-channel-use (npcu). If the instantaneous channel gain realization supports the transmitted data rate $R_{|\hat{g}}$, i.e., $\log(1+gP)\ge R_{|\hat{g}}$, the data can be successfully decoded. Otherwise,  outage occurs. Hence, the outage probability in each time slot is
\begin{align}
    \Pr(\text{outage}|\hat{g}) = F_{g|\hat{g}}\left(\frac{e^{R_{|\hat{g}}}-1}{P}\right).
\end{align}
Also, the instantaneous throughput for a given $\hat{g}$ is
\begin{align}\label{eq_opteta}
\eta_{|\hat {g}}\left(R_{|\hat{g}}\right)=R_{|\hat{g}}\left(1-\Pr\left(\log(1+gP)<R_{|\hat{g}}\right)\right),
\end{align}
and the optimal rate adaptation maximizing the  instantaneous throughput is obtained by
\begin{align}\label{eq_optR}
    R_{|\hat{g}}^{\text{opt}}&=\argmax_{R_{|\hat{g}}\geq 0} \left\{ \left(1-\Pr\left(\log(1+gP)<R_{|\hat{g}}\right)\right)R_{|\hat{g}} \right\}\nonumber\\
    &=\argmax_{R_{|\hat{g}}\geq 0} \left\{ \left(1-F_{g|\hat{g}}\left(\frac{e^{R_{|\hat{g}}}-1}{P}\right)\right) R_{|\hat{g}}\right\}\nonumber\\
    &=\argmax_{R_{|\hat{g}}\geq 0} \left\{ Q_1\left(  \sqrt{\frac{2\hat{g}}{\sigma^2}}, \sqrt{\frac{2(e^{R_{|\hat{g}}}-1)}{P\sigma^2}} \right)R_{|\hat{g}} \right\},
\end{align}
where the last equality comes from (\ref{eq_cdf}). 

Using the derivatives of the Marcum $Q$-function, (\ref{eq_optR}) does not have a closed-form solution\footnote{To solve (\ref{eq_optR}), one can use different approximation methods of the Marcum $Q$-function, e.g., \cite{Guo2019WCLrate}. Here, we use Lemma \ref{Lemma1}/Corollaries \ref{coro1}-\ref{coro2} to solve (\ref{eq_optR}) to show the usefulness of the semi-linear approximation method. As shown, in Figs. \ref{fig_Figure5} and \ref{fig_Figure6}, the semi-linear approximation is tight for a broad range of parameter settings while it simplifies the optimization problem considerably. }. For this reason,  Lemma \ref{Lemma4}  uses the semi-linear approximation scheme of Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro2} to find the optimal data rate maximizing the instantaneous throughput.

\begin{lem}\label{Lemma4}
For a given channel realization $\hat{g}$, the throughput-optimized rate allocation is approximately given by (\ref{eq_appRF}) where $\mathcal{W}(\cdot)$ denotes the Lambert $\mathcal{W}$-function.
\end{lem}
\begin{proof}
The  approximation results of Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro2} can be generalized by $y(\alpha,\beta)\simeq\tilde{\mathcal{Z}}_{\text{general}}(\alpha,\beta)$ where
\begin{align}
\tilde{\mathcal{Z}}_{\text{general}}(\alpha,\beta)\simeq
\begin{cases}
0,~~~~~~~~~~~~~~~~~~~~\mathrm{if}~\beta < c_1(\alpha)  \\ 
o_1(\alpha)(\beta-o_2(\alpha)) + o_3,\\~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ c_1(\alpha) \leq \beta \leq c_2(\alpha)\\ 
1,~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta> c_2(\alpha).
\end{cases}
\end{align}


$o_i,i=1,2,3$, are given by (\ref{eq_lema1}), (\ref{eq_coro1}), or (\ref{eq_coro2}) depending on if we use Lemma \ref{Lemma1} or Corollaries \ref{coro1}-\ref{coro2}. In this way, (\ref{eq_opteta}) is approximated as
\begin{align}\label{eq_appR}
    \eta_{|\hat {g}}\simeq R_{|\hat{g}}\left(1-o_1(\alpha)\beta + o_1(\alpha)o_2(\alpha) - o_3(\alpha)\right),
\end{align}
where $\alpha = \sqrt{\frac{2\hat{g}}{\sigma^2}}$. To simplify the equation, we omit $\alpha$ in the following since it is a constant for given $\hat{g}$, $\sigma$. Then, setting the derivative of (\ref{eq_appR}) equal to zero, we obtain
\begin{align}\label{eq_appRF}
    & R_{|\hat{g}}^{\text{opt}}  \nonumber\\
    & = \operatorname*{arg}_{R_{|\hat{g}}\geq 0}\left\{ 1+o_1o_2-o_3-o_1\left(\frac{(R_{|\hat{g}}+2)e^{R_{|\hat{g}}}-2}{\sqrt{2P\sigma^2\left(e^{R_{|\hat{g}}}-1\right)}}\right)=0\right\}\nonumber\\
    % & = \operatorname*{arg}_{R_{|\hat{g}}\geq 0} \left\{ \left(\frac{(R_{|\hat{g}}+2)e^{R_{|\hat{g}}}-2}{\sqrt{2P\sigma^2\left(e^{R_{|\hat{g}}}-1\right)}}\right) = \frac{1+o_1o_2-o_3}{o_1}\right\}\nonumber\\
    & \overset{(b)}{\simeq} \operatorname*{arg}_{R_{|\hat{g}}\geq 0}\left\{ \left(\frac{R_{|\hat{g}}}{2}+1\right)e^{\frac{R_{|\hat{g}}}{2}+1} = \frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}\right\}\nonumber\\
    & \overset{(c)}{=} 2\mathcal{W}\left(\frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}-1\right).
\end{align}
Here,  $(b)$ comes from $e^{R_{|\hat{g}}}-1 \simeq e^{R_{|\hat{g}}} $ and $(R_{|\hat{g}}+2)e^{R_{|\hat{g}}}-2 \simeq (R_{|\hat{g}}+2)e^{R_{|\hat{g}}} $ which are appropriate at moderate/high values of $R_{|\hat{g}}$. Also, $(c)$ is obtained by the definition of the Lambert $\mathcal{W}$-function $xe^x = y \Leftrightarrow x = \mathcal{W}(y)$ \cite{corless1996lambertw}. 

\end{proof}

Finally, the expected throughput, averaged over multiple time slots, is obtained by $\eta = \mathbb{E}\left\{\eta|{\hat {g}}(R_{|\hat{g}}^{\text{opt}})\right\}$ with expectation over $\hat g$.  

Using (\ref{eq_appRF}) and the approximation \cite[Them. 2.1]{hoorfar2007approximation}
\begin{align}
    \mathcal{W}(x) \simeq \log(x)-\log\log(x), x\geq0,
\end{align}
we obtain
\begin{align}
    R_{|\hat{g}}^{\text{opt}}\simeq 2\log\left(\frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}-1\right)-\nonumber\\
    2\log\log\left(\frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}-1\right)
\end{align}
which implies as the transmit power increases, the optimal instantaneous rate increases with the square root of the transmit power (approximately) logarithmically.

\subsection{On the Effect of Imperfect Channel Estimation}
In Section \ref{In Section III.C,}, we assumed perfect channel estimation at the BS. The deviations of channel estimation, due to, e.g., radio-frequency mismatch, could invalidate the assumption of perfect channel estimation, and should be considered in the system design. Here, we follow the similar approach as in, e.g., \cite{Wang2007TWCperformance}, to add the effect of estimation error of $\hat{h}$ as an independent additive Gaussian variable whose variance is given by the accuracy of channel estimation. 

Let us define $\tilde h$ as the estimate of $\hat h$ at the BS. Then,  we further develop our channel model  (\ref{eq_H}) as
\begin{align}\label{eq_Htp}
    \tilde{h} = \kappa \hat{h} + \sqrt{1-\kappa^2} z, 
\end{align}
for each time slot, where $z \sim \mathcal{CN}(0,1)$ is a Gaussian noise which is uncorrelated with $H_{k}$. Also, $\kappa$ is a known correlation factor which represents the estimation error of $\hat{h}$ by $\kappa = \frac{\mathbb{E}\{\tilde{h}\hat{h}^*\}}{\mathbb{E}\{|\hat{h}|^2\}}$. Substituting (\ref{eq_Htp}) into (\ref{eq_H}), we have
\begin{align}\label{eq_Ht}
    h = \kappa\sqrt{1-\sigma^2}\hat{h}+\kappa\sigma q+\sqrt{1-\kappa^2}z.
\end{align}
Then, because  $\kappa\sigma q + \sqrt{1-\kappa^2}z$ is equivalent to a new Gaussian variable $w \sim\mathcal{CN}\left(0,(\kappa\sigma)^2+1-\kappa^2\right)$, we can follow the same procedure as in (\ref{eq_optR})-(\ref{eq_appRF}) to analyze the system performance with imperfect channel estimation of the PA (see Figs. \ref{fig_Figure5}-\ref{fig_Figure6} for more discussions).

\subsection{Simulation Results}
In this part, we study the performance of the PA system and verify the tightness of the approximation scheme of Lemma \ref{Lemma4}. Particularly, we present the average throughput and the outage probability of the PA setup for different vehicle speeds/channel estimation errors. As an ultimate upper bound for the proposed rate adaptation scheme, we consider a genie-aided setup where we assume that the BS has perfect CSIT of the BS-RA link without uncertainty/outage probability. Then, as a lower-bound of the system performance, we consider the cases with no CSIT/rate adaptation as shown in Fig. \ref{fig_Figure5}. Here, the simulation results for the cases of no adaptation are obtained with only one antenna and no CSIT. In this case,  the data is sent with a fixed rate $R$ and it is decoded if $R<\log(1+gP)$, i.e., $g>\frac{e^{R}-1}{P}$. In this way, assuming Rayleigh fading, the average rate is given by
\begin{align}\label{eq_bench}
    R^{\text{No-adaptation}} = \int_{\frac{e^{R}-1}{P}}^{\infty} Re^{-x} \text{d}x = Re^{-\frac{e^{R}-1}{P}},
\end{align}
and the optimal rate allocation is found by setting the derivative of (\ref{eq_bench}) with respect to $R$ equal to zero leading to $\tilde{R} = \mathcal{W}(P)$, and the throughput is calculated as 
\begin{align}\label{eq_etanocsi}
  \eta^{\text{No-adaptation}} =\mathcal{W}(P)e^{-\frac{e^{\mathcal{W}(P)}-1}{P}}.  
\end{align}
Also, in the simulations, we set  $f_\text{c}$ = 2.68 GHz and $d_\text{a} = 1.5\lambda$. Finally, each point in the figures is obtained by averaging the system performance over $1\times10^5$ channel realizations.

In Fig. \ref{fig_Figure5}, we show the expected throughput $\eta$  in different cases for a broad range of signal-to-noise ratios (SNRs). Here, because the noise has unit variance, we define the SNR as $10\log_{10}P$. Also, we set $v = 114$ km/h in Fig. \ref{fig_Figure5}  as defined in (\ref{eq_d}), and $\kappa = 1$ as discussed in (\ref{eq_Ht}). The analytical results obtained by Lemma \ref{Lemma4} and Corollary \ref{coro2}, i.e., the approximation of (\ref{eq_optR}), are also presented. We have also checked the approximation result of Lemma \ref{Lemma4} while using Lemma \ref{Lemma1}/Corollary \ref{coro1}. Then, because the results are similar as those presented in Fig. \ref{fig_Figure5}, they are not included in the figure. Moreover, the figure shows the results of (\ref{eq_etanocsi}) with no CSIT/rate adaptation as a benchmark. Finally, Fig. \ref{fig_Figure6} studies the expected throughput $\eta$ for different values of estimation error variance $\kappa$ with SNR = 10, 19, 25 dB, in the case of partial CSIT. Also, the figure evaluates the tightness of the approximation results obtained by Lemma \ref{Lemma4}. Here,  we set $v =$ 114.5 km/h and $\delta = 5$ ms.

Setting SNR = 23 dB and $v = $ 120, 150 km/h in Fig. \ref{fig_Figure7},  we study the effect of the processing delay $\delta$ on the throughput. Finally, the outage probability is evaluated in Fig. \ref{fig_Figure8}, where the results are presented for different speeds with SNR = 10 dB, in the case of partial CSIT. Also, we present  the outage probability for $\delta = 5.35$ ms and $\delta = 4.68$ ms in Fig.  \ref{fig_Figure8}. 


\begin{figure}
\centering
  \includegraphics[width=1.0\columnwidth]{Figure5.pdf}\\
\caption{Expected throughput $\eta$ in different cases, $v$ = 114 km/h, $\kappa$ = 1, and $\delta = $ 5 ms. Both the exact values estimated from  simulations as well as the analytical approximations from Lemma \ref{Lemma4} are presented.}\label{fig_Figure5}
\end{figure}

\begin{figure}
%\vspace{-3mm}
\centering
  \includegraphics[width=1.0\columnwidth]{Figure6.pdf}\\
 %\vspace{-4mm}
\caption{Expected throughput $\eta$ for different estimation errors $\kappa$ with SNR = 10, 19, 25 dB, in the case of partial CSIT, exact and approximation,  $v = $  114.5 km/h, and $\delta = 5$ ms. Both the exact values estimated from simulations as well as the analytical approximations from Lemma \ref{Lemma4} are presented.}\label{fig_Figure6}
\end{figure}


\begin{figure}
\centering
  \includegraphics[width=1.0\columnwidth]{Figure7.pdf}\\
\caption{Expected throughput $\eta$ for different processing delays with SNR = 23 dB and $v$ = 120, 150 km/h in the case of partial adaptation. }\label{fig_Figure7}

\end{figure}

\begin{figure}
%\vspace{-3mm}
\centering
  \includegraphics[width=1.0\columnwidth]{Figure8.pdf}\\
 %\vspace{-4mm}
\caption{Outage probability for different velocities with SNR = 10 dB, in the case of partial CSIT.}\label{fig_Figure8}

\end{figure}




From the figures, we can conclude the following points:
\begin{itemize}
    \item The approximation scheme of Lemma \ref{Lemma4} is tight for a broad range of parameter settings (Figs. \ref{fig_Figure5}, \ref{fig_Figure6}). Thus, the throughput-optimized rate allocation can be well approximated by (\ref{eq_appRF}), and the semi-linear approximation of Lemma \ref{Lemma1}/Corollaries \ref{coro1}-\ref{coro2} is a good approach to study the considered optimization problem.
    
    \item With deployment of the PA, remarkable throughput gain is achieved especially in moderate/high SNRs (Fig. \ref{fig_Figure5}). Also, the throughput decreases when the estimation error is considered, i.e., $\kappa$ decreases. Finally, as can be seen in Figs.  \ref{fig_Figure5}, \ref{fig_Figure6}, with rate adaptation,  and without optimizing the processing delay/vehicle speed, the effect of estimation error on expected throughput  is small unless for large values of $\kappa$.

    
    \item As it can be seen in Figs. \ref{fig_Figure7} and \ref{fig_Figure8}, for different channel estimation errors, there are optimal values for the vehicle speed and the BS processing delay optimizing the system throughput and outage probability. Note that the presence of the optimal speed/processing delay can be proved via (\ref{eq_d}) as well. Finally, the optimal value of the vehicle speed, in terms of throughput/outage probability, decreases with the processing delay. However, the optimal vehicle speed/processing delay, in terms of throughput/outage probability, is almost insensitive to the channel estimation error.

    \item With perfect channel estimation, the throughput/outage probability is sensitive to the speed variation, if we move away from the optimal speed (Figs. \ref{fig_Figure7} and \ref{fig_Figure8}). However, the sensitivity to the speed/processing delay variation decreases as the channel estimation error increases, i.e., $\kappa$ decreases (Figs. \ref{fig_Figure7} and \ref{fig_Figure8}). Finally, considering Figs. \ref{fig_Figure7} and \ref{fig_Figure8}, it is expected that adapting the processing delay, as a function of the vehicle speed, and implementing hybrid automatic repeat request protocols can improve the performance of the PA system. These points will be studied in our future works.

\end{itemize}





\section{Conclusion}
We derived a simple semi-linear approximation method for the first-order Marcum $Q$-function, as one of the functions of interest in different problem formulations of wireless networks. As we showed through various analysis, while the proposed approximation is not tight at the tails of the function, it is useful in different optimization- and expectation-based problem formulations. Particularly, as an application of interest, we used the proposed approximation to analyze the performance of PA setups using  rate adaptation. As we showed, with different levels of channel estimation error/processing delay, adaptive rate allocation can effectively compensate for the spatial mismatch problem, and improve the throughput/outage probability of PA networks.  It is expected that increasing the number of RA antennas will improve the performance of the PA system considerably. 







% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/




\appendices
\section{Proof of Lemma \ref{Lemma2}}
  \label{proof_Lemma2}
Using Corollary \ref{coro1},  we have
\begin{align}
G(\alpha,\rho)\simeq
\begin{cases}
\int_\rho^{\breve{c}_1}0\text{d}x + \int_{\breve{c}_1}^{\breve{c}_2}e^{-nx}x^{m}\times\nonumber\\
~~~\left(\frac{1}{\sqrt{2\pi}}(x-\alpha) + \frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\text{d}x +\nonumber\\
~~~\int_{\breve{c}_2}^{\infty}e^{-nx}x^{m}\text{d}x, ~~~~~~~~~~~~~~\mathrm{if}~  \rho < \breve{c}_1  \\ 
 \int_{\rho}^{\breve{c}_2}e^{-nx}x^{m}\times\nonumber\\
~~~\left(\frac{1}{\sqrt{2\pi}}(x-\alpha) + \frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\text{d}x +\nonumber\\
~~~\int_{\breve{c}_2}^{\infty}e^{-nx}x^{m}\text{d}x, ~~~~~~~~~~~~~~\mathrm{if}~  \breve{c}_1\leq\rho<\breve{c}_2,\nonumber\\
\int_\rho^{\infty} e^{-nx}x^{m}\text{d}x, ~~~~~~~~~~~~~~~~~~\mathrm{if}~  \rho\geq\breve{c}_2.
\end{cases}
\end{align}


Then, for $\rho\geq \breve{c}_2$, we obtain
\begin{align}
&    \int_\rho^\infty e^{-nx}\times x^{m}(1-Q_1(\alpha,x))\text{d}x\nonumber\\
  &  \overset{(d)}\simeq\int_\rho^\infty e^{-nx}\times x^{m}\text{d}x
   \overset{(e)}= \Gamma(m+1,n\rho)n^{-m-1}, 
\end{align}
while for $\rho<\breve{c}_2$, we have

\begin{align}
 &  \int_\rho^\infty e^{-nx}\times x^{m}(1-Q_1(\alpha,x))\text{d}x\nonumber\\
&    \overset{(f)}\simeq \int_{\max(\breve{c}_1,\rho)}^{\breve{c}_2} \left(\frac{1}{\sqrt{2\pi}}(x-\alpha) + 
\frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\times\nonumber\\
& ~~~~~~e^{-nx}x^{m}\text{d}x +\int_{\breve{c}_2}^\infty e^{-nx} x^{m}\text{d}x\nonumber\\
& \overset{(g)}= \Gamma(m+1,n\breve{c}_2)n^{-m-1} + \nonumber\\
&~~~~~~\left(-\frac{\alpha}{\sqrt{2\pi}}+0.5*\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\times n^{-m-1}\times\nonumber\\
&~~~~~~\left(\Gamma\left(m+1,n\max(\breve{c}_1,\rho)\right)-\Gamma\left(m+1,n\breve{c}_2\right)\right)+\nonumber\\
&~~~~~~\left(\Gamma(m+2,n\max(\breve{c}_1,\rho))-\Gamma(m+2,n\breve{c}_2)\right)\frac{n^{-m-2}}{\sqrt{2\pi}}.
\end{align}
Note that $(d)$ and $(f)$ come from Corollary \ref{coro1} while $(e)$ and $(g)$ use the fact that $\Gamma(s,x)\rightarrow 0$ as $x\rightarrow\infty$.


\section{Proof of Lemma \ref{Lemma3}}
\label{proof_Lemma3}
Using Lemma \ref{Lemma1}, the  integral (\ref{eq_integralT})  can be approximated as

1) for $\theta_2>\theta_1>c_2$, $T(\alpha,m,a,\theta_1,\theta_2) \simeq 0$,

2) for $c_1<\theta_1\leq c_2, \theta_2>\theta_1$,
\begin{align}
  &  T(\alpha,m,a,\theta_1,\theta_2) = \nonumber\\& ~~\int_{\theta_1}^{\min(c_2,\theta_2)} (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x,
\end{align}

3) for $\theta_1<c_1,\theta_2>c_1$,
\begin{align}
   & T(\alpha,m,a,\theta_1,\theta_2) \simeq \int_{\theta_1}^{c_1} e^{-mx}\log(1+ax)\text{d}x + \nonumber\\
   &~~ \int_{c_1}^{\min(c_2,\theta_2)} (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x,
\end{align}

4) for $\theta_1<\theta_2<c_1$,
\begin{align}
   & T(\alpha,m,a,\theta_1,\theta_2) \simeq \int_{\theta_1}^{\theta_2} e^{-mx}\log(1+ax)\text{d}x.
\end{align}

Then, consider case 3 where
\begin{align}
    T(\alpha,m,a,\theta_1,\theta_2) &= \int_{\theta_1}^{\theta_2} e^{-mx}\log(1+ax)Q_1(\alpha,x)\text{d}x\nonumber\\
    &\simeq \int_{\theta_1}^{c_1} e^{-mx}\log(1+ax)\text{d}x + \nonumber\\
   & \int_{c_1}^{\theta_2} (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x\nonumber\\
   & =  \mathcal{F}_1(c_1) -  \mathcal{F}_1(\theta_1) +  \mathcal{F}_2(\theta_2) -  \mathcal{F}_2(c_1),
\end{align}
with $n_1$ and $n_2$ being functions of the constant $\alpha$ and given by (\ref{eq_n1}) and (\ref{eq_n2}), respectively. Here, we assume $\theta_1<c_1$ and $c_2> \theta_2 > c_1$ for simplicity. The other cases can be proved with the same procedure. Moreover, the functions $\mathcal{F}_1(x)$ and $\mathcal{F}_2(x)$ are obtained by
\begin{align}
    \mathcal{F}_1(x) &= \int e^{-mx}\log(1+ax)\text{d}x\nonumber\\
    &\overset{(h)}= -\frac{e^{-mx}\log(ax+1)}{m}-\int -\frac{ae^{-mx}}{m(ax+1)} \text{d}x\nonumber\\
    & \overset{(i)}=  \frac{1}{m}\left(-e^{\frac{m}{a}}\operatorname{E_1}\left(mx+\frac{m}{a}\right)-e^{-mx}\log(ax+1)\right)+C,
\end{align}
and
\begin{align}
     \mathcal{F}_2(x)& =  \int (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x\nonumber\\
    &\overset{(j)} = -\frac{(mn_2x+n_2+mn_1)e^{-mx}\log(1+ax)}{m^2} - \nonumber\\
    &~~~\int \frac{a(-mn_2x-n2-mn_1)e^{-mx}}{m^2(ax+1)} \text{d}x\nonumber\\
    & \overset{(k)}= -\frac{(mn_2x+n_2+mn_1)e^{-mx}\log(1+ax)}{m^2} - \nonumber\\
    &~~~ -\frac{1}{a}\bigg(e^{\frac{m}{a}}(mn_2x+n_2+mn_1)\nonumber\\
    &~~~ \operatorname{E_1}\left(mx+\frac{m}{a}\right)\bigg)+
    \int - \frac{me^{\frac{m}{a}}n_2}{\operatorname{E_1}\left(mx+\frac{m}{a}\right)} \text{d}x\nonumber\\
    & \overset{(l)}= -\frac{(mn_2x+n_2+mn_1)e^{-mx}\log(1+ax)}{m^2} - \nonumber\\
    &~~~ -\frac{1}{a}\bigg(e^{\frac{m}{a}}(mn_2x+n_2+mn_1) \operatorname{E_1}\left(mx+\frac{m}{a}\right)\bigg)+\nonumber\\
    &~~~  \frac{n_2e^{-mx}}{a} - \frac{e^{\frac{m}{a}}n_2(mx+\frac{m}{a}) \operatorname{E_1}\left(mx+\frac{m}{a}\right)}{a}+C,
\end{align}
where $(h)$, $(j)$ and $(k)$ come from partial integration and some manipulations. Also, $(i)$ and $(l)$ use \cite[p. 195]{geller1969table}
\begin{align}
    \int \operatorname{E_1}(u) \text{d}u = u\operatorname{E_1}(u)-e^{-u}.
\end{align}










==> YourThesis/papers/T1/content.tex <==
\begin{abstract}
First-order Marcum $Q$-function is observed in various problem formulations. However, it is not an easy-to-handle function. For this reason, in this paper, we first present a semi-linear approximation of the Marcum $Q$-function. Our proposed approximation is useful because it simplifies, e.g., various integral calculations including the Marcum $Q$-function as well as different operations such as parameter optimization. Then, as an example of interest, we apply our proposed approximation approach to the performance analysis of predictor antenna (PA) systems. Here, the PA system is referred to as a system with two sets of antennas on the roof of a vehicle. Then, the PA positioned in the front of the vehicle can be used to improve the channel state estimation for data transmission of the receive antenna  that is aligned behind the PA. Considering spatial mismatch due to the mobility, we derive closed-form expressions for the instantaneous and average throughput as well as the throughput-optimized rate allocation. As we show, our proposed approximation scheme enables us to analyze PA systems with high accuracy. Moreover, our results show that rate adaptation can improve the performance of PA systems with different levels of spatial mismatch.
\end{abstract}
\keywords{Backhaul, channel state information (CSI),  integrated access and backhaul (IAB), linear approximation, Marcum $Q$-function, mobility, mobile relay, outage probability, predictor antenna, rate adaptation, spatial correlation, throughput.}


\section{Introduction}

The first-order Marcum $Q$-function\footnote{To simplify the analysis, our paper concentrates on the approximation of the first-order Marcum-$Q$ function. However, our approximation technique can be easily extended to the cases with different orders of Marcum $Q$-function.} is defined as  \cite[Eq. (1)]{Bocus2013CLapproximation}
\begin{align}
    Q_1(\alpha,\beta) = \int_{\beta}^{\infty} xe^{-\frac{x^2+\alpha^2}{2}}I_0(x\alpha)\text{d}x,
\end{align}
where $\alpha, \beta \geq 0$ and $I_n(x) = (\frac{x}{2})^n \sum_{i=0}^{\infty}\frac{(\frac{x}{2})^{2i} }{i!\Gamma(n+i+1)}$ is the $n$-order modified Bessel function of the first kind, and $\Gamma(z) = \int_0^{\infty} x^{z-1}e^{-x} \mathrm{d}x$ represents the Gamma function. Reviewing the literature,  the Marcum $Q$-function has appeared in many areas such as statistics/signal detection \cite{helstrom1994elements}, and in the performance analysis of different setups such as temporally correlated channels \cite{Makki2013TCfeedback}, spatially correlated channels \cite{Makki2011Eurasipcapacity},  free-space optical (FSO) links \cite{Makki2018WCLwireless}, relay networks \cite{Makki2016TVTperformance}, as well as  cognitive radio and radar systems \cite{Simon2003TWCsome,Suraweera2010TVTcapacity,Kang2003JSAClargest,Chen2004TCdistribution,Ma2000JSACunified,Zhang2002TCgeneral,Ghasemi2008ICMspectrum,Digham2007TCenergy, simon2002bookdigital,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan,ermolova2014laplace,peppas2013performance}. However, in these applications, the presence of the Marcum $Q$-function makes the mathematical analysis challenging, because it is  difficult to manipulate  with no closed-form  expressions especially when it appears in parameter optimizations and integral calculations. For this reason, several methods have been developed in \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,zhao2008ELtight,Simon2000TCexponential,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral,jimenez2014connection}  to bound/approximate the  Marcum $Q$-function. For example, \cite{Fu2011GLOBECOMexponential,zhao2008ELtight} have proposed  modified forms of the function, while \cite{Simon2000TCexponential,annamalai2001WCMCcauchy} have derived exponential-type bounds which are good for the bit error rate analysis at high signal-to-noise ratios (SNRs). Other types of bounds are expressed by, e.g., error function \cite{Kam2008TCcomputing} and Bessel functions \cite{Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral}. Some alternative methods have been also proposed in \cite{Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Bocus2013CLapproximation,Gaur2003TVTsome}. Although each of these approximation/bounding techniques are fairly tight for their considered problem formulation, they are still based on difficult functions, or have complicated summation/integration formations, which may be not easy to deal with in, e.g., integral calculations and parameter optimizations. 


In this paper, we first propose a simple semi-linear approximation of the first-order Marcum $Q$-function (Lemma \ref{Lemma1}, Corollaries \ref{coro1}-\ref{coro2}). As we explain in the following (Lemmas \ref{Lemma1}-\ref{Lemma4}), in contrast to the schemes of \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,zhao2008ELtight,Simon2000TCexponential,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral,jimenez2014connection}, our proposed approximation is not tight at the tails of  the Marcum $Q$-function. Therefore, it is not useful in, e.g., error probability-based problem formulations.  On the other hand, the advantages of our proposed approximation method, compared to \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,zhao2008ELtight,Simon2000TCexponential,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral,jimenez2014connection}, are 1) its simplicity, and 2) tightness in the moderate values of the function. This is important because, as observed in, e.g., \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,Makki2013TCfeedback,Makki2011Eurasipcapacity,Makki2018WCLwireless,Makki2016TVTperformance,Simon2003TWCsome,Suraweera2010TVTcapacity,Ma2000JSACunified,Digham2007TCenergy,Cao2016CLsolutions,sofotasios2015solutions,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan}, in different applications, the Marcum $Q$-function is typically combined with other functions which tend to zero at the tails of the Marcum $Q$-function. In such cases, the inaccuracy of the approximation at the tails does not affect the tightness of the final analysis. Thus, our proposed scheme provides tight and simple approximation results for different problem formulations such as capacity calculation \cite{Makki2011Eurasipcapacity,Suraweera2010TVTcapacity}, throughput/average rate derivation \cite{Makki2013TCfeedback,Makki2018WCLwireless,Makki2016TVTperformance}, energy detection of unknown signals over various multipath fading channels \cite{Digham2007TCenergy,Cao2016CLsolutions,sofotasios2015solutions}, as well as  performance evaluation of  non-coherent receivers in radar systems \cite{Cui2012ELtwo}. Also, the simplicity of the approximation method makes it possible to perform further analysis such as parameter optimization and to obtain intuitive insights from the derivations.


To demonstrate the usefulness of the proposed approximation technique in communication systems, we analyze the performance of predictor antenna (PA) systems in presence of spatial mismatch. Here, the PA system is referred to as a setup with two (sets of) antennas on the roof of a vehicle. The PA positioned in the front of a vehicle can be used to improve the channel state estimation for downlink data reception at the receive antenna (RA) on the vehicle that is aligned behind the PA \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects,Guo2019WCLrate}. 


The feasibility of PA setups, which are of interest particularly in public transport systems such as trains and buses, but potentially also for the more design-constrained cars, has been previously shown through experimental tests \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman}. Particularly, as shown in testbed implementations, e.g.,  \cite{BJ2017PIMRCpredictor} and \cite{BJ2017ICCWusing}, with a two-antenna PA setup a normalised mean square error  of around -10 dB can be obtained for speeds up to 50 km/h, with  measured predictions horizons up to three times the wavelengths. This is by an order of magnitude better than state-of-the-art Kalman prediction-based systems \cite{Ekman2002,Aronsson2011} with prediction horizon limited to 0.1-0.3 times the wavelength. Moreover, the  European project deliverables, e.g., ARTIST4G project \cite[Chapter 2]{ARTIST4G}, METIS project \cite[P. 107]{metis2015d33} and 5GCAR project \cite[Chapter 3]{5gcar2019d33}, have  well addressed the feasibility of the PA concept in network-level design. Finally, different works have analyzed the PA system in both frequency division duplex (FDD) \cite{BJ2017ICCWusing,BJ2017PIMRCpredictor,phan2018WSAadaptive} and time division duplex (TDD) \cite{DT2015ITSMmaking,Apelfrojd2018PIMRCkalman} systems, with some developments on addressing the system challenges such as  antenna coupling \cite{Jamaly2014EuCAPanalysis,Jamaly2019IETeffects}, spatial mismatch \cite{Jamaly2019IETeffects,Guo2019WCLrate}, and spectrum underutilization \cite{guo2020power,guo2020rate}. 

Among the challenges of the PA system is the spatial mismatch. If the RA does not arrive in the same position as the PA, the actual channel for the RA would not be identical to the one experienced by the PA before. Such inaccurate channel state information (CSI) estimation will affect the system performance considerably at moderate/high speeds \cite{DT2015ITSMmaking,Guo2019WCLrate}. 

In this paper, we address the spatial  mismatch problem by implementing adaptive rate allocation. In our proposed setup, the instantaneous CSI provided by the PA is used to adapt the data rate of the signals sent to the RA from the base station (BS). The problem is cast in the form of throughput maximization. Particularly, we use our developed approximation approach to derive closed-form expressions for the instantaneous and average throughput as well as the optimal rate allocation maximizing the throughput (Lemma \ref{Lemma4}). Moreover, we study the effect of different parameters such as the antennas distance, the vehicle speed, and the processing delay of the BS on the performance of PA setups. 


Our paper is different from the state-of-the-art literature because the proposed semi-linear approximation of the first-order Marcum $Q$-function and the derived closed-form expressions for the considered integrals have not been presented by, e.g., \cite{Bocus2013CLapproximation,helstrom1994elements,Fu2011GLOBECOMexponential,Makki2013TCfeedback,Makki2011Eurasipcapacity,Makki2018WCLwireless,Makki2016TVTperformance,Simon2003TWCsome,Suraweera2010TVTcapacity,Kang2003JSAClargest,Chen2004TCdistribution,Ma2000JSACunified,Zhang2002TCgeneral,Ghasemi2008ICMspectrum,Digham2007TCenergy, simon2002bookdigital,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan,ermolova2014laplace,peppas2013performance,zhao2008ELtight,Simon2000TCexponential,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral,jimenez2014connection,Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects,Guo2019WCLrate}. Also, as opposed to \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects}, we perform analytical evaluations on the system performance with CSIT (T: at the transmitter)-based rate optimization to mitigate the effect of the spatial mismatch. Moreover, compared to our preliminary results in \cite{Guo2019WCLrate}, this paper develops the semi-linear approximation method for the Marcum $Q$-function, and uses our proposed approximation method to analyze the performance of the PA system. Also, we perform deep analysis of the effect of various parameters, such as imperfect CSIT feedback schemes, and processing delay of the BS on the system performance. 



The simulation and the analytical results indicate that the proposed semi-linear approximation is useful for the mathematical analysis of different Marcum $Q$-function-based problem formulations. Particularly, our approximation method enables us to represent different Marcum $Q$-function-based integrations and optimizations in closed-form. Considering the PA system, our derived analytical results show that adaptive rate allocation can considerably improve the performance of the PA system in the presence of spatial mismatch. Finally, with different levels of channel estimation, our results show that there exists an optimal speed for the vehicle optimizing the throughput/outage probability, and the system performance is sensitive to the vehicle speed/processing delay as the speed moves away from its optimal value. 


This paper is organized as follows. In Section 2, we present our proposed semi-linear approximation of the first-order Marcum $Q$-function, and derive closed-form solutions for some integrals of interest. Section 3 deals with the application of the approximation in the PA system,  deriving closed-form expressions for the optimal rate adaptation, the instantaneous throughput as well as the expected throughput.  In this way, Sections 2 and 3 demonstrate examples on how the proposed approximation can be useful in, respectively, expectation- and optimization-based problem formulations involving the Marcum $Q$-function. Concluding remarks are provided in Section 4. 





\section{Approximation of the first-order Marcum Q-function}
In this section, we present our semi-linear approximation of the cumulative distribution function (CDF) in the form of $y(\alpha, \beta ) = 1-Q_1(\alpha,\beta)$. The idea of this proposed approximation is to use one point and its corresponding slope in that point to create a line  approximating the CDF. The approximation method is summarized in Lemma \ref{Lemma1} as follows.
\begin{lem}\label{Lemma1}
 The CDF of the form $y(\alpha, \beta ) = 1-Q_1(\alpha,\beta)$ can be semi-linearly approximated as $Y(\alpha,\beta)\simeq \mathcal{Z}(\alpha, \beta)$ where
\begin{align}\label{eq_lema1}
\mathcal{Z}(\alpha, \beta)=
\begin{cases}
0,  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta < c_1  \\ 
 \frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}\times\\
 ~~~I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)\times\left(\beta-\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)+\\
 ~~~1-Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right),  ~~~~~~\mathrm{if}~ c_1 \leq\beta\leq c_2 \\
1,  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta> c_2,
\end{cases}
\end{align}
with
\begin{align}\label{eq_c1}
   & c_1(\alpha) =~~~ \max\Bigg(0,\frac{\alpha+\sqrt{\alpha^2+2}}{2}+\nonumber\\
    &~~~\frac{Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)-1}{\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)}\Bigg),
\end{align}
\begin{align}\label{eq_c2}
   & c_2(\alpha) = \frac{\alpha+\sqrt{\alpha^2+2}}{2}+\nonumber\\
   & ~~~\frac{Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)}{\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)}.
\end{align}
\end{lem}
\begin{proof}

We aim to approximate the CDF in the range $y \in [0, 1]$ by 
\begin{align}\label{eq_YY}
    y-y_0 = m(x-x_0),
\end{align}
where $\mathcal{C} = (x_0,y_0)$ is a point on the CDF curve and $m$ is the slope at point $\mathcal{C}$ of $y(\alpha,\beta)$. Then, the parts of the line outside this region are replaced by $y=0$ and $y=1$ (see Fig. \ref{fig_CDFilu}).

To obtain a good approximation of the CDF, we select the point $\mathcal{C}$ by solving

\begin{align}\label{eq_partialsquare}
   x = \mathop{\arg}_{t} \left\{  \frac{\partial^2\left(1-Q_1(\alpha,t)\right)}{\partial t^2} = 0\right\},
\end{align}
because the function is symmetric around this point, and (\ref{eq_partialsquare}) gives the best fit for a linear function. Then, using the derivative of the first-order Marcum $Q$-function with respect to $x$ \cite[Eq. (2)]{Pratt1968PIpartial}
\begin{align}\label{eq_derivativeMarcumQ}
    \frac{\partial Q_1(\alpha,x)}{\partial x} = -x e^{-\frac{\alpha^2+x^2}{2}}I_0(\alpha x),
\end{align}
(\ref{eq_partialsquare}) is equivalent to 
\begin{align}
   x =  \mathop{\arg}_{x} \left\{\frac{\partial\left(x e^{-\frac{\alpha^2+x^2}{2}}I_0(\alpha x)\right)}{\partial x}=0\right\}.
\end{align}
Using the approximation $I_0(x) \simeq \frac{e^x}{\sqrt{2\pi x}} $ \cite[Eq. (9.7.1)]{abramowitz1999ia} and writing
\begin{align}
    &~~~\frac{\partial\left(\sqrt{\frac{x}{2\pi \alpha}}e^{-\frac{(x-\alpha)^2}{2}}\right)}{\partial x} = 0\nonumber\\
   \Rightarrow &\frac{1}{\sqrt{2\pi\alpha}}\left(\frac{e^{-\frac{(x-\alpha)^2}{2}}}{2\sqrt{x}}+\sqrt{x}e^{-\frac{(x-\alpha)^2}{2}}(\alpha-x)\right)  = 0\nonumber\\
    \Rightarrow &2x^2-2\alpha x-1 =0,
\end{align}
we obtain 
\begin{align}\label{eq_beta0}
    x = \frac{\alpha+\sqrt{\alpha^2+2}}{2},
\end{align}
since $x\geq0$. In this way, we find the point 
\begin{align}
    \mathcal{C}=\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}, 1-Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)\right).
\end{align}

To calculate the slope $m$ at the point $\mathcal{C}$, we plug (\ref{eq_beta0}) into (\ref{eq_derivativeMarcumQ}) leading to
\begin{align}\label{eq_m}
   & m = \frac{\alpha+\sqrt{\alpha^2+2}}{2}\times\nonumber\\
    & ~~~e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right).
\end{align}
Finally, using (\ref{eq_YY}), (\ref{eq_beta0}) and (\ref{eq_m}), the CDF $y(\alpha, \beta) = 1-Q_1(\alpha,\beta)$ can be approximated  as in (\ref{eq_lema1}). Note that, because the CDF is limited to the range [0 1], the boundaries $c_1$ and $c_2$ in (\ref{eq_lema1}) are obtained by setting $y=0$ and $y=1$ which leads to the semi-linear approximation as given in (\ref{eq_lema1}).
\end{proof}


%==============
%Corollary 1, 2, 3
%==============
To further simplify the calculation, considering different ranges of $\alpha$, the approximation (\ref{eq_lema1}) can be simplified as stated in the following corollaries. 

\begin{corollary}\label{coro1}
For moderate/large values of $\alpha$, we have $y(\alpha,\beta)\simeq\tilde{\mathcal{Z}}(\alpha,\beta)$ where
\begin{align}\label{eq_coro1}
\tilde{\mathcal{Z}}(\alpha,\beta)&\simeq
\begin{cases}
0,  ~~~~~~~~~~~~~\mathrm{if}~\beta < \frac{-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha  \\ 
\alpha e^{-\alpha^2}I_0(\alpha^2)(\beta-\alpha) + 
\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right), \\ ~~~~~~~~~~~~~~~~\mathrm{if}~\frac{-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha \leq\beta\\
~~~~~~~~~~~~~~~~~~~~\leq\frac{1-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha \\
1,  ~~~~~~~~~~~~~\mathrm{if}~ \beta> \frac{1-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha.
\end{cases}\\
&\overset{(a)}{\simeq}
\begin{cases}
0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \beta < \breve{c}_1  \\ 
\frac{1}{\sqrt{2\pi}}(\beta-\alpha) + 
\frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \breve{c}_1 \leq\beta\leq \breve{c}_2 \\
1, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta>\breve{c}_2,
\end{cases}
\end{align}
with $\breve{c}_1$ and $\breve{c}_2$ given in (\ref{eq_dotc1}) and (\ref{eq_dotc2}), respectively.
\end{corollary}

\begin{proof}
Using (\ref{eq_beta0}) for moderate/large values of $\alpha$, we have $x \simeq \alpha$ and
\begin{align}
        \tilde{c}_1 = \frac{-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha,
\end{align}
\begin{align}
     \tilde{c}_2 = \frac{1-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha,
\end{align}
which leads to (\ref{eq_coro1}). Note that in (\ref{eq_coro1}) we have used the fact that \cite[Eq.  (A-3-2)]{schwartz1995communication}
\begin{align}
    Q_1(\alpha,\alpha) = \frac{1}{2}\left(1+e^{-\alpha^2}I_0(\alpha^2)\right).
\end{align}
Finally, $(a)$ is obtained by using the approximation $I_0(x) \simeq \frac{e^x}{\sqrt{2\pi x}}$ where
\begin{align}\label{eq_dotc1}
        \breve{c}_1 = -\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha,
\end{align}
\begin{align}\label{eq_dotc2}
     \breve{c}_2 = \sqrt{2\pi}-\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha.
\end{align}
\end{proof}

\begin{corollary}\label{coro2}
For small values of $\alpha$, we have  $y(\alpha,\beta)\simeq\hat{ \mathcal{Z}}(\alpha,\beta)$ with
\begin{align}\label{eq_coro2}
\hat{ \mathcal{Z}}(\alpha,\beta)\simeq
\begin{cases}
0,   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~\beta < \hat{c}_1  \\ 
\frac{\alpha+\sqrt{2}}{2}  e^{-\frac{\alpha^2+\left(\frac{\alpha+\sqrt{2}}{2}\right)^2}{2}}\times\\
~~~I_0\left(\frac{\alpha(\alpha+\sqrt{2})}{2}\right)(\beta-\frac{\alpha+\sqrt{2}}{2}) + \\
~~~1-Q_1\left(\alpha,\frac{\alpha+\sqrt{2}}{2}\right), 
~~~~~~~~\mathrm{if}~\hat{c}_1 \leq\beta\leq \hat{c}_2 \\
1, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta> \hat{c}_2
\end{cases}
\end{align}
with $\hat{c}_1$ and $\hat{c}_2$ given in (\ref{eq_hatc1}) and (\ref{eq_hatc2}), respectively.
\end{corollary}
\begin{proof}
Using (\ref{eq_beta0}) for small values of $\alpha$, we have $x\simeq \frac{\alpha+\sqrt{2}}{2}$, which leads to 
\begin{equation}\label{eq_hatc1}
    \hat{c}_1 = \frac{-1+Q_1\left(\alpha,\frac{\alpha+\sqrt{2}}{2}\right)}{\left(\frac{\alpha+\sqrt{2}}{2} \right)^2 e^{-\frac{\alpha^2+\left(\frac{\alpha+\sqrt{2}}{2}\right)^2}{2}} I_0\left(\frac{\alpha(\alpha+\sqrt{2})}{2}\right)}+\alpha,
\end{equation}
and
\begin{equation}\label{eq_hatc2}
    \hat{c}_2 = \frac{Q_1\left(\alpha,\frac{\alpha+\sqrt{2}}{2}\right)}{\left(\frac{\alpha+\sqrt{2}}{2} \right)^2 e^{-\frac{\alpha^2+\left(\frac{\alpha+\sqrt{2}}{2}\right)^2}{2}} I_0\left(\frac{\alpha(\alpha+\sqrt{2})}{2}\right)}+\alpha,
\end{equation}
and simplifies (\ref{eq_lema1}) to (\ref{eq_coro2}).
\end{proof}



% \begin{corollary}\label{coro3}
% Equation (\ref{eq_coro1}) can be further simplified as
% \begin{align}\label{eq_coro3}
% \breve{\mathcal{Z}}(\alpha,\beta)\simeq
% \begin{cases}
% 0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \beta < \breve{c}_1  \\ 
% \frac{1}{\sqrt{2\pi}}(\beta-\alpha) + 
% \frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \breve{c}_1 \leq\beta\leq \breve{c}_2 \\
% 1, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta>\breve{c}_2
% \end{cases}
% \end{align}
% with $\breve{c}_1$ and $\breve{c}_2$ given by (\ref{eq_dotc1}) and (\ref{eq_dotc2}), respectively.
% \end{corollary}
% \begin{proof}
% For moderate/large values of $\alpha$, using the approximation $I_0(x) \simeq \frac{e^x}{\sqrt{2\pi x}}$ for (\ref{eq_coro1}) leads to (\ref{eq_coro3}) where
% \begin{align}\label{eq_dotc1}
%         \breve{c}_1 = -\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha,
% \end{align}
% and
% \begin{align}\label{eq_dotc2}
%      \breve{c}_2 = \sqrt{2\pi}-\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha.
% \end{align}
% \end{proof}














To illustrate these semi-linear approximations, Fig. \ref{fig_CDFilu} shows the CDF $y(\alpha,\beta)= 1-Q_1(\alpha,\beta)$ for both small and large values of $\alpha$, and compares the exact CDF with the approximation schemes of Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro2}. From Fig. \ref{fig_CDFilu}, we can observe that Lemma \ref{Lemma1} is tight for a broad range of $\alpha$  and moderate values of $\beta$. Moreover, the tightness is improved as $\alpha$ decreases. Also,  Corollaries \ref{coro1}-\ref{coro2} provide good approximations for large and small values of $\alpha$, respectively. Then, the proposed approximations are not tight at the tails of the CDF. However, as observed in \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,Makki2013TCfeedback,Makki2011Eurasipcapacity,Makki2018WCLwireless,Makki2016TVTperformance,Simon2003TWCsome,Suraweera2010TVTcapacity,Ma2000JSACunified,Digham2007TCenergy,Cao2016CLsolutions,sofotasios2015solutions,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan}  and in the following, in different applications,  the Marcum $Q$-function is normally combined with other functions which tend to zero of the tails of the CDF. In such cases, the inaccuracy of the approximation at the tails does not affect the tightness of the final result. 














As an example, we first consider a general integral in the form of
\begin{align}\label{eq_integral}
G(\alpha,\rho)=\int_\rho^\infty{e^{-nx} x^m \left(1-Q_1(\alpha,x)\right)\text{d}x} ~~\forall n,m,\alpha,\rho>0.
\end{align}
Such an integral has been observed in various applications, e.g., in bit-error-probability evaluation of a Rayleigh fading channel \cite[eq. (1) (13)]{Simon2003TWCsome}, in energy detection of unknown signals over various multipath fading channels \cite[eq. (2)]{Cao2016CLsolutions}, in capacity analysis with channel inversion and fixed rate over correlated Nakagami fading \cite[eq. (1)]{sofotasios2015solutions}, in performance evaluation of  incoherent receivers in radar systems \cite[eq. (3)]{Cui2012ELtwo}, and in error probability analysis of diversity receivers \cite[eq. (1)]{Gaur2003TVTsome}. However, depending on the values of $n, m$ and $\rho$, (\ref{eq_integral}) may have no closed-form expression. Using Lemma \ref{Lemma1}, $G(\alpha,\rho)$ can be approximated in closed-form as presented in Lemma \ref{Lemma2}.

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure1.pdf}\\
\caption{Illustration of the semi-linear approximation with Lemma \ref{Lemma1}, and Corollaries \ref{coro1}-\ref{coro2}. For each value of $\alpha\in[1,1.5,2]$, the approximated results obtained by Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro2} are compared with the exact value for a broad range of $\beta$.}
\label{fig_CDFilu}
\end{figure}

\begin{lem}\label{Lemma2}
The integral (\ref{eq_integral}) is approximately given by
\begin{align}
G(\alpha,\rho)\simeq
\begin{cases}
\Gamma(m+1,n\rho)n^{-m-1}, ~~~~~~~~~~~~~~~~~~\mathrm{if}~  \rho \geq \breve{c}_2  \\ 
\Gamma(m+1,n\breve{c}_2)n^{-m-1} + \\
~~\left(-\frac{\alpha}{\sqrt{2\pi}}+0.5*\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\times n^{-m-1}\times\\
~~\left(\Gamma(m+1,n\max(\breve{c}_1,\rho))-\Gamma(m+1,n\breve{c}_2)\right)+\\
~~\left(\Gamma(m+2,n\max(\breve{c}_1,\rho))-\Gamma(m+2,n\breve{c}_2)\right)\times\\
~~\frac{n^{-m-2}}{\sqrt{2\pi}},
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \rho<\breve{c}_2,
\end{cases}
\end{align}
where $\Gamma(s,x) = \int_{x}^{\infty} t^{s-1}e^{-t} \mathrm{d}t$ is the upper incomplete gamma function \cite[Eq. 6.5.1]{abramowitz1999ia}.
\end{lem}
\begin{proof}
See Appendix \ref{proof_Lemma2}. 
\end{proof}









As a second integration example of interest, consider
\begin{align}\label{eq_integralT}
    T(\alpha,m,a,\theta_1,\theta_2) = \int_{\theta_1}^{\theta_2} e^{-mx}\log(1+ax)Q_1(\alpha,x)\text{d}x \nonumber\\\forall m>0,a,\alpha,
\end{align}
with $\theta_2>\theta_1\geq0$, which does not have a closed-form expression for different values of $m, a, \alpha$. This type of integral is interesting as it could be used to analyze the expected performance of outage-limited systems, e.g,  the considered integral in the shape of \cite[eq. (1) (13)]{Simon2003TWCsome}, \cite[eq. (2)]{Cao2016CLsolutions}, \cite[eq. (3)]{Cui2012ELtwo}, and \cite[eq. (1)]{Gaur2003TVTsome}, applied in the analysis of the outage-limited throughput, i.e., when the outage-limited throughput $\log(1+ax)Q_1(\alpha,x)$  \cite[p. 2631]{Biglieri1998TITfading}\cite[Theorem 6]{Verdu1994TITgeneral}\cite[Eq. (9)]{Makki2014TCperformance} is averaged over fading statistics. Then, using Lemma \ref{Lemma1}, (\ref{eq_integralT}) can be approximated in closed-form as follows.

\begin{lem}\label{Lemma3}
The integral (\ref{eq_integralT}) is approximately given by
\begin{align}
  T(\alpha,m,a,\theta_1,\theta_2)\simeq~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\nonumber\\
\begin{cases}
\mathcal{F}_1(\theta_2)-\mathcal{F}_1(\theta_1), ~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  0\leq\theta_1<\theta_2 < c_1  \\ 
\mathcal{F}_1(c_1)-\mathcal{F}_1(\theta_1)+\mathcal{F}_2(\max(c_2,\theta_2))-\mathcal{F}_2(c_1),  \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1<c_1, \theta_2\geq c_1\\
 \mathcal{F}_2(\max(c_2,\theta_2))-\mathcal{F}_2(c_1), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1>c_1\\
0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1 > c_2,
\end{cases}  
\end{align}
where 
$c_1$ and $c_2$ are given by (\ref{eq_c1}) and (\ref{eq_c2}), respectively. Moreover,
\begin{align}\label{eq_F1}
    \mathcal{F}_1(x) \doteq \frac{1}{m}\left(-e^{\frac{m}{a}}\operatorname{E_1}\left(mx+\frac{m}{a}\right)-e^{-mx}\log(ax+1)\right),
\end{align}
and
\begin{align}\label{eq_F2}
    \mathcal{F}_2(x) \doteq &~ \mathrm{e}^{-mx}\Bigg(\left(mn_2-an_2-amn_1\right)\mathrm{e}^\frac{m\left(ax+1\right)}{a}\nonumber\\&~~ \operatorname{E_1}\left(\frac{m\left(ax+1\right)}{a}\right)-
    a\left(mn_2x+n_2+mn_1\right)\nonumber\\&~~\log\left(ax+1\right)-an_2\Bigg),
\end{align}
with
\begin{align}\label{eq_n1}
    n_1 = 1+\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}\times\nonumber\\
 I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)\times\frac{\alpha+\sqrt{\alpha^2+2}}{2}-\nonumber\\
 1+Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right),
\end{align}
and
\begin{align}\label{eq_n2}
    n_2 = -\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}\times\nonumber\\
 I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right).
\end{align}
In (\ref{eq_F1}) and (\ref{eq_F2}), $\operatorname{E_1}(x) = \int_x^{\infty} \frac{e^{-t}}{t} \mathrm{d}t$ is the Exponential Integral function \cite[p. 228, (5.1.1)]{abramowitz1999ia}.
\end{lem}

\begin{proof}
See Appendix \ref{proof_Lemma3}.
\end{proof}

Finally, setting $m = 0$ in (\ref{eq_integralT}), i.e.,
\begin{align}\label{eq_integralTs}
     T(\alpha,0,a,\theta_1,\theta_2) = \int_{\theta_1}^{\theta_2} \log(1+ax)Q_1(\alpha,x)\text{d}x,  \forall a,\alpha,
\end{align}
one can follow the same procedure in (\ref{eq_integralT}) to approximate (\ref{eq_integralTs}) as
\begin{align}\label{eq_integralTss}
  T(\alpha,0,a,\theta_1,\theta_2)\simeq~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\nonumber\\
\begin{cases}
\mathcal{F}_3(\theta_2)-\mathcal{F}_3(\theta_1), ~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  0\leq\theta_1<\theta_2 < c_1  \\ 
\mathcal{F}_3(c_1)-\mathcal{F}_3(\theta_1)+\mathcal{F}_4(\max(c_2,\theta_2))-\mathcal{F}_4(c_1),  \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1<c_1, \theta_2\geq c_1\\
 \mathcal{F}_4(\max(c_2,\theta_2))-\mathcal{F}_4(c_1), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1>c_1\\
0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1 > c_2,
\end{cases}  
\end{align}
with $c_1$ and $c_2$ given by (\ref{eq_c1}) and (\ref{eq_c2}), respectively. Also,
\begin{align}
    \mathcal{F}_3 = \frac{(ax+1)(\log(ax+1)-1)}{a},
\end{align}
and
\begin{align}
    \mathcal{F}_4 = \frac{n_2\left((2a^2x^2-2)\log(ax+1)-a^2x^2+2ax\right)}{4a^2}+\nonumber\\\frac{n_1(ax+1)(\log(ax+1)-1)}{a},
\end{align}
where $n_1$ and $n_2$ are given by (\ref{eq_n1}) and (\ref{eq_n2}), respectively.


\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure2.pdf}\\
\caption{The  integral (\ref{eq_integral}) involving Marcum $Q$-function. Solid lines are exact values while crosses are the results obtained from Lemma \ref{Lemma2}, $\alpha = 2$,  $(m,n) = \{(4,4), (3,3), (2,2), (0,1), (1,1)\}$.}\label{fig_integrald}
\end{figure}






In Figs. \ref{fig_integrald} and \ref{fig_t2}, we evaluate the tightness of the approximations in Lemmas \ref{Lemma2}, \ref{Lemma3} and (\ref{eq_integralTss}), for different values of $m$, $n$, $\rho$, $a$ and $\alpha$. From the figures, it can be observed that the approximation schemes of   Lemmas \ref{Lemma2}-\ref{Lemma3} and (\ref{eq_integralTss}) are very tight for different parameter settings, while our proposed semi-linear approximation makes it possible to represent the integrals in closed-form.  In this way, although the approximation (\ref{eq_lema1}) is not tight at the tails of the CDF, it gives tight approximation results when it appears in different integrals (Lemmas \ref{Lemma2}-\ref{Lemma3}) with the Marcum-$Q$ function  combined with other functions tending to zero at the tails of the function. Also, as we show in Section 3, the semi-linear approximation scheme is efficient in optimization problems involving the Marcum $Q$-function. Finally, to tightly approximate the Marcum $Q$-function at the tails, which are the range of interest in, e.g., error probability analysis, one can use the approximation schemes of \cite{Simon2000TCexponential,annamalai2001WCMCcauchy}. 







\section{Applications in PA Systems}
In Section 2, we showed how the proposed approximation scheme enables us to derive closed-form expressions for a broad range of integrals, as required in various expectation-based calculations, e.g., \cite{Simon2003TWCsome,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,Gaur2003TVTsome,Simon2000TCexponential,6911973}. On the other hand, the Marcum $Q$-function may also  appear in  optimization problems, e.g., \cite[eq. (8)]{Azari2018TCultra},\cite[eq. (9)]{Alam2014INFOCOMWrobust}, \cite[eq. (10)]{Gao2018IAadmm}, \cite[eq. (10)]{Shen2018TVToutage}, \cite[eq. (15)]{Song2017JLTimpact}, \cite[eq. (22)]{Tang2019IAan}.  For this reason, in this section, we provide an example of using our proposed semi-linear approximation in an optimization problem for the PA systems.

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure3.pdf}\\
\caption{The integral (\ref{eq_integralT}) involving the Marcum $Q$-function. Solid lines are exact values while crosses are the results obtained from Lemma \ref{Lemma3} and (\ref{eq_integralTss}). $\theta_1 = 0, \theta_2 = \infty$. }\label{fig_t2}
\end{figure}

\subsection{Problem Formulation}
Vehicle communication is one of the most important use cases in 5G.  Here, the main focus is to provide efficient and reliable connections to cars and public transports, e.g., busses and trains. CSIT plays an important role in achieving these goals, since the data transmission efficiency can be improved by updating the transmission parameters relative to the instantaneous channel state.  However, the typical CSIT acquisition systems, which are mostly designed for (semi)static channels, may not work well for high-speed vehicles. This is because, depending on the vehicle speed, the position of the antennas may change quickly and the channel information becomes inaccurate.  To overcome this issue, \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing} propose the PA setup as shown in Fig. \ref{system}. With a PA setup, which is of interesting in Vehicle-to-everything (V2X) communications \cite{Sternad2012WCNCWusing} as well as integrated access and backhauling \cite{Teyeb2019VTCintegrated}, two antennas are deployed on the top of the vehicle. The first antenna,  the PA,  estimates the channel and sends feedback to the BS at time $t$. Then, the BS uses the CSIT provided by the PA to communicate with a second antenna, which we refer to as RA, at time $t+\delta$, where $\delta$ is the processing time at the BS. In this way, the BS can use the CSIT acquired from the PA and perform various CSIT-based transmission schemes, e.g.,  \cite{Sternad2012WCNCWusing,BJ2017ICCWusing}.  


\begin{figure}
%\vspace{-3mm}
\centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.7\columnwidth]{Figure4.pdf}\\
 %\vspace{-4mm}
\caption{A PA system with the mismatch problem. Here, $\hat h$ is the channel between the BS and the PA while $h$ refers to the BS-RA link. The vehicle is moving with speed $v$ and the antenna separation is $d_\text{a}$. The red arrow indicates the spatial mismatch, i.e., when the RA does not reach at the same  point as the PA when sending pilots. Also, $d_\text{m}$ is the moving distance of the vehicle which is affected by the processing delay $\delta$ of the BS. }\label{system}
\end{figure}


We assume that the vehicle moves through a stationary electromagnetic standing wave pattern \footnote{This has been experimentally verified in, e.g., \cite{Jamaly2014EuCAPanalysis}}. Thus, if the RA reaches exactly the same position as the position of the PA when sending the pilots, it will experience the same channel and the CSIT will be perfect. However, if the RA does not reach the same spatial point as the PA, due to, e.g., the BS processing delay is not equal to the time that we need until the RA reaches the same point as the PA, the RA may receive the data in a place different from the one in which the PA was sending the pilots. Such spatial mismatch may lead to CSIT inaccuracy, which will affect the system performance considerably. Thus, we need adaptive schemes to compensate for it.

Considering downlink transmission in the BS-RA link, the received signal is given by
\begin{align}\label{eq_Y}
{{Y}} = \sqrt{P}hX + Z.
\end{align}
Here, $P$ represents the transmit power, $X$ is the input message with unit variance, and $h$ is the fading coefficient between the BS and the RA. Also, $Z \sim \mathcal{CN}(0,1)$ denotes the independent and identically distributed (IID) complex Gaussian noise added at the receiver.



We denote the channel coefficient of the PA-BS uplink as $\hat{h}$. Also, we define $d$ as the effective distance between  the place where the PA estimates the channel at time $t$, and the place where the RA reaches at time $t+\delta$. As can be seen in Fig. \ref{system}, $d$ can be calculated as
\begin{align}\label{eq_d}
    d = |d_\text{a} - d_\text{m} | = |d_\text{a} - v\delta|,
\end{align}
where $d_\text{m}$ is the moving distance of the vehicle during time interval $\delta$, and $v$ is the velocity of the vehicle. Also, $d_\text{a}$ is the antenna separation between the PA and the RA. In conjunction to (\ref{eq_d}), here, we assume $d$ can be calculated by the BS. 

Using the classical Jake's correlation model \cite[p. 2642]{Shin2003TITcapacity} and  assuming a semi-static propagation environment, i.e., assuming that the coherence time of the propagation environment is larger than $\delta$,  the channel coefficient of the BS-RA downlink can be modeled as 
\begin{align}\label{eq_H}
    h = \sqrt{1-\sigma^2} \hat{h} + \sigma q.
\end{align}
Here, $q \sim \mathcal{CN}(0,1)$ which is independent of the known channel value $\hat{h}\sim \mathcal{CN}(0,1)$, and $\sigma$ is a function of the effective distance $d$ as 
\begin{align}
    \sigma = \frac{\frac{\phi_2^2-\phi_1^2}{\phi_1}}{\sqrt{ \left(\frac{\phi_2}{\phi_1}\right)^2 + \left(\frac{\phi_2^2-\phi_1^2}{\phi_1}\right)^2 }} = \frac{\phi_2^2-\phi_1^2}{\sqrt{ \left(\phi_2\right)^2 + \left(\phi_2^2-\phi_1^2\right)^2 }} .
\end{align}
Here, $\phi_1 = \bm{\Phi}_{1,1}^{1/2} $ and $\phi_2 = \bm{\Phi}_{1,2}^{1/2} $, where $\bm{\Phi}$ is  from Jake's model \cite[p. 2642]{Shin2003TITcapacity}
\begin{align}\label{eq_tildeH}
     \bigl[ \begin{smallmatrix}
  \hat{h}\\h
\end{smallmatrix} \bigr]= \bm{\Phi}^{1/2} \bm{H}_{\varepsilon}.
\end{align}
Note that, the channel model (\ref{eq_H}) has been experimentally verified in, e.g., \cite{Jamaly2014EuCAPanalysis} for PA setups. Also, one can follow the same method as in \cite{Guo2019WCLrate} to extend the model to the cases with temporally-correlated channels. Moreover, in (\ref{eq_tildeH}), $\bm{H}_{\varepsilon}$ has independent circularly-symmetric zero-mean complex Gaussian entries with unit variance, and $\bm{\Phi}$ is the channel correlation matrix with the $(i,j)$-th entry given by
\begin{align}\label{eq_phi}
    \Phi_{i,j} = J_0\left((i-j)\cdot2\pi d/ \lambda\right) \forall i,j.
\end{align}
Here, $J_n(x) = (\frac{x}{2})^n \sum_{i=0}^{\infty}\frac{(\frac{x}{2})^{2i}(-1)^{i} }{i!\Gamma(n+i+1)}$ represents the $n$-th order Bessel function of the first kind. Moreover, $\lambda$ denotes the carrier wavelength, i.e., $\lambda = c/f_\text{c}$ where $c$ is the speed of light and $f_\text{c}$ is the carrier frequency. 






From (\ref{eq_H}), for a given $\hat{h}$ and $\sigma \neq 0$, $|h|$ follows a Rician distribution, i.e., the  probability density function (PDF) of $|h|$ is given by 
\begin{align}
    f_{|h|\big|\hat{g}}(x) = \frac{2x}{\sigma^2}e^{-\frac{x^2+\hat{g}}{\sigma^2}}I_0\left(\frac{2x\sqrt{\hat{g}}}{\sigma^2}\right),
\end{align}
where $\hat{g} = (1-\sigma^2)|\hat{h}|^2$. Let us define the channel gain between BS-RA as $ g = |{h}|^2$. Then, the PDF of $f_{g|\hat{g}}$ is given by

\begin{align}\label{eq_pdf}
    f_{g|\hat{g}}(x) = \frac{1}{\sigma^2}e^{-\frac{x+\hat{g}}{\sigma^2}}I_0\left(\frac{2\sqrt{x\hat{g}}}{\sigma^2}\right),
\end{align}
which is non-central Chi-squared distributed with the CDF containing the first-order Marcum $Q$-function as
\begin{align}\label{eq_cdf}
    F_{g|\hat{g}}(x) = 1 - Q_1\left( \sqrt{\frac{2\hat{g}}{\sigma^2}}, \sqrt{\frac{2x}{\sigma^2}}  \right).
\end{align}



\subsection{Analytical Results on Rate Adaptation Using the Semi-Linear Approximation of the First-order Marcum Q-Function}\label{In Section III.C,}
We assume that $d_\text{a}$, $\delta $ and $\hat{g}$ are known by the BS. It can be seen from (\ref{eq_pdf}) that $f_{g|\hat{g}}(x)$ is a function of $v$. For a given $v$, the distribution of $g$ is known by the BS, and a rate adaption scheme can be performed to improve the system performance.

For a given instantaneous value of $\hat g$, the data is transmitted with instantaneous rate $R_{|\hat{g}}$ nats-per-channel-use (npcu). If the instantaneous channel gain realization supports the transmitted data rate $R_{|\hat{g}}$, i.e., $\log(1+gP)\ge R_{|\hat{g}}$, the data can be successfully decoded. Otherwise,  outage occurs. Hence, the outage probability in each time slot is
\begin{align}
    \Pr(\text{outage}|\hat{g}) = F_{g|\hat{g}}\left(\frac{e^{R_{|\hat{g}}}-1}{P}\right).
\end{align}
Also, the instantaneous throughput for a given $\hat{g}$ is
\begin{align}\label{eq_opteta}
\eta_{|\hat {g}}\left(R_{|\hat{g}}\right)=R_{|\hat{g}}\left(1-\Pr\left(\log(1+gP)<R_{|\hat{g}}\right)\right),
\end{align}
and the optimal rate adaptation maximizing the  instantaneous throughput is obtained by
\begin{align}\label{eq_optR}
    R_{|\hat{g}}^{\text{opt}}&=\argmax_{R_{|\hat{g}}\geq 0} \left\{ \left(1-\Pr\left(\log(1+gP)<R_{|\hat{g}}\right)\right)R_{|\hat{g}} \right\}\nonumber\\
    &=\argmax_{R_{|\hat{g}}\geq 0} \left\{ \left(1-F_{g|\hat{g}}\left(\frac{e^{R_{|\hat{g}}}-1}{P}\right)\right) R_{|\hat{g}}\right\}\nonumber\\
    &=\argmax_{R_{|\hat{g}}\geq 0} \left\{ Q_1\left(  \sqrt{\frac{2\hat{g}}{\sigma^2}}, \sqrt{\frac{2(e^{R_{|\hat{g}}}-1)}{P\sigma^2}} \right)R_{|\hat{g}} \right\},
\end{align}
where the last equality comes from (\ref{eq_cdf}). 

Using the derivatives of the Marcum $Q$-function, (\ref{eq_optR}) does not have a closed-form solution\footnote{To solve (\ref{eq_optR}), one can use different approximation methods of the Marcum $Q$-function, e.g., \cite{Guo2019WCLrate}. Here, we use Lemma \ref{Lemma1}/Corollaries \ref{coro1}-\ref{coro2} to solve (\ref{eq_optR}) to show the usefulness of the semi-linear approximation method. As shown, in Figs. \ref{fig_Figure5} and \ref{fig_Figure6}, the semi-linear approximation is tight for a broad range of parameter settings while it simplifies the optimization problem considerably. }. For this reason,  Lemma \ref{Lemma4}  uses the semi-linear approximation scheme of Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro2} to find the optimal data rate maximizing the instantaneous throughput.

\begin{lem}\label{Lemma4}
For a given channel realization $\hat{g}$, the throughput-optimized rate allocation is approximately given by (\ref{eq_appRF}) where $\mathcal{W}(\cdot)$ denotes the Lambert $\mathcal{W}$-function.
\end{lem}
\begin{proof}
The  approximation results of Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro2} can be generalized by $y(\alpha,\beta)\simeq\tilde{\mathcal{Z}}_{\text{general}}(\alpha,\beta)$ where
\begin{align}
\tilde{\mathcal{Z}}_{\text{general}}(\alpha,\beta)\simeq
\begin{cases}
0,~~~~~~~~~~~~~~~~~~~~\mathrm{if}~\beta < c_1(\alpha)  \\ 
o_1(\alpha)(\beta-o_2(\alpha)) + o_3,\\~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ c_1(\alpha) \leq \beta \leq c_2(\alpha)\\ 
1,~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta> c_2(\alpha).
\end{cases}
\end{align}


$o_i,i=1,2,3$, are given by (\ref{eq_lema1}), (\ref{eq_coro1}), or (\ref{eq_coro2}) depending on if we use Lemma \ref{Lemma1} or Corollaries \ref{coro1}-\ref{coro2}. In this way, (\ref{eq_opteta}) is approximated as
\begin{align}\label{eq_appR}
    \eta_{|\hat {g}}\simeq R_{|\hat{g}}\left(1-o_1(\alpha)\beta + o_1(\alpha)o_2(\alpha) - o_3(\alpha)\right),
\end{align}
where $\alpha = \sqrt{\frac{2\hat{g}}{\sigma^2}}$. To simplify the equation, we omit $\alpha$ in the following since it is a constant for given $\hat{g}$, $\sigma$. Then, setting the derivative of (\ref{eq_appR}) equal to zero, we obtain
\begin{align}\label{eq_appRF}
    & R_{|\hat{g}}^{\text{opt}}  \nonumber\\
    & = \operatorname*{arg}_{R_{|\hat{g}}\geq 0}\left\{ 1+o_1o_2-o_3-o_1\left(\frac{(R_{|\hat{g}}+2)e^{R_{|\hat{g}}}-2}{\sqrt{2P\sigma^2\left(e^{R_{|\hat{g}}}-1\right)}}\right)=0\right\}\nonumber\\
    % & = \operatorname*{arg}_{R_{|\hat{g}}\geq 0} \left\{ \left(\frac{(R_{|\hat{g}}+2)e^{R_{|\hat{g}}}-2}{\sqrt{2P\sigma^2\left(e^{R_{|\hat{g}}}-1\right)}}\right) = \frac{1+o_1o_2-o_3}{o_1}\right\}\nonumber\\
    & \overset{(b)}{\simeq} \operatorname*{arg}_{R_{|\hat{g}}\geq 0}\left\{ \left(\frac{R_{|\hat{g}}}{2}+1\right)e^{\frac{R_{|\hat{g}}}{2}+1} = \frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}\right\}\nonumber\\
    & \overset{(c)}{=} 2\mathcal{W}\left(\frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}-1\right).
\end{align}
Here,  $(b)$ comes from $e^{R_{|\hat{g}}}-1 \simeq e^{R_{|\hat{g}}} $ and $(R_{|\hat{g}}+2)e^{R_{|\hat{g}}}-2 \simeq (R_{|\hat{g}}+2)e^{R_{|\hat{g}}} $ which are appropriate at moderate/high values of $R_{|\hat{g}}$. Also, $(c)$ is obtained by the definition of the Lambert $\mathcal{W}$-function $xe^x = y \Leftrightarrow x = \mathcal{W}(y)$ \cite{corless1996lambertw}. 

\end{proof}

Finally, the expected throughput, averaged over multiple time slots, is obtained by $\eta = \mathbb{E}\left\{\eta|{\hat {g}}(R_{|\hat{g}}^{\text{opt}})\right\}$ with expectation over $\hat g$.  

Using (\ref{eq_appRF}) and the approximation \cite[Them. 2.1]{hoorfar2007approximation}
\begin{align}
    \mathcal{W}(x) \simeq \log(x)-\log\log(x), x\geq0,
\end{align}
we obtain
\begin{align}
    R_{|\hat{g}}^{\text{opt}}\simeq 2\log\left(\frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}-1\right)-\nonumber\\
    2\log\log\left(\frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}-1\right)
\end{align}
which implies as the transmit power increases, the optimal instantaneous rate increases with the square root of the transmit power (approximately) logarithmically.

\subsection{On the Effect of Imperfect Channel Estimation}
In Section \ref{In Section III.C,}, we assumed perfect channel estimation at the BS. The deviations of channel estimation, due to, e.g., radio-frequency mismatch, could invalidate the assumption of perfect channel estimation, and should be considered in the system design. Here, we follow the similar approach as in, e.g., \cite{Wang2007TWCperformance}, to add the effect of estimation error of $\hat{h}$ as an independent additive Gaussian variable whose variance is given by the accuracy of channel estimation. 

Let us define $\tilde h$ as the estimate of $\hat h$ at the BS. Then,  we further develop our channel model  (\ref{eq_H}) as
\begin{align}\label{eq_Htp}
    \tilde{h} = \kappa \hat{h} + \sqrt{1-\kappa^2} z, 
\end{align}
for each time slot, where $z \sim \mathcal{CN}(0,1)$ is a Gaussian noise which is uncorrelated with $H_{k}$. Also, $\kappa$ is a known correlation factor which represents the estimation error of $\hat{h}$ by $\kappa = \frac{\mathbb{E}\{\tilde{h}\hat{h}^*\}}{\mathbb{E}\{|\hat{h}|^2\}}$. Substituting (\ref{eq_Htp}) into (\ref{eq_H}), we have
\begin{align}\label{eq_Ht}
    h = \kappa\sqrt{1-\sigma^2}\hat{h}+\kappa\sigma q+\sqrt{1-\kappa^2}z.
\end{align}
Then, because  $\kappa\sigma q + \sqrt{1-\kappa^2}z$ is equivalent to a new Gaussian variable\\ $w \sim\mathcal{CN}\left(0,(\kappa\sigma)^2+1-\kappa^2\right)$, we can follow the same procedure as in (\ref{eq_optR})-(\ref{eq_appRF}) to analyze the system performance with imperfect channel estimation of the PA (see Figs. \ref{fig_Figure5}-\ref{fig_Figure6} for more discussions).



\subsection{Simulation Results}
In this part, we study the performance of the PA system and verify the tightness of the approximation scheme of Lemma \ref{Lemma4}. Particularly, we present the average throughput and the outage probability of the PA setup for different vehicle speeds/channel estimation errors. As an ultimate upper bound for the proposed rate adaptation scheme, we consider a genie-aided setup where we assume that the BS has perfect CSIT of the BS-RA link without uncertainty/outage probability. Then, as a lower-bound of the system performance, we consider the cases with no CSIT/rate adaptation as shown in Fig. \ref{fig_Figure5}. Here, the simulation results for the cases of no adaptation are obtained with only one antenna and no CSIT. In this case,  the data is sent with a fixed rate $R$ and it is decoded if $R<\log(1+gP)$, i.e., $g>\frac{e^{R}-1}{P}$. In this way, assuming Rayleigh fading, the average rate is given by
\begin{align}\label{eq_bench}
    R^{\text{No-adaptation}} = \int_{\frac{e^{R}-1}{P}}^{\infty} Re^{-x} \text{d}x = Re^{-\frac{e^{R}-1}{P}},
\end{align}
and the optimal rate allocation is found by setting the derivative of (\ref{eq_bench}) with respect to $R$ equal to zero leading to $\tilde{R} = \mathcal{W}(P)$, and the throughput is calculated as 
\begin{align}\label{eq_etanocsi}
  \eta^{\text{No-adaptation}} =\mathcal{W}(P)e^{-\frac{e^{\mathcal{W}(P)}-1}{P}}.  
\end{align}
Also, in the simulations, we set  $f_\text{c}$ = 2.68 GHz and $d_\text{a} = 1.5\lambda$. Finally, each point in the figures is obtained by averaging the system performance over $1\times10^5$ channel realizations.




In Fig. \ref{fig_Figure5}, we show the expected throughput $\eta$  in different cases for a broad range of signal-to-noise ratios (SNRs). Here, because the noise has unit variance, we define the SNR as $10\log_{10}P$. Also, we set $v = 114$ km/h in Fig. \ref{fig_Figure5}  as defined in (\ref{eq_d}), and $\kappa = 1$ as discussed in (\ref{eq_Ht}). The analytical results obtained by Lemma \ref{Lemma4} and Corollary \ref{coro2}, i.e., the approximation of (\ref{eq_optR}), are also presented. We have also checked the approximation result of Lemma \ref{Lemma4} while using Lemma \ref{Lemma1}/Corollary \ref{coro1}. Then, because the results are similar as those presented in Fig. \ref{fig_Figure5}, they are not included in the figure. Moreover, the figure shows the results of (\ref{eq_etanocsi}) with no CSIT/rate adaptation as a benchmark. Finally, Fig. \ref{fig_Figure6} studies the expected throughput $\eta$ for different values of estimation error variance $\kappa$ with SNR = 10, 19, 25 dB, in the case of partial CSIT. Also, the figure evaluates the tightness of the approximation results obtained by Lemma \ref{Lemma4}. Here,  we set $v =$ 114.5 km/h and $\delta = 5$ ms.

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure5.pdf}\\
\caption{Expected throughput $\eta$ in different cases, $v$ = 114 km/h, $\kappa$ = 1, and $\delta = $ 5 ms. Both the exact values estimated from  simulations as well as the analytical approximations from Lemma \ref{Lemma4} are presented.}\label{fig_Figure5}
\end{figure}



Setting SNR = 23 dB and $v = $ 120, 150 km/h in Fig. \ref{fig_Figure7},  we study the effect of the processing delay $\delta$ on the throughput. Finally, the outage probability is evaluated in Fig. \ref{fig_Figure8}, where the results are presented for different speeds with SNR = 10 dB, in the case of partial CSIT. Also, we present  the outage probability for $\delta = 5.35$ ms and $\delta = 4.68$ ms in Fig.  \ref{fig_Figure8}. 









From the figures, we can conclude the following points:
\begin{itemize}
    \item The approximation scheme of Lemma \ref{Lemma4} is tight for a broad range of parameter settings (Figs. \ref{fig_Figure5}, \ref{fig_Figure6}). Thus, the throughput-optimized rate allocation can be well approximated by (\ref{eq_appRF}), and the semi-linear approximation of Lemma \ref{Lemma1}/Corollaries \ref{coro1}-\ref{coro2} is a good approach to study the considered optimization problem.
    
\begin{figure}
%\vspace{-3mm}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure6.pdf}\\
 %\vspace{-4mm}
\caption{Expected throughput $\eta$ for different estimation errors $\kappa$ with SNR = 10, 19, 25 dB, in the case of partial CSIT, exact and approximation,  $v = $  114.5 km/h, and $\delta = 5$ ms. Both the exact values estimated from simulations as well as the analytical approximations from Lemma \ref{Lemma4} are presented.}\label{fig_Figure6}
\end{figure}
    
    \item With deployment of the PA, remarkable throughput gain is achieved especially in moderate/high SNRs (Fig. \ref{fig_Figure5}). Also, the throughput decreases when the estimation error is considered, i.e., $\kappa$ decreases. Finally, as can be seen in Figs.  \ref{fig_Figure5}, \ref{fig_Figure6}, with rate adaptation,  and without optimizing the processing delay/vehicle speed, the effect of estimation error on expected throughput  is small unless for large values of $\kappa$.
    
\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure7.pdf}\\
\caption{Expected throughput $\eta$ for different processing delays with SNR = 23 dB and $v$ = 120, 150 km/h in the case of partial adaptation. }\label{fig_Figure7}

\end{figure}

\begin{figure}
%\vspace{-3mm}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure8.pdf}\\
 %\vspace{-4mm}
\caption{Outage probability for different velocities with SNR = 10 dB, in the case of partial CSIT.}\label{fig_Figure8}

\end{figure}

    
    \item As it can be seen in Figs. \ref{fig_Figure7} and \ref{fig_Figure8}, for different channel estimation errors, there are optimal values for the vehicle speed and the BS processing delay optimizing the system throughput and outage probability. Note that the presence of the optimal speed/processing delay can be proved via (\ref{eq_d}) as well. Finally, the optimal value of the vehicle speed, in terms of throughput/outage probability, decreases with the processing delay. However, the optimal vehicle speed/processing delay, in terms of throughput/outage probability, is almost insensitive to the channel estimation error.
    




    \item With perfect channel estimation, the throughput/outage probability is sensitive to the speed variation, if we move away from the optimal speed (Figs. \ref{fig_Figure7} and \ref{fig_Figure8}). However, the sensitivity to the speed/processing delay variation decreases as the channel estimation error increases, i.e., $\kappa$ decreases (Figs. \ref{fig_Figure7} and \ref{fig_Figure8}). Finally, considering Figs. \ref{fig_Figure7} and \ref{fig_Figure8}, it is expected that adapting the processing delay, as a function of the vehicle speed, and implementing hybrid automatic repeat request protocols can improve the performance of the PA system. These points will be studied in our future works.

\end{itemize}









\section{Conclusion}
We derived a simple semi-linear approximation method for the first-order Marcum $Q$-function, as one of the functions of interest in different problem formulations of wireless networks. As we showed through various analysis, while the proposed approximation is not tight at the tails of the function, it is useful in different optimization- and expectation-based problem formulations. Particularly, as an application of interest, we used the proposed approximation to analyze the performance of PA setups using  rate adaptation. As we showed, with different levels of channel estimation error/processing delay, adaptive rate allocation can effectively compensate for the spatial mismatch problem, and improve the throughput/outage probability of PA networks.  It is expected that increasing the number of RA antennas will improve the performance of the PA system considerably. 





\appendix
\renewcommand{\thesection}{\Alph{section}}
\section{Proof of Lemma 2}
  \label{proof_Lemma2}
Using Corollary \ref{coro1},  we have
\begin{align}
G(\alpha,\rho)\simeq
\begin{cases}
\int_\rho^{\breve{c}_1}0\text{d}x + \int_{\breve{c}_1}^{\breve{c}_2}e^{-nx}x^{m}\times\nonumber\\
~~~\left(\frac{1}{\sqrt{2\pi}}(x-\alpha) + \frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\text{d}x +\nonumber\\
~~~\int_{\breve{c}_2}^{\infty}e^{-nx}x^{m}\text{d}x, ~~~~~~~~~~~~~~\mathrm{if}~  \rho < \breve{c}_1  \\ 
 \int_{\rho}^{\breve{c}_2}e^{-nx}x^{m}\times\nonumber\\
~~~\left(\frac{1}{\sqrt{2\pi}}(x-\alpha) + \frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\text{d}x +\nonumber\\
~~~\int_{\breve{c}_2}^{\infty}e^{-nx}x^{m}\text{d}x, ~~~~~~~~~~~~~~\mathrm{if}~  \breve{c}_1\leq\rho<\breve{c}_2,\nonumber\\
\int_\rho^{\infty} e^{-nx}x^{m}\text{d}x, ~~~~~~~~~~~~~~~~~~\mathrm{if}~  \rho\geq\breve{c}_2.
\end{cases}
\end{align}


Then, for $\rho\geq \breve{c}_2$, we obtain
\begin{align}
&    \int_\rho^\infty e^{-nx}\times x^{m}(1-Q_1(\alpha,x))\text{d}x\nonumber\\
  &  \overset{(d)}\simeq\int_\rho^\infty e^{-nx}\times x^{m}\text{d}x
   \overset{(e)}= \Gamma(m+1,n\rho)n^{-m-1}, 
\end{align}
while for $\rho<\breve{c}_2$, we have

\begin{align}
 &  \int_\rho^\infty e^{-nx}\times x^{m}(1-Q_1(\alpha,x))\text{d}x\nonumber\\
&    \overset{(f)}\simeq \int_{\max(\breve{c}_1,\rho)}^{\breve{c}_2} \left(\frac{1}{\sqrt{2\pi}}(x-\alpha) + 
\frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\times\nonumber\\
& ~~~~~~e^{-nx}x^{m}\text{d}x +\int_{\breve{c}_2}^\infty e^{-nx} x^{m}\text{d}x\nonumber\\
& \overset{(g)}= \Gamma(m+1,n\breve{c}_2)n^{-m-1} + \nonumber\\
&~~~~~~\left(-\frac{\alpha}{\sqrt{2\pi}}+0.5*\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\times n^{-m-1}\times\nonumber\\
&~~~~~~\left(\Gamma\left(m+1,n\max(\breve{c}_1,\rho)\right)-\Gamma\left(m+1,n\breve{c}_2\right)\right)+\nonumber\\
&~~~~~~\left(\Gamma(m+2,n\max(\breve{c}_1,\rho))-\Gamma(m+2,n\breve{c}_2)\right)\frac{n^{-m-2}}{\sqrt{2\pi}}.
\end{align}
Note that $(d)$ and $(f)$ come from Corollary \ref{coro1} while $(e)$ and $(g)$ use the fact that $\Gamma(s,x)\rightarrow 0$ as $x\rightarrow\infty$.


\section{Proof of Lemma 3}
\label{proof_Lemma3}
Using Lemma \ref{Lemma1}, the  integral (\ref{eq_integralT})  can be approximated as

1) for $\theta_2>\theta_1>c_2$, $T(\alpha,m,a,\theta_1,\theta_2) \simeq 0$,

2) for $c_1<\theta_1\leq c_2, \theta_2>\theta_1$,
\begin{align}
  &  T(\alpha,m,a,\theta_1,\theta_2) = \nonumber\\& ~~\int_{\theta_1}^{\min(c_2,\theta_2)} (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x,
\end{align}

3) for $\theta_1<c_1,\theta_2>c_1$,
\begin{align}
   & T(\alpha,m,a,\theta_1,\theta_2) \simeq \int_{\theta_1}^{c_1} e^{-mx}\log(1+ax)\text{d}x + \nonumber\\
   &~~ \int_{c_1}^{\min(c_2,\theta_2)} (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x,
\end{align}

4) for $\theta_1<\theta_2<c_1$,
\begin{align}
   & T(\alpha,m,a,\theta_1,\theta_2) \simeq \int_{\theta_1}^{\theta_2} e^{-mx}\log(1+ax)\text{d}x.
\end{align}

Then, consider case 3 where
\begin{align}
    T(\alpha,m,a,\theta_1,\theta_2) &= \int_{\theta_1}^{\theta_2} e^{-mx}\log(1+ax)Q_1(\alpha,x)\text{d}x\nonumber\\
    &\simeq \int_{\theta_1}^{c_1} e^{-mx}\log(1+ax)\text{d}x + \nonumber\\
   & \int_{c_1}^{\theta_2} (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x\nonumber\\
   & =  \mathcal{F}_1(c_1) -  \mathcal{F}_1(\theta_1) +  \mathcal{F}_2(\theta_2) -  \mathcal{F}_2(c_1),
\end{align}
with $n_1$ and $n_2$ being functions of the constant $\alpha$ and given by (\ref{eq_n1}) and (\ref{eq_n2}), respectively. Here, we assume $\theta_1<c_1$ and $c_2> \theta_2 > c_1$ for simplicity. The other cases can be proved with the same procedure. Moreover, the functions $\mathcal{F}_1(x)$ and $\mathcal{F}_2(x)$ are obtained by
\begin{align}
    \mathcal{F}_1(x) &= \int e^{-mx}\log(1+ax)\text{d}x\nonumber\\
    &\overset{(h)}= -\frac{e^{-mx}\log(ax+1)}{m}-\int -\frac{ae^{-mx}}{m(ax+1)} \text{d}x\nonumber\\
    & \overset{(i)}=  \frac{1}{m}\left(-e^{\frac{m}{a}}\operatorname{E_1}\left(mx+\frac{m}{a}\right)-e^{-mx}\log(ax+1)\right)+C,
\end{align}
and
\begin{align}
     \mathcal{F}_2(x)& =  \int (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x\nonumber\\
    &\overset{(j)} = -\frac{(mn_2x+n_2+mn_1)e^{-mx}\log(1+ax)}{m^2} - \nonumber\\
    &~~~\int \frac{a(-mn_2x-n2-mn_1)e^{-mx}}{m^2(ax+1)} \text{d}x\nonumber\\
    & \overset{(k)}= -\frac{(mn_2x+n_2+mn_1)e^{-mx}\log(1+ax)}{m^2} - \nonumber\\
    &~~~ -\frac{1}{a}\bigg(e^{\frac{m}{a}}(mn_2x+n_2+mn_1)\nonumber\\
    &~~~ \operatorname{E_1}\left(mx+\frac{m}{a}\right)\bigg)+
    \int - \frac{me^{\frac{m}{a}}n_2}{\operatorname{E_1}\left(mx+\frac{m}{a}\right)} \text{d}x\nonumber\\
    & \overset{(l)}= -\frac{(mn_2x+n_2+mn_1)e^{-mx}\log(1+ax)}{m^2} - \nonumber\\
    &~~~ -\frac{1}{a}\bigg(e^{\frac{m}{a}}(mn_2x+n_2+mn_1) \operatorname{E_1}\left(mx+\frac{m}{a}\right)\bigg)+\nonumber\\
    &~~~  \frac{n_2e^{-mx}}{a} - \frac{e^{\frac{m}{a}}n_2(mx+\frac{m}{a}) \operatorname{E_1}\left(mx+\frac{m}{a}\right)}{a}+C,
\end{align}
where $(h)$, $(j)$ and $(k)$ come from partial integration and some manipulations. Also, $(i)$ and $(l)$ use \cite[p. 195]{geller1969table}
\begin{align}
    \int \operatorname{E_1}(u) \text{d}u = u\operatorname{E_1}(u)-e^{-u}.
\end{align}










==> YourThesis/papers/T1/content1.tex <==
\begin{abstract}
First-order Marcum $Q$-function is observed in various problem formulations. However, it is not an easy-to-handle function. For this reason, in this paper, we first present a semi-linear approximation of the Marcum $Q$-function. Our proposed approximation is useful because it simplifies, e.g., various integral calculations including the Marcum $Q$-function as well as different operations such as parameter optimization. Then, as an example of interest, we apply our proposed approximation approach to the performance analysis of predictor antenna (PA) systems. Here, the PA system is referred to as a system with two sets of antennas on the roof of a vehicle. Then, the PA positioned in the front of the vehicle can be used to improve the channel state estimation for data transmission of the receive antenna  that is aligned behind the PA. Considering spatial mismatch due to the mobility, we derive closed-form expressions for the instantaneous and average throughput as well as the throughput-optimized rate allocation. As we show, our proposed approximation scheme enables us to analyze PA systems with high accuracy. Moreover, our results show that rate adaptation can improve the performance of PA systems with different levels of spatial mismatch.
\end{abstract}
\keywords{Backhaul, channel state information (CSI),  integrated access and backhaul (IAB), linear approximation, Marcum $Q$-function, mobility, mobile relay, outage probability, predictor antenna, rate adaptation, spatial correlation, throughput.}


\section{Introduction}
The first-order Marcum $Q$-function\footnote{To simplify the analysis, our paper concentrates on the approximation of the first-order Marcum-$Q$ function. However, our approximation technique can be easily extended to the cases with different orders of Marcum $Q$-function.} is defined as  \cite[Eq. (1)]{Bocus2013CLapproximation}
\begin{align}
    Q_1(\alpha,\beta) = \int_{\beta}^{\infty} xe^{-\frac{x^2+\alpha^2}{2}}I_0(x\alpha)\text{d}x,
\end{align}
where $\alpha, \beta \geq 0$ and $I_n(x) = (\frac{x}{2})^n \sum_{i=0}^{\infty}\frac{(\frac{x}{2})^{2i} }{i!\Gamma(n+i+1)}$ is the $n$-order modified Bessel function of the first kind, and $\Gamma(z) = \int_0^{\infty} x^{z-1}e^{-x} \mathrm{d}x$ represents the Gamma function. Reviewing the literature, the Marcum $Q$-function has appeared in many areas such as statistics/signal detection \cite{helstrom1994elements}, and in the performance analysis of different setups such as temporally correlated channels \cite{Makki2013TCfeedback}, spatial correlated channels \cite{Makki2011Eurasipcapacity},  free-space optical (FSO) links \cite{Makki2018WCLwireless}, relay networks \cite{Makki2016TVTperformance}, as well as  cognitive radio and radar systems \cite{Simon2003TWCsome,Suraweera2010TVTcapacity,Kang2003JSAClargest,Chen2004TCdistribution,Ma2000JSACunified,Zhang2002TCgeneral,Ghasemi2008ICMspectrum,Digham2007TCenergy, simon2002bookdigital,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan}. However, in these applications, the presence of the Marcum $Q$-function makes the mathematical analysis challenging, because it is  difficult to manipulate  with no closed-form  expressions especially when it appears in parameter optimizations and integral calculations. For this reason, several methods have been developed in \cite{Bocus2013CLapproximation,Fu2011GLOBECOMexponential,zhao2008ELtight,Simon2000TCexponential,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral}  to bound/approximate the Marcum $Q$-function. For example, \cite{Fu2011GLOBECOMexponential,zhao2008ELtight} have proposed  modified forms of the function, while \cite{Simon2000TCexponential,annamalai2001WCMCcauchy} have derived exponential-type bounds which are good for the bit error rate analysis at high signal-to-noise ratios (SNRs). Other types of bounds are expressed by, e.g., error function \cite{Kam2008TCcomputing} and Bessel functions \cite{Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral}. Some alternative methods have been also proposed in \cite{Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Bocus2013CLapproximation,Gaur2003TVTsome}. Although each of these approximation/bounding techniques are fairly tight for their considered problem formulation, they are still based on difficult functions, or have complicated summation/integration formations, which may be not easy to deal with in, e.g., integral calculations and parameter optimizations. 


In this paper, we first propose a simple semi-linear approximation of the first-order Marcum $Q$-function (Lemma \ref{Lemma1}, Corollaries \ref{coro1}-\ref{coro3}). As we show through various examples, the developed linearization technique is tight for a broad range of parameter settings. More importantly, the proposed approach simplifies various integral calculations and derivations and, consequently, allows us to express different expectation- and optimization-based operations in closed-form (Lemmas \ref{Lemma2}-\ref{Lemma4}). 

To demonstrate the usefulness of the proposed approximation technique in communication systems, we analyze the performance of predictor antenna (PA) systems which is of our current interest. Here, the PA system is referred to as a setup with two (sets of) antennas on the roof of a vehicle. The PA positioned in the front of a vehicle can be used to improve the channel state estimation for downlink data reception at the receive antenna (RA) on the vehicle that is aligned behind the PA \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects,Guo2019WCLrate}. The feasibility of such setups,   which are of interest particular in public transport systems such as trains and buses, but potentially also for the more design-constrained cars, have been previously shown through experimental tests \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive}, and different works have analyzed their system performance from different perspectives \cite{Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects,Guo2019WCLrate}. 

Among the challenges of the PA system is the spatial mismatch. If the RA does not arrive in the same position as the PA, the actual channel for the RA would not be identical to the one experienced by the PA before. Such inaccurate channel state information (CSI) estimation will affect the system performance considerably at moderate/high speeds \cite{DT2015ITSMmaking,Guo2019WCLrate}. In this paper, we address this problem by implementing adaptive rate allocation. In our proposed setup, the instantaneous CSI provided by the PA is used to adapt the data rate of the signals sent to the RA from the base station (BS). The problem is cast in the form of throughput maximization. Particularly, we use our developed approximation approach to derive closed-form expressions for the instantaneous and average throughput as well as the optimal rate allocation maximizing the throughput (Lemma \ref{Lemma4}). Moreover, we study the effect of different parameters such as the antennas distance, the vehicle speed, and the processing delay of the BS on the performance of PA setups. 


Our paper is different from the state-of-the-art literature because the proposed semi-linear approximation of the first-order Marcum $Q$-function and the derived closed-form expressions for the considered integrals have not been presented by, e.g., \cite{Bocus2013CLapproximation,helstrom1994elements,Makki2013TCfeedback,Makki2011Eurasipcapacity,Makki2018WCLwireless,Makki2016TVTperformance,Simon2003TWCsome,Suraweera2010TVTcapacity,Kang2003JSAClargest,Chen2004TCdistribution,Ma2000JSACunified,Zhang2002TCgeneral,Ghasemi2008ICMspectrum,Digham2007TCenergy, simon2002bookdigital,Fu2011GLOBECOMexponential,zhao2008ELtight,Simon2000TCexponential,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,Azari2018TCultra,Alam2014INFOCOMWrobust,Gao2018IAadmm,Shen2018TVToutage,Song2017JLTimpact,Tang2019IAan,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral,Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects,Guo2019WCLrate}. Also, as opposed to \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing,Apelfrojd2018PIMRCkalman,Jamaly2019IETeffects}, we perform analytical evaluations on the system performance with CSIT (T: at the transmitter)-based rate optimization to mitigate the effect of the spatial mismatch. Moreover, compared to our preliminary results in \cite{Guo2019WCLrate}, this paper develops the semi-linear approximation method for the Marcum $Q$-function and uses our proposed approximation method to analyze the performance of the PA system. Also, we perform deep analysis of the effect of various parameters, such as imperfect CSIT feedback schemes, and processing delay of the BS on the system performance. 



The simulation and the analytical results indicate that the proposed semi-linear approximation is useful for the mathematical analysis of different Marcum $Q$-function-based problem formulations. Particularly, our approximation method enables us to represent different Marcum $Q$-function-based integrations and optimizations in closed-form. Considering the PA system, our derived analytical results show that adaptive rate allocation can considerably improve the performance of the PA system in the presence of spatial mismatch. Finally, with different levels of channel estimation, our results show that there exists an optimal speed for the vehicle optimizing the throughput/outage probability, and the system performance is sensitive to the vehicle speed/processing delay as speed moves away from its optimal value. 


This paper is organized as follows. In Section II, we present our proposed semi-linear approximation of the first-order Marcum $Q$-function, and derive closed-form solutions for some integrals of interest. Section III deals with the application of the approximation in the PA system,  deriving closed-form expressions for the optimal rate adaptation, the instantaneous throughput as well as the expected throughput.  In this way, Sections II and III demonstrate examples on how the proposed approximation can be useful in, respectively, expectation- and optimization-based problem formulations including the Marcum $Q$-function. Concluding remarks are provided in Section IV. 





\section{Approximation of the first-order Marcum Q-function}
In this section, we present our semi-linear approximation of the cumulative distribution function (CDF) in the form of $y(\alpha, \beta ) = 1-Q_1(\alpha,\beta)$. The idea of this proposed approximation is to use one point and its corresponding slope in that point to create a line  approximating the CDF. The approximation method is summarized in Lemma \ref{Lemma1} as follows.
\begin{lem}\label{Lemma1}
 The CDF of the form $y(\alpha, \beta ) = 1-Q_1(\alpha,\beta)$ can be semi-linearly approximated as $Y(\alpha,\beta)\simeq \mathcal{Z}(\alpha, \beta)$ where
\begin{align}\label{eq_lema1}
\mathcal{Z}(\alpha, \beta)=
\begin{cases}
0,  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta < c_1  \\ 
 \frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}\times\\
 ~~~I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)\times\left(\beta-\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)+\\
 ~~~1-Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right),  ~~~~~~\mathrm{if}~ c_1 \leq\beta\leq c_2 \\
1,  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta> c_2,
\end{cases}
\end{align}
with
\begin{align}\label{eq_c1}
  & c_1(\alpha) =~~~ \max\Bigg(0,\frac{\alpha+\sqrt{\alpha^2+2}}{2}+\nonumber\\
    &~~~\frac{Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)-1}{\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)}\Bigg),
\end{align}
\begin{align}\label{eq_c2}
  & c_2(\alpha) = \frac{\alpha+\sqrt{\alpha^2+2}}{2}+\nonumber\\
  & ~~~\frac{Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)}{\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)}.
\end{align}
\end{lem}
\begin{proof}

We aim to approximate the CDF in the range $y \in [0, 1]$ by 
\begin{align}\label{eq_YY}
    y-y_0 = m(x-x_0),
\end{align}
where $\mathcal{C} = (x_0,y_0)$ is a point on the CDF curve and $m$ is the slope at point $\mathcal{C}$ of $y(\alpha,\beta)$. Then, the parts of the line outside this region are replaced by $y=0$ and $y=1$ (see Fig. \ref{fig_largealpha}).

To obtain a good approximation of the CDF, we select the point $\mathcal{C}$ by solving

\begin{align}\label{eq_partialsquare}
  x = \mathop{\arg}_{x} \left\{  \frac{\partial^2\left(1-Q_1(\alpha,x)\right)}{\partial x^2} = 0\right\}.
\end{align}
Using the derivative of the first-order Marcum $Q$-function with respect to $x$ \cite[Eq. (2)]{Pratt1968PIpartial}
\begin{align}\label{eq_derivativeMarcumQ}
    \frac{\partial Q_1(\alpha,x)}{\partial x} = -x e^{-\frac{\alpha^2+x^2}{2}}I_0(\alpha x),
\end{align}
(\ref{eq_partialsquare}) is equivalent to 
\begin{align}
  x =  \mathop{\arg}_{x} \left\{\frac{\partial\left(x e^{-\frac{\alpha^2+x^2}{2}}I_0(\alpha x)\right)}{\partial x}=0\right\}.
\end{align}
Using the approximation $I_0(x) \simeq \frac{e^x}{\sqrt{2\pi x}} $ \cite[Eq. (9.7.1)]{abramowitz1999ia} for moderate/large values of $x$ and writing
\begin{align}
    &~~~\frac{\partial\left(\sqrt{\frac{x}{2\pi \alpha}}e^{-\frac{(x-\alpha)^2}{2}}\right)}{\partial x} = 0\nonumber\\
  \Rightarrow &\frac{1}{\sqrt{2\pi\alpha}}\left(\frac{e^{-\frac{(x-\alpha)^2}{2}}}{2\sqrt{x}}+\sqrt{x}e^{-\frac{(x-\alpha)^2}{2}}(\alpha-x)\right)  = 0\nonumber\\
    \Rightarrow &2x^2-2\alpha x-1 =0,
\end{align}
we obtain 
\begin{align}\label{eq_beta0}
    x = \frac{\alpha+\sqrt{\alpha^2+2}}{2},
\end{align}
since $x\geq0$. In this way, we find the point 
\begin{align}
    \mathcal{C}=\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}, 1-Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)\right).
\end{align}

To calculate the slope $m$ at the point $\mathcal{C}$, we plug (\ref{eq_beta0}) into (\ref{eq_derivativeMarcumQ}) leading to
\begin{align}\label{eq_m}
  & m = \frac{\alpha+\sqrt{\alpha^2+2}}{2}\times\nonumber\\
    & ~~~e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right).
\end{align}
Finally, using (\ref{eq_YY}), (\ref{eq_beta0}) and (\ref{eq_m}), the CDF $y(\alpha, \beta) = 1-Q_1(\alpha,\beta)$ can be approximated  as in (\ref{eq_lema1}). Note that, because the CDF is limited to the range [0 1], the boundaries $c_1$ and $c_2$ in (\ref{eq_lema1}) are obtained by setting $y=0$ and $y=1$ which leads to the semi-linear approximation as given in (\ref{eq_lema1}).
\end{proof}


%==============
%Corollary 1, 2, 3
%==============
To further simplify the calculation, considering different ranges of $\alpha$, the approximation (\ref{eq_lema1}) can be simplified as stated in the following corollaries. 

\begin{corollary}\label{coro1}
For moderate/large values of $\alpha$, we have $y(\alpha,\beta)\simeq\tilde{\mathcal{Z}}(\alpha,\beta)$ where
\begin{align}\label{eq_coro1}
\tilde{\mathcal{Z}}(\alpha,\beta)\simeq
\begin{cases}
0,  ~~~~~~~~~~~~~\mathrm{if}~\beta < \frac{-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha  \\ 
\alpha e^{-\alpha^2}I_0(\alpha^2)(\beta-\alpha) + 
\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right), \\ ~~~~~~~~~~~~~~~~\mathrm{if}~\frac{-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha \leq\beta\\
~~~~~~~~~~~~~~~~~~~~\leq\frac{1-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha \\
1,  ~~~~~~~~~~~~~\mathrm{if}~ \beta> \frac{1-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha.
\end{cases}
\end{align}
\end{corollary}

\begin{proof}
Using (\ref{eq_beta0}) for moderate/large values of $\alpha$, we have $x \simeq \alpha$ and
\begin{align}
        \tilde{c}_1 = \frac{-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha,
\end{align}
\begin{align}
     \tilde{c}_2 = \frac{1-\frac{1}{2}\left(1-e^{-\alpha^2}I_0(\alpha^2)\right)}{\alpha e^{-\alpha^2}I_0(\alpha^2)}+\alpha,
\end{align}
which leads to (\ref{eq_coro1}). Note that in (\ref{eq_coro1}) we have used the fact that \cite[Eq.  (A-3-2)]{schwartz1995communication}
\begin{align}
    Q_1(\alpha,\alpha) = \frac{1}{2}\left(1+e^{-\alpha^2}I_0(\alpha^2)\right).
\end{align}
\end{proof}

\begin{corollary}\label{coro2}
For small values of $\alpha$, we have  $y(\alpha,\beta)\simeq\hat{ \mathcal{Z}}(\alpha,\beta)$ with
\begin{align}\label{eq_coro2}
\hat{ \mathcal{Z}}(\alpha,\beta)\simeq
\begin{cases}
0,   ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~\beta < \hat{c}_1  \\ 
\frac{\alpha+\sqrt{2}}{2}  e^{-\frac{\alpha^2+\left(\frac{\alpha+\sqrt{2}}{2}\right)^2}{2}}\times\\
~~~I_0\left(\frac{\alpha(\alpha+\sqrt{2})}{2}\right)(\beta-\frac{\alpha+\sqrt{2}}{2}) + \\
~~~1-Q_1\left(\alpha,\frac{\alpha+\sqrt{2}}{2}\right), 
~~~~~~~~\mathrm{if}~\hat{c}_1 \leq\beta\leq \hat{c}_2 \\
1, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta> \hat{c}_2
\end{cases}
\end{align}
with $\hat{c}_1$ and $\hat{c}_2$ given in (\ref{eq_hatc1}) and (\ref{eq_hatc2}), respectively.
\end{corollary}
\begin{proof}
Using (\ref{eq_beta0}) for small values of $\alpha$, we have $x\simeq \frac{\alpha+\sqrt{2}}{2}$, which leads to 
\begin{equation}\label{eq_hatc1}
    \hat{c}_1 = \frac{-1+Q_1\left(\alpha,\frac{\alpha+\sqrt{2}}{2}\right)}{\left(\frac{\alpha+\sqrt{2}}{2} \right)^2 e^{-\frac{\alpha^2+\left(\frac{\alpha+\sqrt{2}}{2}\right)^2}{2}} I_0\left(\frac{\alpha(\alpha+\sqrt{2})}{2}\right)}+\alpha,
\end{equation}
and
\begin{equation}\label{eq_hatc2}
    \hat{c}_2 = \frac{Q_1\left(\alpha,\frac{\alpha+\sqrt{2}}{2}\right)}{\left(\frac{\alpha+\sqrt{2}}{2} \right)^2 e^{-\frac{\alpha^2+\left(\frac{\alpha+\sqrt{2}}{2}\right)^2}{2}} I_0\left(\frac{\alpha(\alpha+\sqrt{2})}{2}\right)}+\alpha,
\end{equation}
and simplifies (\ref{eq_lema1}) to (\ref{eq_coro2}).
\end{proof}



\begin{corollary}\label{coro3}
Equation (\ref{eq_coro1}) can be further simplified as
\begin{align}\label{eq_coro3}
\breve{\mathcal{Z}}(\alpha,\beta)\simeq
\begin{cases}
0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \beta < \breve{c}_1  \\ 
\frac{1}{\sqrt{2\pi}}(\beta-\alpha) + 
\frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \breve{c}_1 \leq\beta\leq \breve{c}_2 \\
1, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta>\breve{c}_2
\end{cases}
\end{align}
with $\breve{c}_1$ and $\breve{c}_2$ given by (\ref{eq_dotc1}) and (\ref{eq_dotc2}), respectively.
\end{corollary}
\begin{proof}
For moderate/large values of $\alpha$, using the approximation $I_0(x) \simeq \frac{e^x}{\sqrt{2\pi x}}$ for (\ref{eq_coro1}) leads to (\ref{eq_coro3}) where
\begin{align}\label{eq_dotc1}
        \breve{c}_1 = -\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha,
\end{align}
and
\begin{align}\label{eq_dotc2}
     \breve{c}_2 = \sqrt{2\pi}-\frac{\sqrt{2\pi}}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)+\alpha.
\end{align}
\end{proof}










\begin{figure}
%\vspace{-3mm}
\centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.7\columnwidth]{Figure1.pdf}\\
 %\vspace{-4mm}
\caption{Illusion of the semi-linear approximation with Lemma \ref{Lemma1}, and Corollaries \ref{coro1}-\ref{coro3}. For each value of $\alpha\in[0.1,0.5,1]$, the approximated results obtained by Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro3} are compared with the exact value for a broad range of $\beta$.}
\label{fig_largealpha}
\end{figure}




To illustrate these semi-linear approximations, Fig. \ref{fig_largealpha} shows the CDF $y(\alpha,\beta)= 1-Q_1(\alpha,\beta)$ for both small and large values of $\alpha$, and compares the exact CDF with the approximation schemes of Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro3}. From Fig. \ref{fig_largealpha}, we can observe that Lemma \ref{Lemma1} is tight for a broad range of $\alpha$  and moderate values of $\beta$. Moreover, the tightness is improved as $\alpha$ decreases. Also,  Corollaries \ref{coro1}, \ref{coro3} and Corollary \ref{coro2} provide good approximations for large and small values of $\alpha$, respectively. Then, the proposed approximations are not tight at the tails of the CDF. However, as observed in \cite{Bocus2013CLapproximation,helstrom1994elements,Makki2013TCfeedback,Makki2011Eurasipcapacity,Makki2018WCLwireless,Makki2016TVTperformance,Simon2003TWCsome,Suraweera2010TVTcapacity,Kang2003JSAClargest,Chen2004TCdistribution,Ma2000JSACunified,Zhang2002TCgeneral,Ghasemi2008ICMspectrum,Digham2007TCenergy, simon2002bookdigital,Fu2011GLOBECOMexponential,zhao2008ELtight,Simon2000TCexponential,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,annamalai2001WCMCcauchy,Sofotasios2010ISWCSnovel,Li2010TCnew,andras2011Mathematicageneralized,Gaur2003TVTsome,Kam2008TCcomputing,Corazza2002TITnew,Baricz2009TITnew,chiani1999ELintegral}, in different applications, the Marcum $Q$-function is typically combined with other functions which tend to zero of the tails of the CDF. In such cases, the inaccuracy of the approximation at the tails does not affect the tightness of the final analysis. 













As an example, we first consider a general integral in the form of
\begin{align}\label{eq_integral}
G(\alpha,\rho)=\int_\rho^\infty{e^{-nx} x^m \left(1-Q_1(\alpha,x)\right)\text{d}x} ~~\forall n,m,\alpha,\rho>0.
\end{align}
Such an integral has been observed in various applications, e.g., \cite[eq. (1)]{Simon2003TWCsome}\cite[eq. (2)]{Cao2016CLsolutions}, \cite[eq. (1)]{sofotasios2015solutions}, \cite[eq. (3)]{Cui2012ELtwo}, and \cite[eq. (1)]{Gaur2003TVTsome}. However, depending on the values of $n, m$ and $\rho$, (\ref{eq_integral}) may have no closed-form expression. Using Lemma \ref{Lemma1}, $G(\alpha,\rho)$ can be approximated in closed-form as presented in Lemma \ref{Lemma2}.

\begin{lem}\label{Lemma2}
The integral (\ref{eq_integral}) is approximately given by
\begin{align}
G(\alpha,\rho)\simeq
\begin{cases}
\Gamma(m+1,n\rho)n^{-m-1}, ~~~~~~~~~~~~~~~~~~\mathrm{if}~  \rho \geq \breve{c}_2  \\ 
\Gamma(m+1,n\breve{c}_2)n^{-m-1} + \\
~~\left(-\frac{\alpha}{\sqrt{2\pi}}+0.5*\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\times n^{-m-1}\times\\
~~\left(\Gamma(m+1,n\max(\breve{c}_1,\rho))-\Gamma(m+1,n\breve{c}_2)\right)+\\
~~\left(\Gamma(m+2,n\max(\breve{c}_1,\rho))-\Gamma(m+2,n\breve{c}_2)\right)\times\\
~~\frac{n^{-m-2}}{\sqrt{2\pi}},
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  \rho<\breve{c}_2,
\end{cases}
\end{align}
where $\Gamma(s,x) = \int_{x}^{\infty} t^{s-1}e^{-t} \mathrm{d}t$ is the upper incomplete gamma function \cite[Eq. 6.5.1]{abramowitz1999ia}.
\end{lem}
\begin{proof}
See Appendix \ref{proof_Lemma2}. 
\end{proof}









As a second integration example of interest, consider
\begin{align}\label{eq_integralT}
    T(\alpha,m,a,\theta_1,\theta_2) = \int_{\theta_1}^{\theta_2} e^{-mx}\log(1+ax)Q_1(\alpha,x)\text{d}x \nonumber\\\forall m>0,a,\alpha,
\end{align}
with $\theta_2>\theta_1\geq0$, which does not have a closed-form expression for different values of $m, a, \alpha$. This integral is interesting as it is often used to analyse the expected performance of outage-limited systems, e.g,  \cite{Simon2003TWCsome,Simon2000TCexponential,Gaur2003TVTsome,6911973}. Then, using Lemma \ref{Lemma1}, $T(\alpha,m,a)$ can be approximated in closed-form as  follows.

\begin{lem}\label{Lemma3}
The integral (\ref{eq_integralT}) is approximately given by
\begin{align}
  T(\alpha,m,a,\theta_1,\theta_2)\simeq~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\nonumber\\
\begin{cases}
\mathcal{F}_1(\theta_2)-\mathcal{F}_1(\theta_1), ~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  0\leq\theta_1<\theta_2 < c_1  \\ 
\mathcal{F}_1(c_1)-\mathcal{F}_1(\theta_1)+\mathcal{F}_2(\max(c_2,\theta_2))-\mathcal{F}_2(c_1),  \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1<c_1, \theta_2\geq c_1\\
 \mathcal{F}_2(\max(c_2,\theta_2))-\mathcal{F}_2(c_1), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1>c_1\\
0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1 > c_2,
\end{cases}  
\end{align}
where 
$c_1$ and $c_2$ are given by (\ref{eq_c1}) and (\ref{eq_c2}), respectively. Moreover,
\begin{align}\label{eq_F1}
    \mathcal{F}_1(x) \doteq \frac{1}{m}\left(-e^{\frac{m}{a}}\operatorname{E_1}\left(mx+\frac{m}{a}\right)-e^{-mx}\log(ax+1)\right),
\end{align}
and
\begin{align}\label{eq_F2}
    \mathcal{F}_2(x) \doteq &~ \mathrm{e}^{-mx}\Bigg(\left(mn_2-an_2-amn_1\right)\mathrm{e}^\frac{m\left(ax+1\right)}{a}\nonumber\\&~~ \operatorname{E_1}\left(\frac{m\left(ax+1\right)}{a}\right)-
    a\left(mn_2x+n_2+mn_1\right)\nonumber\\&~~\log\left(ax+1\right)-an_2\Bigg),
\end{align}
with
\begin{align}\label{eq_n1}
    n_1 = 1+\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}\times\nonumber\\
 I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)\times\frac{\alpha+\sqrt{\alpha^2+2}}{2}-\nonumber\\
 1+Q_1\left(\alpha,\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right),
\end{align}
and
\begin{align}\label{eq_n2}
    n_2 = -\frac{\alpha+\sqrt{\alpha^2+2}}{2} e^{-\frac{1}{2}\left(\alpha^2+\left(\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right)^2\right)}\times\nonumber\\
 I_0\left(\alpha\frac{\alpha+\sqrt{\alpha^2+2}}{2}\right).
\end{align}
In (\ref{eq_F1}) and (\ref{eq_F2}), $\operatorname{E_1}(x) = \int_x^{\infty} \frac{e^{-t}}{t} \mathrm{d}t$ is the Exponential Integral function \cite[p. 228, (5.1.1)]{abramowitz1999ia}.
\end{lem}

\begin{proof}
See Appendix \ref{proof_Lemma3}.
\end{proof}

Finally, setting $m = 0$ in (\ref{eq_integralT}), i.e.,
\begin{align}\label{eq_integralTs}
     T(\alpha,0,a,\theta_1,\theta_2) = \int_{\theta_1}^{\theta_2} \log(1+ax)Q_1(\alpha,x)\text{d}x,  \forall a,\alpha,
\end{align}
one can follow the same procedure in (\ref{eq_integralT}) to approximate (\ref{eq_integralTs}) as
\begin{align}\label{eq_integralTss}
  T(\alpha,0,a,\theta_1,\theta_2)\simeq~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\nonumber\\
\begin{cases}
\mathcal{F}_3(\theta_2)-\mathcal{F}_3(\theta_1), ~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~  0\leq\theta_1<\theta_2 < c_1  \\ 
\mathcal{F}_3(c_1)-\mathcal{F}_3(\theta_1)+\mathcal{F}_4(\max(c_2,\theta_2))-\mathcal{F}_4(c_1),  \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1<c_1, \theta_2\geq c_1\\
 \mathcal{F}_4(\max(c_2,\theta_2))-\mathcal{F}_4(c_1), \\~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1>c_1\\
0, ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \theta_1 > c_2,
\end{cases}  
\end{align}
with $c_1$ and $c_2$ given by (\ref{eq_c1}) and (\ref{eq_c2}), respectively. Also,
\begin{align}
    \mathcal{F}_3 = \frac{(ax+1)(\log(ax+1)-1)}{a},
\end{align}
and
\begin{align}
    \mathcal{F}_4 = \frac{n_2\left((2a^2x^2-2)\log(ax+1)-a^2x^2+2ax\right)}{4a^2}+\nonumber\\\frac{n_1(ax+1)(\log(ax+1)-1)}{a},
\end{align}
where $n_1$ and $n_2$ are given by (\ref{eq_n1}) and (\ref{eq_n2}), respectively.


\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure2.pdf}\\
\caption{The  integral (\ref{eq_integral}) involving Marcum $Q$-function. Solid lines are exact values while crosses are the results obtained from Lemma \ref{Lemma2}, $\alpha = 2$,  $(m,n) = \{(4,4), (3,3), (2,2), (0,1), (1,1)\}$.}\label{fig_integrald}
\end{figure}


\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure3.pdf}\\
\caption{The integral (\ref{eq_integralT}) involving Marcum $Q$-function. Solid lines are exact values while crosses are the results obtained from Lemma \ref{Lemma3} and (\ref{eq_integralTss}). $\theta_1 = 0, \theta_2 = \infty$. }\label{fig_t2}
\end{figure}



In Figs. \ref{fig_integrald} and \ref{fig_t2}, we evaluate the tightness of the approximations in Lemmas \ref{Lemma2}, \ref{Lemma3} and (\ref{eq_integralTss}), for different values of $m$, $n$, $\rho$, $a$ and $\alpha$. From the figures, it can be observed that the approximation schemes of   Lemmas \ref{Lemma2}-\ref{Lemma3} and (\ref{eq_integralTss}) are very tight for different parameter settings, while our proposed semi-linear approximation makes it possible to represent the integrals in closed-form.  In this way, although the approximation (\ref{eq_lema1}) is not tight at the tails of the CDF, it gives tight approximation results when it appears in different integrals. Also, as we show in Section III, the semi-linear approximation scheme is efficient in optimization problems involving the Marcum $Q$-function. Finally, to tightly approximate the Marcum $Q$-function at the tails, which are the range of interest in, e.g., error probability analysis, one can use the approximation schemes of \cite{Simon2000TCexponential,annamalai2001WCMCcauchy}.






\section{Applications in PA Systems}
In Section II, we showed how the proposed approximation scheme enables us to derive closed-form expressions for a broad range of integrals, as required in various expectation-based calculations, e.g., \cite{Simon2003TWCsome,Cao2016CLsolutions,sofotasios2015solutions,Cui2012ELtwo,Gaur2003TVTsome,Simon2000TCexponential,6911973}. On other hand, the Marcum $Q$-function may also  appear in  optimization problems, e.g., \cite[eq. (8)]{Azari2018TCultra},\cite[eq. (9)]{Alam2014INFOCOMWrobust}, \cite[eq. (10)]{Gao2018IAadmm}, \cite[eq. (10)]{Shen2018TVToutage}, \cite[eq. (15)]{Song2017JLTimpact}, \cite[eq. (22)]{Tang2019IAan}.  For this reason, in this section, we provide an example of using our proposed semi-linear approximation in an optimization problem for the PA systems.

\subsection{Problem Formulation}
Vehicle communication is one of the most important use cases in 5G.  Here, the main focus is to provide efficient and reliable connections to cars and public transports, e.g., busses and trains. CSIT plays an important role in achieving these goals, since the data transmission efficiency can be improved by updating the transmission parameters relative to the instantaneous channel state.  However, the typical CSIT acquisition systems, which are mostly designed for (semi)static channels, may not work well for high-speed vehicles. This is because, depending on the vehicle speed, the position of the antennas may change quickly and the channel information becomes inaccurate.  To overcome this issue, \cite{Sternad2012WCNCWusing,DT2015ITSMmaking,BJ2017PIMRCpredictor,phan2018WSAadaptive,Jamaly2014EuCAPanalysis, BJ2017ICCWusing} propose the PA setup as shown in Fig. \ref{system}. With a PA setup, which is of interesting in Vehicle-to-everything (V2X) communications \cite{Sternad2012WCNCWusing} as well as integrated access and backhauling \cite{Teyeb2019VTCintegrated}, two antennas are deployed on the top of the vehicle. The first antenna,  the PA,  estimates the channel and sends feedback to the BS at time $t$. Then, the BS uses the CSIT provided by the PA to communicate with a second antenna, which we refer to as RA, at time $t+\delta$, where $\delta$ is the processing time at the BS. In this way, BS can use the CSIT acquired from the PA and perform various CSIT-based transmission schemes, e.g.,  \cite{Sternad2012WCNCWusing,BJ2017ICCWusing}.  


\begin{figure}
%\vspace{-3mm}
\centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.7\columnwidth]{Figure4.pdf}\\
 %\vspace{-4mm}
\caption{A PA system with  mismatch problem. Here, $\hat h$ is the channel between the BS and the PA while $h$ refers to the BS-RA link. The vehicle is moving with speed $v$ and the antenna separation is $d_\text{a}$. The red arrow indicates the spatial mismatch, i.e., when the RA does not reach at the same  point as the PA when sending pilots. Also, $d_\text{m}$ is the moving distance of the vehicle which is affected by the processing delay $\delta$ of the BS. }\label{system}
\end{figure}


We assume that the vehicle moves through a stationary electromagnetic standing wave pattern. Thus, if the RA reaches exactly the same position as the position of the PA when sending the pilots, it will experience the same channel and the CSIT will be perfect. However, if the RA does not reach the same spatial point as the PA, due to, e.g., the BS processing delay is not equal to the time that we need until the RA reaches the same point as the PA, the RA may receive the data in a place different from the one in which the PA was sending the pilots. Such spatial mismatch may lead to CSIT inaccuracy, which will affect the system performance considerably. Thus, we need adaptive schemes to compensate for it.

Considering downlink transmission in the BS-RA link, the received signal is given by
\begin{align}\label{eq_Y}
{{Y}} = \sqrt{P}hX + Z.
\end{align}
Here, $P$ represents the transmit power, $X$ is the input message with unit variance, and $h$ is the fading coefficient between the BS and the RA. Also, $Z \sim \mathcal{CN}(0,1)$ denotes the independent and identically distributed (IID) complex Gaussian noise added at the receiver.



We denote the channel coefficient of the PA-BS uplink as $\hat{h}$. Also, we define $d$ as the effective distance between  the place where the PA estimates the channel at time $t$, and the place where the RA reaches at time $t+\delta$. As can be seen in Fig. \ref{system}, $d$ can be calculated as
\begin{align}\label{eq_d}
    d = |d_\text{a} - d_\text{m} | = |d_\text{a} - v\delta|,
\end{align}
where $d_\text{m}$ is the moving distance of the vehicle during time interval $\delta$, and $v$ is the velocity of the vehicle. Also, $d_\text{a}$ is the antenna separation between the PA and the RA. In conjunction to (\ref{eq_d}), here, we assume $d$ can be calculated by the BS. 

Using the classical Jake's correlation model \cite[p. 2642]{Shin2003TITcapacity} by assuming uniform angular spectrum, the channel coefficient of the BS-RA downlink can be modeled as 
\begin{align}\label{eq_H}
    h = \sqrt{1-\sigma^2} \hat{h} + \sigma q,
\end{align}
Here, $q \sim \mathcal{CN}(0,1)$ which is independent of the known channel value $\hat{h}\sim \mathcal{CN}(0,1)$, and $\sigma$ is a function of the effective distance $d$ as 
\begin{align}
    \sigma = \frac{\frac{\phi_2^2-\phi_1^2}{\phi_1}}{\sqrt{ \left(\frac{\phi_2}{\phi_1}\right)^2 + \left(\frac{\phi_2^2-\phi_1^2}{\phi_1}\right)^2 }}.
\end{align}
Here, $\phi_1 = \bm{\Phi}_{1,1}^{1/2} $ and $\phi_2 = \bm{\Phi}_{1,2}^{1/2} $, where $\bm{\Phi}$ is  from Jake's model \cite[p. 2642]{Shin2003TITcapacity}
\begin{align}\label{eq_tildeH}
     \bigl[ \begin{smallmatrix}
  \hat{h}\\h
\end{smallmatrix} \bigr]= \bm{\Phi}^{1/2} \bm{H}_{\varepsilon}.
\end{align}
In (\ref{eq_tildeH}), $\bm{H}_{\varepsilon}$ has independent circularly-symmetric zero-mean complex Gaussian entries with unit variance, and $\bm{\Phi}$ is the channel correlation matrix with the $(i,j)$-th entry given by
\begin{align}\label{eq_phi}
    \Phi_{i,j} = J_0\left((i-j)\cdot2\pi d/ \lambda\right) \forall i,j.
\end{align}
Here, $J_n(x) = (\frac{x}{2})^n \sum_{i=0}^{\infty}\frac{(\frac{x}{2})^{2i}(-1)^{i} }{i!\Gamma(n+i+1)}$ represents the $n$-th order Bessel function of the first kind. Moreover, $\lambda$ denotes the carrier wavelength, i.e., $\lambda = c/f_\text{c}$ where $c$ is the speed of light and $f_\text{c}$ is the carrier frequency. 






From (\ref{eq_H}), for a given $\hat{h}$ and $\sigma \neq 0$, $|h|$ follows a Rician distribution, i.e., the  probability density function (PDF) of $|h|$ is given by 
\begin{align}
    f_{|h|\big|\hat{g}}(x) = \frac{2x}{\sigma^2}e^{-\frac{x^2+\hat{g}}{\sigma^2}}I_0\left(\frac{2x\sqrt{\hat{g}}}{\sigma^2}\right),
\end{align}
where $\hat{g} = |\hat{h}|^2$. Let us define the channel gain between BS-RA as $ g = |{h}|^2$. Then, the PDF of $f_{g|\hat{g}}$ is given by

\begin{align}\label{eq_pdf}
    f_{g|\hat{g}}(x) = \frac{1}{\sigma^2}e^{-\frac{x+\hat{g}}{\sigma^2}}I_0\left(\frac{2\sqrt{x\hat{g}}}{\sigma^2}\right),
\end{align}
which is non-central Chi-squared distributed with the CDF containing the first-order Marcum $Q$-function as
\begin{align}\label{eq_cdf}
    F_{g|\hat{g}}(x) = 1 - Q_1\left( \sqrt{\frac{2\hat{g}}{\sigma^2}}, \sqrt{\frac{2x}{\sigma^2}}  \right).
\end{align}



\subsection{Analytical Results on Rate Adaptation Using the Semi-Linear Approximation of the First-order Marcum Q-Function}\label{In Section III.C}
We assume that $d_\text{a}$, $\delta $ and $\hat{g}$ are known by the BS. It can be seen from (\ref{eq_pdf}) that $f_{g|\hat{g}}(x)$ is a function of $v$. For a given $v$, the distribution of $g$ is known by the BS, and a rate adaption scheme can be performed to improve the system performance.

For a given instantaneous value of $\hat g$, the data is transmitted with instantaneous rate $R_{|\hat{g}}$ nats-per-channel-use (npcu). If the instantaneous channel gain realization supports the transmitted data rate $R_{|\hat{g}}$, i.e., $\log(1+gP)\ge R_{|\hat{g}}$, the data can be successfully decoded. Otherwise,  outage occurs. Hence, the outage probability in each time slot is
\begin{align}
    \Pr(\text{outage}|\hat{g}) = F_{g|\hat{g}}\left(\frac{e^{R_{|\hat{g}}}-1}{P}\right).
\end{align}
Also, the instantaneous throughput for a given $\hat{g}$ is
\begin{align}\label{eq_opteta}
\eta_{|\hat {g}}\left(R_{|\hat{g}}\right)=R_{|\hat{g}}\left(1-\Pr\left(\log(1+gP)<R_{|\hat{g}}\right)\right),
\end{align}
and the optimal rate adaptation maximizing the  instantaneous throughput is obtained by
\begin{align}\label{eq_optR}
    R_{|\hat{g}}^{\text{opt}}&=\argmax_{R_{|\hat{g}}\geq 0} \left\{ \left(1-\Pr\left(\log(1+gP)<R_{|\hat{g}}\right)\right)R_{|\hat{g}} \right\}\nonumber\\
    &=\argmax_{R_{|\hat{g}}\geq 0} \left\{ \left(1-F_{g|\hat{g}}\left(\frac{e^{R_{|\hat{g}}}-1}{P}\right)\right) R_{|\hat{g}}\right\}\nonumber\\
    &=\argmax_{R_{|\hat{g}}\geq 0} \left\{ Q_1\left(  \sqrt{\frac{2\hat{g}}{\sigma^2}}, \sqrt{\frac{2(e^{R_{|\hat{g}}}-1)}{P\sigma^2}} \right)R_{|\hat{g}} \right\},
\end{align}
where the last equality comes from (\ref{eq_cdf}). 

Using the derivatives of the Marcum $Q$-function, (\ref{eq_optR}) does not have a closed-form solution\footnote{To solve (\ref{eq_optR}), one can use different approximation methods of Marcum $Q$-function, e.g., \cite{Guo2019WCLrate}. Here, we use Lemma \ref{Lemma1}/Corollaries \ref{coro1}-\ref{coro3} to solve (\ref{eq_optR}) to show the usefulness of the semi-linear approximation method. As shown, in Figs. \ref{fig_Figure5} and \ref{fig_Figure6}, the semi-linear approximation is tight for a broad range of parameter settings while it simplifies the optimization problem considerably. }. For this reason,  Lemma \ref{Lemma4}  uses the semi-linear approximation scheme of Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro3} to find the optimal data rate maximizing the instantaneous throughput.

\begin{lem}\label{Lemma4}
For a given channel realization $\hat{g}$, the throughput-optimized rate allocation is approximately given by (\ref{eq_appRF}) where $\mathcal{W}(\cdot)$ denotes the Lambert $\mathcal{W}$-function.
\end{lem}
\begin{proof}
The  approximation results of Lemma \ref{Lemma1} and Corollaries \ref{coro1}-\ref{coro3} can be generalized by $y(\alpha,\beta)\simeq\tilde{\mathcal{Z}}_{\text{general}}(\alpha,\beta)$ where
\begin{align}
\tilde{\mathcal{Z}}_{\text{general}}(\alpha,\beta)\simeq
\begin{cases}
0,~~~~~~~~~~~~~~~~~~~~\mathrm{if}~\beta < c_1(\alpha)  \\ 
o_1(\alpha)(\beta-o_2(\alpha)) + o_3,\\~~~~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ c_1(\alpha) \leq \beta \leq c_2(\alpha)\\ 
1,~~~~~~~~~~~~~~~~~~~~\mathrm{if}~ \beta> c_2(\alpha).
\end{cases}
\end{align}


$o_i,i=1,2,3$, are given by (\ref{eq_lema1}), (\ref{eq_coro1}), (\ref{eq_coro2}), or (\ref{eq_coro3}) depending on if we use Lemma \ref{Lemma1} or Corollaries \ref{coro1}-\ref{coro3}. In this way, (\ref{eq_opteta}) is approximated as
\begin{align}\label{eq_appR}
    \eta_{|\hat {g}}\simeq R_{|\hat{g}}\left(1-o_1(\alpha)\beta + o_1(\alpha)o_2(\alpha) - o_3(\alpha)\right),
\end{align}
where $\alpha = \sqrt{\frac{2\hat{g}}{\sigma^2}}$. To simplify the equation, we omit $\alpha$ in the following since it is a constant for given $\hat{g}$, $\sigma$. Then, setting the derivative of (\ref{eq_appR}) equal to zero, we obtain
\begin{align}\label{eq_appRF}
    & R_{|\hat{g}}^{\text{opt}}  \nonumber\\
    & = \operatorname*{arg}_{R_{|\hat{g}}\geq 0}\left\{ 1+o_1o_2-o_3-o_1\left(\frac{(R_{|\hat{g}}+2)e^{R_{|\hat{g}}}-2}{\sqrt{2P\sigma^2\left(e^{R_{|\hat{g}}}-1\right)}}\right)=0\right\}\nonumber\\
    % & = \operatorname*{arg}_{R_{|\hat{g}}\geq 0} \left\{ \left(\frac{(R_{|\hat{g}}+2)e^{R_{|\hat{g}}}-2}{\sqrt{2P\sigma^2\left(e^{R_{|\hat{g}}}-1\right)}}\right) = \frac{1+o_1o_2-o_3}{o_1}\right\}\nonumber\\
    & \overset{(a)}{\simeq} \operatorname*{arg}_{R_{|\hat{g}}\geq 0}\left\{ \left(\frac{R_{|\hat{g}}}{2}+1\right)e^{\frac{R_{|\hat{g}}}{2}+1} = \frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}\right\}\nonumber\\
    & \overset{(b)}{=} 2\mathcal{W}\left(\frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}-1\right).
\end{align}
Here,  $(a)$ comes from $e^{R_{|\hat{g}}}-1 \simeq e^{R_{|\hat{g}}} $ and $(R_{|\hat{g}}+2)e^{R_{|\hat{g}}}-2 \simeq (R_{|\hat{g}}+2)e^{R_{|\hat{g}}} $ which are appropriate at moderate/high values of $R_{|\hat{g}}$. Also, $(b)$ is obtained by the definition of the Lambert $\mathcal{W}$-function $xe^x = y \Leftrightarrow x = \mathcal{W}(y)$ \cite{corless1996lambertw}. 

\end{proof}

Finally, the expected throughput, averaged over multiple time slots, is obtained by $\eta = \mathbb{E}\left\{\eta|{\hat {g}}(R_{|\hat{g}}^{\text{opt}})\right\}$ with expectation over $\hat g$.  

Using (\ref{eq_appRF}) and the approximation \cite[Them. 2.1]{hoorfar2007approximation}

\begin{align}
    \mathcal{W}(x) \simeq \log(x)-\log\log(x), x\geq0,
\end{align}
we obtain
\begin{align}
    R_{|\hat{g}}^{\text{opt}}\simeq 2\log\left(\frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}-1\right)-\nonumber\\
    2\log\log\left(\frac{(1+o_1o_2-o_3)e\sqrt{2P\sigma^2}}{2o_1}-1\right)
\end{align}
which implies as the transmit power increases, the optimal instantaneous rate increases with the square root of the transmit power (approximately) logarithmically.

\subsection{On the Effect of Imperfect Channel Estimation}
In Section \ref{In Section III.C}, we assumed perfect channel estimation at the BS. Here, we follow the similar approach as in, e.g., \cite{Wang2007TWCperformance}, to add the effect of estimation error of $\hat{h}$ as an independent additive Gaussian variable whose variance is given by the accuracy of channel estimation. 

Let us define $\tilde h$ as the estimate of $\hat h$ at the BS. Then,  we further develop our channel model  (\ref{eq_H}) as
\begin{align}\label{eq_Htp}
    \tilde{h} = \kappa \hat{h} + \sqrt{1-\kappa^2} z, 
\end{align}
for each time slot, where $z \sim \mathcal{CN}(0,1)$ is a Gaussian noise which is uncorrelated with $H_{k}$. Also, $\kappa$ is a known correlation factor which represents estimation error of $\hat{h}$ by $\kappa = \frac{\mathbb{E}\{\tilde{h}\hat{h}^*\}}{\mathbb{E}\{|\hat{h}|^2\}}$. Substituting (\ref{eq_Htp}) into (\ref{eq_H}), we have
\begin{align}\label{eq_Ht}
    h = \kappa\sqrt{1-\sigma^2}\hat{h}+\kappa\sigma q+\sqrt{1-\kappa^2}z.
\end{align}
Then, because  $\kappa\sigma q + \sqrt{1-\kappa^2}z$ is equivalent to a new Gaussian variable 

$w \sim\mathcal{CN}\left(0,(\kappa\sigma)^2+1-\kappa^2\right)$, we can follow the same procedure as in (\ref{eq_optR})-(\ref{eq_appRF}) to analyze the system performance with imperfect channel estimation of the PA (see Figs. \ref{fig_Figure5}-\ref{fig_Figure6} for more discussions).

\subsection{Simulation Results}
In this part, we study the performance of the PA system and verify the tightness of the approximation scheme of Lemma \ref{Lemma4}. Particularly, we present the average throughput and the outage probability of the PA setup for different vehicle speeds/channel estimation errors. As an ultimate upper bound for the proposed rate adaptation scheme, we consider a genie-aided setup where we assume that the BS has perfect CSIT of the BS-RA link without uncertainty/outage probability. Then, as a lower-bound of the system performance, we consider the cases with no CSIT/rate adaptation as shown in Fig. \ref{fig_Figure5}. In the simulations, we set  $f_\text{c}$ = 2.68 GHz and $d_\text{a} = 1.5\lambda$. Finally, each point in the figures is obtained by averaging the system performance over $1\times10^5$ channel realizations.

\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure5.pdf}\\
\caption{Expected throughput $\eta$ in different cases, $v$ = 114 Km/h, $\kappa$ = 1, and $\delta = $ 5 ms. Both the exact values from simulation as well as the analytical approximations from Lemma \ref{Lemma4} are presented.}\label{fig_Figure5}
\end{figure}


In Fig. \ref{fig_Figure5}, we show the expected throughput $\eta$  in different cases for a broad range of signal-to-noise ratios (SNRs). Here, because the noise has unit variance, we define the SNR as $10\log_{10}P$. Also, we set $v = 114$ Km/h in Fig. \ref{fig_Figure5}  as defined in (\ref{eq_d}). The analytical results obtained by Lemma \ref{Lemma4} and Corollary \ref{coro2}, i.e., the approximation of (\ref{eq_optR}), are also presented. We have also checked the approximation result of Lemma \ref{Lemma4} while using Lemma \ref{Lemma1}/Corollaries \ref{coro1}, \ref{coro3}. Then, because the results are similar as those presented in Fig. \ref{fig_Figure5}, they are not included to the figure. Moreover, the figure shows the results with no CSIT/rate adaptation as a benchmark. Finally, Fig. \ref{fig_Figure6} studies the expected throughput $\eta$ for different values of estimation error variance $\kappa$ with SNR = 10, 19, 25 dB, in the case of partial CSIT. Also, the figure evaluates the tightness of the approximation results obtained by Lemma \ref{Lemma4}. Here,  we set $v =$ 114.5 Km/h and $\delta = 5$ ms.

Setting SNR = 23 dB and $v = $ 120, 150 Km/h in Fig. \ref{fig_Figure7},  we study the effect of the processing delay $\delta$ on the throughput. Finally, the outage probability is evaluated in Fig. \ref{fig_Figure8}, where the results are presented for different speeds with SNR = 10 dB, in the case of partial CSIT. Also, we present  the outage probability for $\delta = 5.35$ ms and $\delta = 4.68$ ms in Fig.  \ref{fig_Figure8}. 




\begin{figure}
%\vspace{-3mm}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure6.pdf}\\
 %\vspace{-4mm}
\caption{Expected throughput $\eta$ for different estimation errors $\kappa$ with SNR = 10, 19, 25 dB, in the case of partial CSIT, exact and approximation,  $v = $  114.5 Km/h, and $\delta = 5$ ms. Both the exact values from simulation as well as the analytical approximations from Lemma \ref{Lemma4} are presented.}\label{fig_Figure6}
\end{figure}


\begin{figure}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure7.pdf}\\
\caption{Expected throughput $\eta$ for different processing delays with SNR = 23 dB and $v$ = 120, 150 Km/h in the case of partial adaptation. }\label{fig_Figure7}

\end{figure}

\begin{figure}
%\vspace{-3mm}
\centering
  \includegraphics[width=0.7\columnwidth]{Figure8.pdf}\\
 %\vspace{-4mm}
\caption{Outage probability for different velocities with SNR = 10 dB, in the case of partial CSIT.}\label{fig_Figure8}

\end{figure}




From the figures, we can conclude the following points:
\begin{itemize}
    \item The approximation scheme of Lemma \ref{Lemma4} is tight for a broad range of parameter settings (Figs. \ref{fig_Figure5}, \ref{fig_Figure6}). Thus, the throughput-optimized rate allocation can be well approximated by (\ref{eq_appRF}), and the semi-linear approximation of Lemma \ref{Lemma1}/Corollaries \ref{coro1}-\ref{coro3} is a good approach to study the considered optimization problem.
    
    \item With deployment of the PA, remarkable throughput gain is achieved especially in moderate/high SNRs (Fig. \ref{fig_Figure5}). Also, the throughput decreases when the estimation error is considered, i.e., $\kappa$ decreases. Finally, as can be seen in Figs.  \ref{fig_Figure5}, \ref{fig_Figure6}, with rate adaptation,  and without optimizing the processing delay/vehicle speed, the effect of estimation error on expected throughput  is small unless for large values of $\kappa$.

    
    \item As it can be seen in Figs. \ref{fig_Figure7} and \ref{fig_Figure8}, for different channel estimation errors, there are optimal values for the vehicle speed and the BS processing delay optimizing the system throughput and outage probability. Note that the presence of the optimal speed/processing delay can be proved via (\ref{eq_d}) as well. Finally, the optimal value of the vehicle speed, in terms of throughput/outage probability, decreases with the processing delay. However, the optimal vehicle speed/processing delay, in terms of throughput/outage probability, is almost insensitive to the channel estimation error.

    \item With perfect channel estimation, the throughput/outage probability is sensitive to the speed variation, if we move away from the optimal speed (Figs. \ref{fig_Figure7} and \ref{fig_Figure8}). However, the sensitivity to the speed/processing delay variation decreases as the channel estimation error increases, i.e., $\kappa$ decreases (Figs. \ref{fig_Figure7} and \ref{fig_Figure8}). Finally, considering Figs. \ref{fig_Figure7} and \ref{fig_Figure8}, it is expected that adapting the processing delay, as a function of the vehicle speed, and implementing hybrid automatic repeat request protocols can improve the performance of the PA system. These points will be studied in our future works.

\end{itemize}





\section{Conclusion}
We derived a simple semi-linear approximation method for the first-order Marcum $Q$-function, as one of the functions of interest in different problem formulations of wireless networks. As we showed through various analysis, while the proposed approximation is not tight at the tails of the function, it is useful in different optimization- and expectation-based problem formulations. Particularly, as an application of interest, we used the proposed approximation to analyze the performance of PA setups using  rate adaptation. As we showed, with different levels of channel estimation error/processing delay, adaptive rate allocation can effectively compensate for the spatial mismatch problem, and improve the throughput/outage probability of PA networks.  It is expected that increasing the number of RA antennas will improve the performance of the PA system considerably.







% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/



\appendix
\renewcommand{\thesection}{\Alph{section}}
\section{Proof of Lemma \ref{Lemma2}}
  \label{proof_Lemma2}
Using Corollary \ref{coro1},  we have
\begin{align}
G(\alpha,\rho)\simeq
\begin{cases}
\int_\rho^{\breve{c}_1}0\text{d}x + \int_{\breve{c}_1}^{\breve{c}_2}e^{-nx}x^{m}\times\nonumber\\
~~~\left(\frac{1}{\sqrt{2\pi}}(x-\alpha) + \frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\text{d}x +\nonumber\\
~~~\int_{\breve{c}_2}^{\infty}e^{-nx}x^{m}\text{d}x, ~~~~~~~~~~~~~~\mathrm{if}~  \rho < \breve{c}_1  \\ 
 \int_{\rho}^{\breve{c}_2}e^{-nx}x^{m}\times\nonumber\\
~~~\left(\frac{1}{\sqrt{2\pi}}(x-\alpha) + \frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\text{d}x +\nonumber\\
~~~\int_{\breve{c}_2}^{\infty}e^{-nx}x^{m}\text{d}x, ~~~~~~~~~~~~~~\mathrm{if}~  \breve{c}_1\leq\rho<\breve{c}_2,\nonumber\\
\int_\rho^{\infty} e^{-nx}x^{m}\text{d}x, ~~~~~~~~~~~~~~~~~~\mathrm{if}~  \rho\geq\breve{c}_2.
\end{cases}
\end{align}


Then, for $\rho\geq \breve{c}_2$, we obtain
\begin{align}
&    \int_\rho^\infty e^{-nx}\times x^{m}(1-Q_1(\alpha,x))\text{d}x\nonumber\\
  &  \overset{(d)}\simeq\int_\rho^\infty e^{-nx}\times x^{m}\text{d}x
   \overset{(e)}= \Gamma(m+1,n\rho)n^{-m-1}, 
\end{align}
while for $\rho<\breve{c}_2$, we have

\begin{align}
 &  \int_\rho^\infty e^{-nx}\times x^{m}(1-Q_1(\alpha,x))\text{d}x\nonumber\\
&    \overset{(f)}\simeq \int_{\max(\breve{c}_1,\rho)}^{\breve{c}_2} \left(\frac{1}{\sqrt{2\pi}}(x-\alpha) + 
\frac{1}{2}\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\times\nonumber\\
& ~~~~~~e^{-nx}x^{m}\text{d}x +\int_{\breve{c}_2}^\infty e^{-nx} x^{m}\text{d}x\nonumber\\
& \overset{(g)}= \Gamma(m+1,n\breve{c}_2)n^{-m-1} + \nonumber\\
&~~~~~~\left(-\frac{\alpha}{\sqrt{2\pi}}+0.5*\left(1-\frac{1}{\sqrt{2\pi\alpha^2}}\right)\right)\times n^{-m-1}\times\nonumber\\
&~~~~~~\left(\Gamma\left(m+1,n\max(\breve{c}_1,\rho)\right)-\Gamma\left(m+1,n\breve{c}_2\right)\right)+\nonumber\\
&~~~~~~\left(\Gamma(m+2,n\max(\breve{c}_1,\rho))-\Gamma(m+2,n\breve{c}_2)\right)\frac{n^{-m-2}}{\sqrt{2\pi}}.
\end{align}
Note that $(d)$ and $(f)$ come from Corollary \ref{coro1} while $(e)$ and $(g)$ use the fact that $\Gamma(s,x)\rightarrow 0$ as $x\rightarrow\infty$.


\section{Proof of Lemma \ref{Lemma3}}
\label{proof_Lemma3}
Using Lemma \ref{Lemma1}, the  integral (\ref{eq_integralT})  can be approximated as

1) for $\theta_2>\theta_1>c_2$, $T(\alpha,m,a,\theta_1,\theta_2) \simeq 0$,

2) for $c_1<\theta_1\leq c_2, \theta_2>\theta_1$,
\begin{align}
  &  T(\alpha,m,a,\theta_1,\theta_2) = \nonumber\\& ~~\int_{\theta_1}^{\min(c_2,\theta_2)} (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x,
\end{align}

3) for $\theta_1<c_1,\theta_2>c_1$,
\begin{align}
   & T(\alpha,m,a,\theta_1,\theta_2) \simeq \int_{\theta_1}^{c_1} e^{-mx}\log(1+ax)\text{d}x + \nonumber\\
   &~~ \int_{c_1}^{\min(c_2,\theta_2)} (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x,
\end{align}

4) for $\theta_1<\theta_2<c_1$,
\begin{align}
   & T(\alpha,m,a,\theta_1,\theta_2) \simeq \int_{\theta_1}^{\theta_2} e^{-mx}\log(1+ax)\text{d}x.
\end{align}

Then, consider case 3 where
\begin{align}
    T(\alpha,m,a,\theta_1,\theta_2) &= \int_{\theta_1}^{\theta_2} e^{-mx}\log(1+ax)Q_1(\alpha,x)\text{d}x\nonumber\\
    &\simeq \int_{\theta_1}^{c_1} e^{-mx}\log(1+ax)\text{d}x + \nonumber\\
   & \int_{c_1}^{\theta_2} (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x\nonumber\\
   & =  \mathcal{F}_1(c_1) -  \mathcal{F}_1(\theta_1) +  \mathcal{F}_2(\theta_2) -  \mathcal{F}_2(c_1),
\end{align}
with $n_1$ and $n_2$ being functions of the constant $\alpha$ and given by (\ref{eq_n1}) and (\ref{eq_n2}), respectively. Here, we assume $\theta_1<c_1$ and $c_2> \theta_2 > c_1$ for simplicity. The other cases can be proved with the same procedure. Moreover, the functions $\mathcal{F}_1(x)$ and $\mathcal{F}_2(x)$ are obtained by
\begin{align}
    \mathcal{F}_1(x) &= \int e^{-mx}\log(1+ax)\text{d}x\nonumber\\
    &\overset{(h)}= -\frac{e^{-mx}\log(ax+1)}{m}-\int -\frac{ae^{-mx}}{m(ax+1)} \text{d}x\nonumber\\
    & \overset{(i)}=  \frac{1}{m}\left(-e^{\frac{m}{a}}\operatorname{E_1}\left(mx+\frac{m}{a}\right)-e^{-mx}\log(ax+1)\right)+C,
\end{align}
and
\begin{align}
     \mathcal{F}_2(x)& =  \int (n_2x+n_1)e^{-mx}\log(1+ax) \text{d}x\nonumber\\
    &\overset{(j)} = -\frac{(mn_2x+n_2+mn_1)e^{-mx}\log(1+ax)}{m^2} - \nonumber\\
    &~~~\int \frac{a(-mn_2x-n2-mn_1)e^{-mx}}{m^2(ax+1)} \text{d}x\nonumber\\
    & \overset{(k)}= -\frac{(mn_2x+n_2+mn_1)e^{-mx}\log(1+ax)}{m^2} - \nonumber\\
    &~~~ -\frac{1}{a}\bigg(e^{\frac{m}{a}}(mn_2x+n_2+mn_1)\nonumber\\
    &~~~ \operatorname{E_1}\left(mx+\frac{m}{a}\right)\bigg)+
    \int - \frac{me^{\frac{m}{a}}n_2}{\operatorname{E_1}\left(mx+\frac{m}{a}\right)} \text{d}x\nonumber\\
    & \overset{(l)}= -\frac{(mn_2x+n_2+mn_1)e^{-mx}\log(1+ax)}{m^2} - \nonumber\\
    &~~~ -\frac{1}{a}\bigg(e^{\frac{m}{a}}(mn_2x+n_2+mn_1) \operatorname{E_1}\left(mx+\frac{m}{a}\right)\bigg)+\nonumber\\
    &~~~  \frac{n_2e^{-mx}}{a} - \frac{e^{\frac{m}{a}}n_2(mx+\frac{m}{a}) \operatorname{E_1}\left(mx+\frac{m}{a}\right)}{a}+C,
\end{align}
where $(h)$, $(j)$ and $(k)$ come from partial integration and some manipulations. Also, $(i)$ and $(l)$ use \cite[p. 195]{geller1969table}
\begin{align}
    \int \operatorname{E_1}(u) \text{d}u = u\operatorname{E_1}(u)-e^{-u}.
\end{align}










==> YourThesis/papers/T1/info.tex <==


% only comma separated full names
\paperauthor{\textbf{H. Guo}, B. Makki, M.-S. Alouini, and T. Svensson}

% \paperinfo[short info]{full info}
\paperinfo[Submitted to  \textit{IEEE Transactions on Vehicular Technology}, May 2020]{
    \textit{Submitted to IEEE Transactions on Vehicular Technology},\\
	 May 2020.\\
	\copyright 2020 IEEE
}

% \papertitle[short title]{full title}
\papertitle[A Semi-Linear Approximation of the First-Order Marcum Q-Function with Application to Predictor Antenna Systems]{A semi-linear approximation of the first-order Marcum $Q$-function with application to predictor antenna systems}

% if you want to use an auto-generated paper summary, please fill in the variable \papersummary{}.
\papersummary{In this paper we...}






==> main111.tex <==
%
% This is the main/root file of the thesis, which initiate the template files
% No changes should be made to this file, it is just for easy access.
%
% All files that has to be changed is contained within the folder ``YourThesis''.
%
%\input{t.tex}




